Towards reliable real-time trajectory optimization

Motion planning is a key aspect of robotics. A common approach to address motion planning problems is trajectory optimization. Trajectory optimization can represent the high-level behaviors of robots through mathematical formulations. However, current trajectory optimization approaches have two main challenges. Firstly, their solution heavily depends on the initial guess, and they are prone to get stuck in local minima. Secondly, they face scalability limitations by increasing the number of constraints. This thesis endeavors to tackle these challenges by introducing four innovative trajectory optimization algorithms to improve reliability, scalability, and computational efficiency. There are two novel aspects of the proposed algorithms. The first key innovation is remodeling the kinematic constraints and collision avoidance constraints. Another key innovation lies in the design of algorithms that effectively utilize parallel computation on GPU accelerators. By using reformulated constraints and leveraging the computational power of GPUs, the proposed algorithms of this thesis demonstrate significant improvements in efficiency and scalability compared to the existing methods. Parallelization enables faster computation times, allowing for real-time decision-making in dynamic environments. Moreover, the algorithms are designed to adapt to changes in the environment, ensuring robust performance. Extensive benchmarking for each proposed optimizer validates their efficacy. Overall, this thesis makes a significant contribution to the field of trajectory optimization algorithms. It introduces innovative solutions that specifically address the challenges faced by existing methods. The proposed algorithms pave the way for more efficient and robust motion planning solutions in robotics by leveraging parallel computation and specific mathematical structures.

==> sections/chapterI.tex <==


\chapter{Motion Planning As An Optimization Problem}

\subsection{Symbols and Notations}

\noindent Small case letters with regular and bold font represent scalars and vectors, respectively. Matrices have upper-case bold fonts. The variable $t$ represents time stamps. The right superscript $T$ shows transpose. The left subscript $k$ denotes the trajectory optimizer's iteration. The rest of the symbols will be defined in the first place of use. 

\subsection{Trajectory Optimization Formulation }

\begin{subequations}
\begin{align}
   \min_{x(t), y(t), z(t)} c_1(x^{(q)}(t), y^{(q)}(t), z^{(q)}(t)),  
\label{cost_func}\\
   x^{(q)}(t), y^{(q)}(t), z^{(q)}(t)|_{t=t_{0}} = \textbf{b}_{0},\label{initial_cond} \\
   x^{(q)}(t), y^{(q)}(t), z^{(q)}(t)|_{t=t_{f}} = \textbf{b}_{f},\label{fin_cond}\\
    \dot{x}^{2}(t) + \dot{y}^{2}(t) + \dot{z}^{2}(t) \leq v^{2}_{max}, \label{vel_constraint} \\
    \ddot{x}^{2}(t) + \ddot{y}^{2}(t) + \ddot{z}^{2}(t) \leq a^{2}_{max}, \label{acc_constraint}\\
    s_{min} \leq (x(t), y(t), z(t)) \leq s_{max} \label{affine_ineq}  \\
    -\frac{(x(t)-
 x_{o, j}(t))^{2}}{a^2} - 
 \frac{(y(t)-y_{o, j}(t))^{2}}{a^2} 
  -\frac{(z(t)- 
z_{o, j}(t))^{2}}{b^2}
  + 1\leq 0, \label{coll_cond}
\end{align}
\end{subequations}
\normalsize

==> sections/contribution.tex <==
\chapter{Contribution}

This chapter provides a concise summary of the papers presented in this thesis. It covers the context of each paper, explores the existing methods within the context, highlights our novel contributions, defines the problem formulation, presents the main results, and investigates the interrelationships among each paper and the overarching theme of the thesis. In essence, it encapsulates the essence of the individual papers while providing a cohesive understanding of their collective significance within the broader context of the thesis.

%%%%%%%%%%%%%%%%%%%%%%Paper I %%%%%%%%%
\section{Paper I}
\subsection{Context:}
This paper introduces a novel trajectory optimization algorithm to generate collision-free trajectories within the affine motion models and convex cost functions framework. The optimization problem can be defined as:

\vspace{-0.2cm}
\small
\begin{subequations}
    \begin{align}
    \min _{x(t),y(t),z(t)}f_{x}+f_{y}+f_{z}+ I_{x}+I_{y}+I_{z}, \label{cost_1}
    \\
        -\frac{\hspace{-0.07cm}(x(t)\hspace{-0.09cm}-
 \hspace{-0.06cm}x_{o, j}(t)\hspace{-0.01cm})^{2}}{a^2}\hspace{-0.09cm} - \hspace{-0.09cm}
 \frac{\hspace{-0.07cm}(y(t) \hspace{-0.075cm}-\hspace{-0.065cm}y_{o, j}(t)\hspace{-0.02cm})^{2}}{a^2} 
  \hspace{-0.09cm}-\hspace{-0.09cm}\frac{\hspace{-0.07cm}(z(t)\hspace{-0.09cm}- 
 \hspace{-0.08cm}z_{o, j}(t)\hspace{-0.01cm})^{2}}{b^2}\hspace{-0.06cm} \hspace{-0.06cm}
  + \hspace{-0.05cm}1\leq 0,
\label{ellipse_avoid}
    \end{align}
\end{subequations}
\normalsize

\noindent Where $(x(t),y(t),z(t))$ and $(x_{o, j}(t),y_{o, j}(t),z_{o, j}(t))$ respectively denote the robot and the $j^{th}$ obstacle position at time $t$. The cost $f_{x}, f_{y}$ and $f_{z}$ are assumed to be a convex quadratic function of optimization variables, $(x(t),y(t),z(t))$, and their derivations. $I_{x}, I_{y}$ and $I_{z}$ are quadratic penalties formed from the affine bounds on the derivations of the optimization variables (refer to \cite{ghadimi2014optimal} for more details). The inequality \eqref{ellipse_avoid} presents the collision avoidance constraints. We assumed that obstacles are modeled as ellipsoids with dimensions $(a, a, b)$. 

Notably, \eqref{ellipse_avoid} exhibits a non-convex nature, introducing a challenge in solving the optimization problem \eqref{cost_1}-\eqref{ellipse_avoid}. An effective strategy to address this non-convexity involves leveraging its concave structure. Specifically, it is possible to establish a global upper bound through its affine approximation (see Fig. \ref{affine_approximation}) and solve the optimization problem. This simple adjustment forms the foundation of \gls{ccp} and has been widely adopted in recent literature \cite{boyd2004convex,rey2018fully}. This strategic adaptation not only simplifies the optimization problem but also enables the application of convex optimization techniques to effectively tackle the challenges posed by the non-convex nature of \eqref{ellipse_avoid}.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.5]{figures/affine_approx.png}
    \vspace{-0.3cm}
    \caption[Affine approximation of collision-avoidance constraints]{\small{(a)Feasible region (in green) in general, (b) feasible region (in green) using affine approximation of collision-avoidance constraints  }}
    \label{affine_approximation}
\end{figure}

While \gls{ccp} has proven effective, it faces critical limitations, particularly in cluttered and dynamic environments. The first limitation stems from the necessity of providing a collision-free initial trajectory guess, a condition challenging to meet in cluttered and dynamic scenarios. The second limitation arises from the need to solve a constrained optimization problem at each iteration, making real-time implementation impractical even for scenarios with a moderate number of obstacles.

In response to these challenges, we aim to propose a novel collision-free trajectory optimization method under affine motion models. Our method eliminates the need for an initial trajectory guess and boasts reduced complexity, offering a promising solution to the issues presented by \gls{ccp}. 

\vspace{0.2cm}
\subsection{Contribution:} 
Our primary contribution in this paper is the introduction of an innovative convex approximation for a trajectory optimization problem characterized by a unique modeling approach tailored for addressing collision avoidance constraints. Our model for collision avoidance constraints showcases a bi-convex structure (see Section \ref{}), a feature that can be effectively harnessed using advanced techniques such as \gls{am} and the augmented Lagrangian method. Moreover, our optimizer exhibits the following advantages over the \gls{ccp} method.

\begin{itemize}
\item \textbf{Efficient Computational Complexity:} The per-iteration computational complexity of our proposed optimizer is significantly lower than that of \gls{ccp}. Notably, it demonstrates a sub-linear increase with the number of collision avoidance constraints, in contrast to the quadratic increase observed in \gls{ccp} (refer to Fig.\ref{comptime_scaling}). Consequently, depending on the number of obstacles and the planning horizon length, our optimizer can be several orders of magnitude faster than a \gls{ccp}-based approach.
\item \textbf{Lower Computation time:} The reduced computation time of our proposed optimizer is underpinned by intriguing mathematical structures. For instance, certain components involve solving unconstrained \gls{qp} problems or, equivalently, solving linear equations in parallel. Additionally, other parts of our optimizer boast symbolic solutions. These solutions are available in a form that can be evaluated without necessitating computations involving matrix products, factorization, or inverses.
\end{itemize}

\begin{figure}[!h]
  \centering  
    \includegraphics[scale=0.30]{figures/time_scale.png}
    \vspace{-0.3cm}
\caption[Comparison of computation time scaling between our method and CCP]{\small{Scaling of computation time with the number of collision avoidance constraints: \gls{ccp} has quadratic scaling, while our optimizer shows sub-linear growth.}}
\label{comptime_scaling}
\end{figure}

We validate the efficacy of the proposed optimizer through comprehensive benchmarks, comparing its performance with \gls{ccp} across various challenging scenarios involving static and dynamic obstacles. Our evaluation encompasses considerations of smoothness cost, tracking cost, and computation time, providing a comprehensive understanding of the optimizer's capabilities and advantages.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Main Results:} \label{main_result_1}

In this section, we present our main theoretical breakthrough, a trajectory optimizer that outperforms \gls{ccp} in terms of computational efficiency. We initiate our discussion by providing the context and rationale behind the novel collision avoidance model we propose. Following this, we delve into the detail of how this model is leveraged within the optimization problem.

\noindent\textbf{Modelling collision avoidance constraint:} We adopt polar representation to reformulate the collision avoidance constraints \eqref{ellipse_avoid} as:

\small
\begin{subequations}
\begin{align}
\colorbox{my_green}{$x(t)-x_{o,j}(t)\hspace{-0.1cm}- ad_{o,j}(t)\hspace{-0.02cm}\cos{\alpha_{o,j}}(t)\hspace{-0.01cm}\sin{\beta_{o,j}}(t)=0,$} \label{collision_x}\\
\colorbox{my_pink}{$y(t)-y_{o,j}(t) 
-\hspace{-0.08cm}ad_{o,j}(t)\sin{\alpha_{o,j}(t)}\sin{\beta_{o,j}}(t)=0,$}\\
\colorbox{my_blue}{$z(t)  -z_{o,j}(t) -bd_{o,j}(t)\cos{\beta_{o,j}(t)}=0,$}
\\d_{o,j}(t) \geq 1, \forall t, 
\label{collision_d} 
\end{align}
\end{subequations}
\normalsize

\noindent Where $d_{o,j}(t),\alpha_{o,j}(t)$ and $\beta_{o,j}(t)$ are the line-of-sight distance and angles between the robot center and $j^{th}$ obstacle (see Fig. \ref{polar}(a)). These variables, derived from the polar representation, play a key role in guiding the optimization problem to avoid collisions effectively. To understand it better, let's consider a scenario where a point $(x(t), y(t), z(t))$ resides within an obstacle (Fig. \ref{polar}(b)). The collision can be avoided if we push away the considered point from the center of the obstacle, $(x_{o, j}(t), y_{o, j}(t), z_{o, j}(t))$ along the directions of $\alpha_{o,j}(t)$ and $\beta_{o,j}(t)$. The parameter $d_{o,j}(t)$ tells us how much the point needs to move away from the obstacle's center. We considered that $d_{o,j}(t)$ has an analytical form as \eqref{d_max}. Note that for clarity and to facilitate the tracking of changes in the optimization problem, each optimization formulation is highlighted in specific colors.

\small
\begin{align}
    d_{o,j}(t) = \max(1, \sqrt{\frac{(x(t)-x_{o,j}(t))^{2}}{a^2}, \frac{(y(t)-y_{o,j}(t))^{2}}{a^2}, \frac{(z(t)-z_{o,j}(t))^{2}}{b^2}}). \label{d_max}
\end{align}
\normalsize
\vspace{-0.2cm}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.98]{figures/polar_2.png}
    \vspace{-0.6cm}
    \caption[Intuition behind our collision avoidance model]{\small{(a) The polar relationship between the positions of the robot and the obstacle can be derived through trigonometry. The vector $d_{o,j}(t)$ represents the line-of-sight distance, representing the distance between the centers of the robot and the obstacle. It is defined by the polar angle, $\beta_{o,j}(t)$, which signifies the angle that $d_{o,j}(t)$ makes with the z-axis. Additionally, the azimuth angle, $\alpha_{o,j}(t)$, serves as the normal polar coordinate in the x-y plane. Together, these parameters provide a comprehensive polar representation capturing the geometric relationship between the robot and obstacle positions (b) Intuition behind our collision avoidance model: the point $\hspace{-0.1cm}(x(\hspace{-0.02cm}t\hspace{-0.02cm}),y(\hspace{-0.02cm}t\hspace{-0.02cm}),z(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.02cm})$ in collision with the obstacle needs to be pushed away from the center of the obstacle.}
}
\vspace{-0.3cm}
    \label{polar}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=1]{figures/collision_2.png}
%     \vspace{-0.3cm}
%     \caption[Intuition behind our collision avoidance model]{\hspace{-0.1cm}\small{Intuition behind our collision avoidance model: the point $\hspace{-0.1cm}(x(\hspace{-0.02cm}t\hspace{-0.02cm}),y(\hspace{-0.02cm}t\hspace{-0.02cm}),z(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.02cm})$ in collision with the obstacle needs to be pushed away from $(x_{o,j}(t),y_{o,j}(t),z_{o,j}(t))$.}}
%     \label{collision_2}
% \end{figure}

\noindent \textbf{Reformulating Trajectory Optimization Problem:} By considering the new formulation of collision avoidance constraints \eqref{collision_x}-\eqref{collision_d}, we reframe the optimization problem \eqref{cost_1}-\eqref{ellipse_avoid}

\small
\begin{subequations}
    \begin{align} 
    \min_{\scalebox{0.7}{$\begin{matrix} x_(t), y(t),z(t),c_{\alpha,j}(t),\\s_{\alpha,j}(t),c_{\beta,j}(t),
 s_{\beta,j}(t),\\ d_{o,j}(t),\alpha_{o,j}(t),\beta_{o,j}(t)   \end{matrix}$}}f_{x}+f_{y}+f_{z}+I_{x}+I_{y}+I_{z}, \label{cost_2}\\
  \colorbox{my_orange}{$   c_{\alpha,j}(t) = \cos{\alpha_{o,j}(t)}$},~  \colorbox{my_yellow}{$
     s_{\alpha,j}(t) = \sin{\alpha_{o,j}(t)} $},\label{new_var_1}\\
   \colorbox{my_purple}{$  c_{\beta,j}(t) = \cos{\beta_{o,j}(t)}$}, \colorbox{my_grey}{$
     s_{\beta,j}(t) = \sin{\beta_{o,j}(t)} $},\label{new_var_2}\\
    d_{o,j}(t) \geq 1,\\
\colorbox{my_green}{$x(t)-x_{o,j}(t)- ad_{o,j}c_{\alpha,j}(t)s_{\beta,j}(t)=0,$} \label{eq1} \\
\colorbox{my_pink}{$y(t)-y_{o,j}(t)
-ad_{o,j}s_{\alpha,j}(t)s_{\beta,j}(t)=0, $} \label{eq2}\\
\colorbox{my_blue}{$z(t)-z_{o,j}(t) -bd_{o,j}c_{\beta,j}(t)=0,$} 
\label{collision_proposed_1} 
    \end{align}
\end{subequations}
\normalsize

\noindent where the new variables $c_{\alpha,j}, s_{\alpha,j},c_{\beta,j}$ and $s_{\beta,j}$ act as a copy of sine and cosine of angles in the collision avoidance constraints \eqref{collision_x}-\eqref{collision_d}. To know how the new representation leverages the trajectory optimization problem, we use the augmented Lagrangian method and reformulate the \eqref{cost_2}-\eqref{collision_proposed_1} as the following

\vspace{-0.4cm}
\small
\begin{subequations}
    \begin{align}
     \min_{\scalebox{0.7}{$\begin{matrix} x(t), y(t),z(t),c_{\alpha,j}(t),s_{\alpha,j}(t),c_{\beta,j}(t),
 s_{\beta,j}(t), d_{o,j}(t),\alpha_{o,j}(t),\beta_{o,j}(t)   \end{matrix}$}}\hspace{-0.3cm}f_{x}+f_{y}+f_{z}+I_{x}+I_{y}+I_{z}, \nonumber \\
+\sum_{t=0}^{t=n_{p}}\sum_{j=1}^{j=n_{o}} \Big( \lambda_{x,j}(t)(\colorbox{my_green}{$x(t)-x_{o,j}(t)- ad_{o,j}c_{\alpha,j}(t)s_{\beta,j}(t)$}) \nonumber \\+ \frac{\rho_{o}}{2}(\colorbox{my_green}{$x(t)-x_{o,j}(t)- ad_{o,j}c_{\alpha,j}(t)s_{\beta,j}(t)$})^{2} \Big)\nonumber \\
+\sum_{t=0}^{t=n_{p}}\hspace{-0.1cm}\sum_{j=1}^{j=n_{o}}\Big(\lambda_{y,j}(t)(\colorbox{my_pink}{$y(t)-y_{o,j}(t)
-ad_{o,j}s_{\alpha,j}(t)s_{\beta,j}(t) $}) \nonumber \\
+ \frac{\rho_{o}}{2}(\colorbox{my_pink}{$y(t)-y_{o,j}(t)
-ad_{o,j}s_{\alpha,j}(t)s_{\beta,j}(t) $}) \Big)
\nonumber \\
+\sum_{t=0}^{t=n_{p}}\sum_{j=1}^{j=n_{o}}\Big(\lambda_{z,j}(t)(\colorbox{my_blue}{$z(t)-z_{o,j}(t) -bd_{o,j}c_{\beta,j}(t)$} ) \nonumber \\
+ \frac{\rho_{o}}{2}(\colorbox{my_blue}{$z(t)-z_{o,j}(t) -bd_{o,j}c_{\beta,j}(t)$} )\Big) \nonumber \\
+\hspace{-0.22cm}\sum_{t=0}^{t=n_{p}}\hspace{-0.1cm}\sum_{j=1}^{j=n_{o}}\hspace{-0.16cm}\Big(\hspace{-0.06cm}\frac{\rho}{2}(\colorbox{my_orange}{$\hspace{-0.05cm}c_{\alpha,j}\hspace{-0.04cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}- \hspace{-0.07cm}\cos{\alpha_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{c_{\alpha,j}}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.2cm}+\hspace{-0.12cm}\frac{\rho}{2}(\colorbox{my_yellow}{$s_{\alpha,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}- \hspace{-0.05cm}\sin{\alpha_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{s_{\alpha,j}}\hspace{-0.04cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.1cm}\Big) \nonumber 
\\
+\hspace{-0.22cm}\sum_{t=0}^{t=n_{p}}\hspace{-0.1cm}\sum_{j=1}^{j=n_{o}}\hspace{-0.16cm}\Big(\hspace{-0.06cm}
\frac{\rho}{2}(\colorbox{my_purple}{$\hspace{-0.05cm}c_{\beta,j}\hspace{-0.04cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}- \hspace{-0.07cm}\cos{\beta_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})}$}\hspace{-0.2cm}+ \hspace{-0.12cm}\frac{\lambda_{c_{\beta,j}}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho})^{2}\hspace{-0.2cm}+\hspace{-0.12cm}\frac{\rho}{2}(\colorbox{my_grey}{$s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.05cm} \sin{\beta_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{s_{\beta,j}}\hspace{-0.04cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho})^{2}\hspace{-0.1cm}\Big) \label{cost_aug}\\
d_{o,j}(t) \geq 1, \label{ineq_1}
    \end{align}
\end{subequations}
\normalsize

\noindent where $n_{p}$ and $n_{o}$ stands for the number of planning steps and obstacles, respectively. The parameters $\hspace{-0.1cm}\lambda_{x,j}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.03cm}\lambda_{y,j}(\hspace{-0.02cm}t\hspace{-0.02cm}),\hspace{-0.03cm}\lambda_{z,j}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.03cm}\lambda_{c_{\alpha,j}}\hspace{-0.03cm}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.03cm}\lambda_{s_{\alpha,j}}\hspace{-0.03cm}(\hspace{-0.02cm}t\hspace{-0.02cm}),\hspace{-0.03cm}\lambda_{c_{\beta,j}}(\hspace{-0.02cm}t\hspace{-0.02cm})$ and $\lambda_{s_{\beta,j}}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm})$ are Lagrange multipliers. The $\rho_{o}$ and $\rho$ are scalar. As evident, we relaxed the equality constraints in \eqref{eq1}-\eqref{collision_proposed_1} and transferred them~into cost function \eqref{cost_aug} using a combination of quadratic penalties and linear terms multiplied with Lagrange multipliers. Along similar lines, we also relaxed the equality constraints in \eqref{new_var_1}-\eqref{new_var_2} as quadratic penalties in~\eqref{cost_aug}.
     
On initial inspection, the formulation \eqref{cost_aug}-\eqref{ineq_1} may seem like a typical non-linear programming problem. However, upon closer examination, we recognize its bi-convex structure within the space $(x(t),y(t), z(t))$, $d_{o,j}(t)$, $(c_{\alpha,j}(t), s_{\alpha,j})(t)$, and $(c_{\beta,j}(t),s_{\beta,j}(t))$. This unique structure is particularly advantageous, as it enables the application of techniques such as \gls{am} to effectively resolve the trajectory optimization problem. Alg. \ref{alg_1} outlines the step-by-step process of solving \eqref{cost_aug}-\eqref{ineq_1}. We comprehensively analyze each stage of Alg. \ref{alg_1} in the subsequent paragraphs

\noindent \textbf{Analysis and Description of Alg. \ref{alg_1}: } Now, the details of Alg. \ref{alg_1} can be explained as following:

\begin{itemize}
    \item \textbf{Lines 1-2:} Our algorithm begins with initializing $^{k}d_{o,j}(t)$, $^{k}\alpha_{o,j}(t)$, and $^{k}\beta_{o,j}(t)$, and subsequently calculating $^{k}c_{\alpha,j}(t)$, $^{k}s_{\alpha,j}(t)$, $^{k}c_{\beta,j}(t)$, and $^{k}s_{\beta,j}(t)$ at $k=0$.
    \item \textbf{Line 3:} Following this, we compute the optimization variables $^{k+1}x(t),^{k+1}y(t)~ \text{and} ^{k+1}z(t)$. Thus, first, we inspect equations \eqref{cost_aug}-\eqref{ineq_1} and identify terms associated with $x(t),y(t)$, and $z(t)$ and rewrite the trajectory optimization as \eqref{com_x}-\eqref{com_z}. Remarkably, given values of $^{k}d_{o,j}(t)$, $^{k}\alpha_{o,j}(t)$, and $^{k}\beta_{o,j}(t)$, \eqref{com_x}-\eqref{com_z} are decoupled from each other, as they involve distinct terms (illustrated in different colors). So they can be solved in parallel. To solve trajectory optimization, \eqref{com_x}, we parametrize $x(t)$ and its derivatives as 

\vspace{-0.2cm}
\small
\begin{align}
    \begin{bmatrix}
x(t_1)\\
x(t_2)\\
\vdots\\
x(t_{n_p})
\end{bmatrix} = \textbf{P}\textbf{c}_x, \begin{bmatrix}
\dot{x}(t_1)\\
\dot{x}(t_2)\\
\vdots\\
\dot{x}(t_{n_p})
\end{bmatrix} = \dot{\textbf{P}}\textbf{c}_x,  \begin{bmatrix}
\ddot{x}(t_1)\\
\ddot{x}(t_2)\\
\vdots\\
\ddot{x}(t_{n_p})
\end{bmatrix} = \ddot{\textbf{P}}\textbf{c}_x,
\label{param}
\end{align}
\normalsize

\noindent Where $\textbf{P}$ is a matrix constructed with time-dependent basis functions (such as polynomials), and $\textbf{c}_x$ represents the coefficients of these polynomials (see Section \ref{}). Utilizing \eqref{param}, since the first two terms in \eqref{com_x} have the quadratic structure, they can be formulated as:

\vspace{-0.3cm}
\small
\begin{align}
f_x+\mathcal{I}_x = \frac{1}{2}\textbf{c}_x^T\textbf{Q}_x\textbf{c}_x+\textbf{q}_x^T\textbf{c}_x.
\label{quad_form}
\end{align}
\normalsize

\noindent Also, by substituting \eqref{param} into the last two terms of \eqref{com_x} and some simplifications, an unconstrained quadratic programming problem \eqref{com_x} can be reduced to solving the following linear equations (see Section \ref{} for more detail).

\vspace{-0.2cm}
\small
\begin{align}
(\textbf{Q}_x+\rho_{o}n_{o}\textbf{P}^T\textbf{P})\textbf{c}_x\hspace{-0.1cm}=\hspace{-0.1cm}-(\textbf{q}_x\hspace{-0.1cm}+\hspace{-0.1cm}\sum_{j=1}^{n_{o}}\textbf{P}^T\boldsymbol{\lambda}_{x,j}\hspace{-0.1cm}-\hspace{-0.1cm}\rho_{o}\textbf{P}^T(\textbf{x}_{o,j}\hspace{-0.1cm}+\hspace{-0.1cm}a\textbf{d}_{o,j}\textbf{c}_{\alpha,j}\textbf{s}_{\beta,j})),
\label{step_x_2d_simplify}
\end{align}
\normalsize

\noindent where $\boldsymbol{\lambda}_{x,j}, \textbf{x}_{o,j}, \textbf{d}_{o,j},\textbf{c}_{\alpha,j}$ and $\textbf{s}_{\beta,j}$ are formed by stacking $\lambda_{x,j}(t), x_{o,j}(t), d_{o,j}(t),c_{\alpha,j}(t)$ and $s_{\beta,j}(t)$ at different time steps. Similarly, we solve \eqref{com_y} and \eqref{com_z} to compute $y(t)$ and $z(t)$.

\item \textbf{Line 4:} In this stage, we derive the optimization variables $^{k+1}c_{\alpha,j}(t)$ and $^{k+1}s_{\alpha,j}(t)$. To compute these variables, we scrutinize equations \eqref{cost_aug}-\eqref{ineq_1} and identify terms associated with $c_{\alpha,j}(t)$ and $s_{\alpha,j}(t)$. The trajectory optimization is then reformulated as \eqref{com_c_alpha}-\eqref{com_s_alpha}. Importantly, with given values of $^{k}d_{o,j}(t)$, $^{k+1}x(t)$, $^{k+1}y(t)$, $^{k+1}z(t)$, $^{k}\alpha_{o,j}(t)$ and $^{k}\beta_{o,j}(t)$, the trajectory optimization problems \eqref{com_c_alpha}-\eqref{com_s_alpha} are independent, featuring distinct terms (color-coded for clarity). Thus, they are thus amenable to parallel computation. Crucially, for a specific obstacle index $j$, $^{k+1}c_{\alpha,j}(t)$ and $^{k+1}s_{\alpha,j}(t)$ are temporally uncorrelated. Similar to line 3, we stack our optimization variables at different time instances. Moreover, we observe the decoupling of optimization variables across various obstacles. Consequently, optimization \eqref{com_c_alpha}-\eqref{com_s_alpha} can be decomposed into $n_{o}\times n_{p}$ parallel optimizations, each entailing the minimization of a single-variable quadratic function. The solutions for each can be derived symbolically, further enhancing the computational efficiency of the algorithm.

\item \textbf{Line 5:} While optimization \eqref{com_alpha} poses a non-convex challenge, an approximate solution can be derived through simple geometric intuition. Illustrated in Fig. \ref{polar} (b), each set of feasible $x(t)- x_{o,j}(t)$, $y(t)- y_{o,j}(t)$, and $z(t)- z_{o,j}(t)$ forms an ellipsoid centered at the origin with dimensions $(ad_{o,j}(t),ad_{o,j}(t),bd_{o,j}(t))$. Consequently, \eqref{com_alpha} can be viewed and obtained as a projection of $x(t)- x_{o,j}(t)$ and $y(t)- y_{o,j}(t)$ onto an axis-aligned ellipsoid centered at the origin. 

\item \textbf{Line 6:} In this phase, we determine the optimization variables $^{k+1}c_{\beta,j}(t)$ and $^{k+1}s_{\beta,j}(t)$. To achieve this, we meticulously examine equations \eqref{cost_aug}-\eqref{ineq_1}, isolating terms associated with $c_{\beta,j}(t)$ and $s_{\beta,j}(t)$. The trajectory optimization is then reconfigured as \eqref{com_c_alpha}-\eqref{com_s_alpha}. Importantly, given values of $^{k}d_{o,j}(t)$, $^{k+1}x(t)$, $^{k+1}y(t)$, and $^{k+1}\alpha_{o,j}(t)$, the trajectory optimization problems \eqref{com_c_beta}-\eqref{com_s_beta} are independent, featuring distinct terms (color-coded for clarity). Hence, they lend themselves to parallel computation.  Similar to line 4, our optimization problems \eqref{com_c_beta}-\eqref{com_s_beta} can be decomposed into $n_{o}\times n_{p}$ parallel optimizations, each entailing the minimization of a single-variable quadratic function. 

\item \textbf{Line 7:} Similar to the intuition applied in line 5, optimization problem \eqref{com_beta} can be understood and derived as a projection of $z(t)- z_{o,j}(t)$ and $y(t)- y_{o,j}(t)$ onto an axis-aligned ellipsoid centered at the origin.

\item \textbf{Line 8:} We compute $^{k+1}d_{o,j}(t)$ using \eqref{d_max}.

\item \textbf{Line 9:} In this step, we update the Lagrange multipliers based on \eqref{lamda_x}-\eqref{lamda_s_beta}. The rules for these updates are adopted from \cite{boyd2011distributed}. Additionally, in each iteration, we increment the weights of the quadratic penalties, $\rho$ and $\rho_{o}$, if the residuals do not fall below the specified threshold.

\vspace{-0.2cm}
\small
\begin{subequations}
    \begin{align}
\hspace{-0.33cm}^{k+1}\lambda_{x\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.02cm}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.1cm}=\hspace{-0.08cm}^{k}\lambda_{x\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.1cm}+\hspace{-0.1cm}\rho_{o}
  (\colorbox{my_green}{$\hspace{-0.1cm}^{k+1}x(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}x_{o\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k+1}d_{o\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}^{k+1}c_{\alpha\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.02cm}t\hspace{-0.03cm})^{k+1}s_{\beta,j}(\hspace{-0.02cm}t\hspace{-0.03cm}))$},\label{lamda_x} \\
\hspace{-0.33cm}^{k+1}\lambda_{y\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}= \hspace{-0.08cm}^{k}\lambda_{y\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho_{o} (\colorbox{my_pink}{$\hspace{-0.1cm}^{k+1}y(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}y_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k+1}d_{o\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}^{k+1}s_{\alpha\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.02cm}t\hspace{-0.03cm})^{k+1}s_{\beta,j}(\hspace{-0.02cm}t\hspace{-0.03cm}))\hspace{-0.1cm}$}
  ,\label{lamda_y}\\^{k+1}\lambda_{z\hspace{-0.02cm},\hspace{-0.02cm}j} (\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}= \hspace{-0.08cm}^{k}\lambda_{z\hspace{-0.02cm},\hspace{-0.02cm}j}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho_{o}(\colorbox{my_blue}{$\hspace{-0.1cm}^{k+1}z(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}z_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}b\hspace{0.03cm}^{k+1}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}^{k+1}c_{\beta,j}(\hspace{-0.02cm}t\hspace{-0.03cm}))$}, \label{lamda_z}\\
^{k+1}\lambda_{c_{\alpha,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}=\hspace{-0.08cm}
^{k}\lambda_{c_{\alpha,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho (\colorbox{my_orange}{$   c_{\alpha,j}(t) - \cos{\alpha_{o,j}(t)})$}, \label{lamda_c_alpha}\\
^{k+1}\lambda_{s_{\alpha,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}=\hspace{-0.08cm}
^{k}\lambda_{s_{\alpha,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho( \colorbox{my_yellow}{$
     s_{\alpha,j}(t) - \sin{\alpha_{o,j}(t)}) $},\label{lamda_s_alpha}\\
^{k+1}\lambda_{c_{\beta,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}=\hspace{-0.08cm}
^{k}\lambda_{c_{\beta,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho \colorbox{my_purple}{$ ( c_{\beta,j}(t) - \cos{\beta_{o,j}(t)})$}, \label{lamda_c_beta}\\ 
^{k+1}\lambda_{s_{\beta,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}=\hspace{-0.08cm}
^{k}\lambda_{s_{\beta,\hspace{-0.02cm}j}}(\hspace{-0.035cm}t\hspace{-0.035cm})\hspace{-0.08cm}+\hspace{-0.08cm}\rho\colorbox{my_grey}{$(
     s_{\beta,j}(t) - \sin{\beta_{o,j}(t)}). $} \label{lamda_s_beta}
\end{align}
\end{subequations}
\normalsize
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!h]
\DontPrintSemicolon
\SetAlgoLined
\SetNoFillComment
\scriptsize
\caption{\scriptsize Alternating Minimization for Solving \eqref{cost_aug}-\eqref{ineq_1}  }\label{alg_1}
\KwInitialization{Initiate $^{k}d_{o,j}(t)$, $^{k}\alpha_{o,j}(t)$, $^{k}\beta_{o,j}(t)$  }
\While{$k \leq maxiter$}{

%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.07cm}
\hspace{-0.15cm}Compute \hspace{-0.05cm}\colorbox{my_orange}{\hspace{-0.1cm}$^{k}\hspace{-0.05cm}c_{\hspace{-0.031cm}\alpha\hspace{-0.021cm},\hspace{-0.031cm}j}\hspace{-0.021cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}=\hspace{-0.05cm}\cos{^{k}\alpha_{\hspace{-0.031cm}o\hspace{-0.031cm},\hspace{-0.05cm}j}\hspace{-0.051cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}\hspace{-0.041cm}\hspace{-0.05cm}$},\colorbox{my_yellow}{\hspace{-0.1cm}$
^{k}s_{\hspace{-0.04cm}\alpha\hspace{-0.021cm},\hspace{-0.031cm}j}\hspace{-0.07cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}=\hspace{-0.1cm}\sin{^{k}\hspace{-0.05cm}\alpha_{\hspace{-0.03cm}o\hspace{-0.02cm},\hspace{-0.035cm}j}\hspace{-0.02cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}\hspace{-0.05cm},\hspace{-0.2cm}$}
   \colorbox{my_purple}{$\hspace{-0.12cm}^{k}c_{\beta,\hspace{-0.02cm}j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}=\hspace{-0.1cm}\cos{\hspace{-0.02cm}^{k}\hspace{-0.035cm}\beta_{\hspace{-0.03cm}o\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.06cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}$},\colorbox{my_grey}{\hspace{-0.1cm}$
^{k}\hspace{-0.021cm}s_{\beta\hspace{-0.021cm},\hspace{-0.021cm}j}\hspace{-0.011cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}=\hspace{-0.1cm}\sin{^{k}\hspace{-0.02cm}\beta_{o,\hspace{-0.01cm}j}\hspace{-0.02cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}\hspace{-0.19cm}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Compute $^{k+1}x(t)$,$^{k+1}y(t)$ and $^{k+1}z(t)$ 
\vspace{-0.6cm}
\begin{subequations}
    \begin{align}
\hspace{-0.3cm}^{k+1}x(\hspace{-0.02cm}t\hspace{-0.02cm}) = \arg \min_{x(t)}f_{x}\hspace{-0.07cm}+\hspace{-0.07cm}I_{x}\hspace{-0.07cm}+\hspace{-0.07cm}\sum_{t=0}^{t=n_{p}}\sum_{j=1}^{j=n_{o}}\Big(\hspace{0.05cm}^{k}\lambda_{x,j}(t)
 (\colorbox{my_green}{$\hspace{-0.1cm}x(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}x_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})
 $} \nonumber \\ \colorbox{my_green}{$-
  a^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}c_{\alpha,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.04cm}$\hspace{-0.1cm}})\hspace{-0.1cm}+\hspace{-0.1cm} \frac{\rho_{o}}{2}(\colorbox{my_green}{$\hspace{-0.1cm}x(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}x_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.05cm}^{k}c_{\alpha,j}(\hspace{-0.02cm}t\hspace{-0.03cm}) \hspace{0.03cm}^{k}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}})^{2}\hspace{-0.1cm}\Big) \label{com_x}\\
   ^{k+1}y(t)
   \hspace{-0.1cm} =\hspace{-0.1cm}\arg \min_{y(\hspace{-0.03cm}t\hspace{-0.03cm})}f_{y}\hspace{-0.07cm}+\hspace{-0.07cm}I_{y}\hspace{-0.1cm}+\sum_{t=0}^{t=n_{p}}\sum_{j=1}^{j=n_{o}}\Big(\hspace{0.05cm}^{k}\lambda_{y,j}(t)(\colorbox{my_pink}{$y(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}y_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm}) 
    \hspace{-0.1cm}$}\nonumber \\\colorbox{my_pink}{$\hspace{-0.15cm}
-a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm}) \hspace{0.03cm}^{k}s_{\alpha,j}(\hspace{-0.03cm}t\hspace{-0.03cm}) \hspace{0.03cm}^{k}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}$}\hspace{-0.03cm}) 
\hspace{-0.1cm}+\hspace{-0.1cm}\frac{\rho_{o}}{2}(\colorbox{my_pink}{$\hspace{-0.1cm}y(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.07cm}-\hspace{-0.07cm}y_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})
\hspace{-0.07cm}-\hspace{-0.07cm}a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}s_{\alpha,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}$}\hspace{-0.03cm})^2\hspace{-0.03cm}\Big) \label{com_y}\\
^{k+1}z(t)\hspace{-0.07cm}=\hspace{-0.07cm}\arg \min_{z(t)}f_{z}+I_{z}
\hspace{-0.07cm}+\hspace{-0.2cm}\sum_{t=0}^{t=n_{p}}\sum_{j=1}^{j=n_{o}}\hspace{-0.1cm}\Big(\hspace{0.05cm}^{k}\lambda_{z,j}(\hspace{-0.03cm}t\hspace{-0.03cm})(\colorbox{my_blue}{$\hspace{-0.1cm}z(\hspace{-0.03cm}t\hspace{-0.03cm})-z_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm}) $} \nonumber \\
\colorbox{my_blue}{$-b\hspace{0.05cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.05cm}^{k}c_{\beta,j}(t)$} ) 
+ \frac{\rho_{o}}{2}(\colorbox{my_blue}{$z(t)-z_{o,j}(t) -b\hspace{0.05cm}^{k}d_{o,j}\hspace{0.05cm}^{k}c_{\beta,j}(t)$} )^{2}\Big) \label{com_z}
\end{align}
\end{subequations}
\vspace{-0.45cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}c_{\alpha,j}(t)$,$\hspace{0.05cm}^{k+1}s_{\alpha,j}(t)$
%%%%%%%%%%%%%%%%
\vspace{-0.4cm}
\begin{subequations}
    \begin{align}
\hspace{-0.65cm}^{k+1}c_{\alpha,j}\hspace{-0.06cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}=\hspace{-0.1cm}\arg\hspace{-0.13cm}\min_{c_{\alpha,j}\hspace{-0.07cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}\hspace{-0.05cm}\sum_{t}\hspace{-0.08cm}\sum_{j}\hspace{-0.10cm}\Big(\hspace{-0.07cm}\frac{\rho}{2}\hspace{-0.03cm}(\hspace{-0.01cm}\colorbox{my_orange}{$\hspace{-0.15cm}c_{\alpha,j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}- \hspace{-0.07cm}\cos{^{k}\alpha_{o,j}\hspace{-0.05cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{c_{\alpha,j}}\hspace{-0.05cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.12cm}+\hspace{-0.1cm} \lambda_{x,j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})(\colorbox{my_green}{$\hspace{-0.15cm}^{k+1}x(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}-\hspace{-0.1cm}\hspace{-0.05cm}x_{o,j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.07cm} $} \nonumber \\
\colorbox{my_green}{$\hspace{-0.2cm}-\hspace{-0.07cm}
  a^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.03cm}c_{\alpha,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}s_{\beta,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.04cm}$\hspace{-0.1cm}})\hspace{-0.1cm}+\hspace{-0.1cm} \frac{\rho_{o}}{2}\hspace{-0.05cm}(\colorbox{my_green}{$\hspace{-0.1cm}^{k+1}x(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}x_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}c_{\alpha,j}(\hspace{-0.02cm}t\hspace{-0.03cm}) \hspace{0.03cm}^{k}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}})^{2}\hspace{-0.1cm}\Big) \label{com_c_alpha}\\
\hspace{-0.75cm}^{k+1}s_{\alpha\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}=\hspace{-0.1cm}\arg\hspace{-0.13cm}\min_{s_{\alpha,j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}\hspace{-0.05cm}\sum_{t}\hspace{-0.08cm}\sum_{j}\hspace{-0.10cm}\Big(\hspace{-0.07cm}\frac{\rho}{2}\hspace{-0.03cm}(\hspace{-0.01cm}\colorbox{my_yellow}{$\hspace{-0.15cm}s_{\alpha\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}- \hspace{-0.07cm}\sin{^{k}\alpha_{o,j}\hspace{-0.05cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{s_{\alpha\hspace{-0.04cm},\hspace{-0.04cm}j}}\hspace{-0.05cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.12cm}+\hspace{-0.1cm}^{k}\lambda_{y\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})(\colorbox{my_pink}{$\hspace{-0.15cm}^{k+1}y(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}-\hspace{-0.06cm}y_{o\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.07cm} $} \nonumber \\
\hspace{-0.2cm}
\colorbox{my_pink}{$\hspace{-0.2cm}-\hspace{-0.07cm}
  a^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.03cm}s_{\alpha,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}^{k}s_{\beta,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.04cm}$\hspace{-0.1cm}})\hspace{-0.1cm}+\hspace{-0.1cm} \frac{\rho_{o}}{2}\hspace{-0.05cm}(\colorbox{my_pink}{$\hspace{-0.1cm}^{k+1}y(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}y_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}s_{\alpha,j}(\hspace{-0.02cm}t\hspace{-0.03cm}) \hspace{0.03cm}^{k}s_{\beta,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}$\hspace{-0.1cm}})^{2}\hspace{-0.1cm}\Big) \label{com_s_alpha}
\end{align}
\end{subequations}
\vspace{-0.55cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}\alpha_{o,j}(t)$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}
\begin{align}
    \hspace{0.05cm}^{k+1}\alpha_{o,j}(t) = \arg \min_{\alpha_{o,j}(t)}\sum_{t}\hspace{-0.08cm}\sum_{j}(\alpha_{o,j}(t) - \arctan 2\frac{^{k+1}s_{\alpha,j}(t)}{^{k+1}c_{\alpha,j}(t)})^2 \label{com_alpha}
\end{align}
\vspace{-0.6cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}c_{\beta,j}(t)$,$\hspace{0.05cm}^{k+1}s_{\beta,j}(t)$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.4cm}
\begin{subequations}
    \begin{align}
\hspace{-1cm}^{k+1}c_{\beta,j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}=\hspace{-0.1cm}\arg\hspace{-0.13cm}\min_{c_{\beta,j}\hspace{-0.05cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}\hspace{-0.05cm}\sum_{t}\hspace{-0.08cm}\sum_{j}\hspace{-0.10cm}\Big(\hspace{-0.07cm}\frac{\rho}{2}\hspace{-0.03cm}(\hspace{-0.01cm}\colorbox{my_purple}{$\hspace{-0.15cm}c_{\beta,j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}- \hspace{-0.07cm}\cos{^{k}\beta_{o,j}\hspace{-0.05cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{c_{\beta,j}}\hspace{-0.05cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.12cm}+\hspace{-0.1cm}^{k}\lambda_{z\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})(\colorbox{my_blue}{$\hspace{-0.15cm}^{k+1}z(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}-\hspace{-0.1cm}\hspace{-0.05cm}z_{o,j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.07cm} $} \nonumber \\
\colorbox{my_blue}{$\hspace{-0.2cm}-\hspace{-0.07cm}
  b^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.03cm}c_{\beta,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}})\hspace{-0.1cm}+\hspace{-0.1cm} \frac{\rho_{o}}{2}\hspace{-0.05cm}(\colorbox{my_blue}{$\hspace{-0.1cm}^{k+1}z(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}z_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}b\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}c_{\beta,j}(\hspace{-0.02cm}t\hspace{-0.03cm})$\hspace{-0.1cm}})^{2}\hspace{-0.1cm}\Big) \label{com_c_beta}\\
  \hspace{-0.85cm}
\hspace{-0.65cm}^{k+1}s_{\beta,j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}=\hspace{-0.1cm}\arg\hspace{-0.13cm}\min_{s_{\beta,j}\hspace{-0.07cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}\hspace{-0.05cm}\sum_{t}\hspace{-0.08cm}\sum_{j}\hspace{-0.10cm}\Big(\hspace{-0.07cm}\frac{\rho}{2}\hspace{-0.03cm}(\hspace{-0.01cm}\colorbox{my_grey}{$\hspace{-0.15cm}s_{\beta,j}\hspace{-0.04cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}- \hspace{-0.07cm}\sin{^{k}\beta_{o,j}\hspace{-0.05cm}(\hspace{-0.04cm}t\hspace{-0.04cm})}$}\hspace{-0.2cm}+\hspace{-0.1cm}\frac{\lambda_{s_{\beta,j}}\hspace{-0.05cm}(\hspace{-0.03cm}t\hspace{-0.03cm})}{\rho}\hspace{-0.07cm})^{2}\hspace{-0.12cm}+\hspace{-0.1cm}^{k}\lambda_{y\hspace{-0.02cm},\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.02cm}(\colorbox{my_pink}{$\hspace{-0.15cm}^{k+1}y(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.1cm}-\hspace{-0.07cm}y_{o,\hspace{-0.02cm}j}\hspace{-0.03cm}(\hspace{-0.04cm}t\hspace{-0.04cm})\hspace{-0.07cm} $} \nonumber \\
\hspace{-0.2cm}\colorbox{my_pink}{$\hspace{-0.2cm}-\hspace{-0.07cm}
  a^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.03cm}^{k+1}s_{\alpha,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}s_{\beta,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.04cm}$\hspace{-0.1cm}})\hspace{-0.1cm}+\hspace{-0.1cm} \frac{\rho_{o}}{2}\hspace{-0.05cm}(\colorbox{my_pink}{$\hspace{-0.1cm}^{k+1}y(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}y_{o,j}\hspace{-0.03cm}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k}d_{o,j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.05cm}^{k+1}s_{\alpha,j}(\hspace{-0.02cm}t\hspace{-0.03cm}) \hspace{0.03cm}s_{\beta,j}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}})^{2}\hspace{-0.1cm}\Big) \label{com_s_beta}
\end{align}
\end{subequations}
\vspace{-0.6cm}

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}\beta_{o,j}(t)$
%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}
\begin{align}
    \hspace{0.05cm}^{k+1}\beta_{o,j}(t) = \arg \min_{\beta_{o,j}(t)}\sum_{t}\hspace{-0.08cm}\sum_{j}(\beta_{o,j}(t) - \arctan 2\frac{^{k+1}s_{\beta,j}(t)}{^{k+1}c_{\beta,j}(t)}^2
    \label{com_beta}
\end{align}
\vspace{-0.5cm}
%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}d_{o,j}(t)$ through \eqref{d_max} using updated $(x(t),y(t),z(t))$

\hspace{-0.15cm}Update $\lambda_{x,j}(t), \lambda_{y,j}(t), \lambda_{z,j}, \lambda_{c_{\alpha,j}}(t), \lambda_{s_{\alpha,j}}(t),\lambda_{c_{\beta,j}}(t)$ and $\lambda_{s_{\beta,j}}(t)$ at $k+1$
}
\end{algorithm}
\normalsize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation and Benchmarking}
\noindent \textbf{Implementation Details:}
We implemented Algorithm \ref{alg_1} in Python, utilizing the Numpy libraries, and incorporated CVXOPT \cite{vandenberghe2010cvxopt} to solve the \gls{qp}s within each iteration of the \gls{ccp}. The execution of all benchmarks took place on a laptop with a 2.60 GHz processor and 32 GB RAM. To enhance the computational efficiency of the \gls{ccp}, we adopted the heuristic proposed in \cite{boyd2004convex}, which involves considering only $6-8\%$ of the total number of collision avoidance constraints at each iteration. It is crucial to note that this heuristic's effectiveness is highly dependent on problem parameters, and determining the specific percentage involved multiple trial and error iterations. The following cost function was employed in our analysis

\vspace{-0.4cm}
\small
\begin{align}
f_{x} = \sum_{t=0}^{n_{p}} w_{1}\ddot{x}(t)^2+w_{2}(x(t)-x_{des}(t))^{2},
\label{cost_sim}
\end{align}
\normalsize

\noindent where the cost function comprises two terms: the first term ensures smoothness, while the second term relates to the tracking of the desired trajectory $x_{des}(t)$. The weights $w_{1}$ and $w_{2}$ enable a trade-off between different components of the cost function. Similarly, cost functions for the y and z axes, denoted as $f_{y}$ and $f_{z}$, can be formulated in the same way. We employ three metrics to evaluate our proposed method, each defined as: 
\begin{itemize}
     \item Optimal cost: we compute two costs including smoothness cost, $\small{\sum_{t=0}^{n_{p}}(\ddot{x}(t)^2\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{y}(t)^2\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{z}(t)^2)}$, and tracking cost $\small{\sum_{t=0}^{n_{p}}((x(t)-x_{des}(t))^{2}+(y(t)-y_{des}(t))^{2}+(z(t)-z_{des}(t))^{2})}$. 
    \item Computation time: How long does it take for our proposed optimizer to find a collision-free trajectory?
    \item scalability: Computation time changes by increasing the number of obstacles and for a fixed number of iterations. 
\end{itemize}
\noindent \textbf{Benchmarks and Qualitative Results:}
We designed three benchmarks, including scenarios with 2D static obstacles (Figs. \ref{traj_1_static} and \ref{traj_2_static}, for a narrow corridor-like scene and an environment with randomly placed obstacles), 2D dynamic obstacles (Figs. \ref{traj_1_dyn} and \ref{traj_2_dyn}) and 3D collision avoidance (Fig. \ref{fig_3d}). For each benchmark, we considered $n_{o}=10$ obstacles and generated 15 different problem instances by varying the initial position and velocity for a given final state. The planning time interval ranged from $15s$ to $60s$, depending on the start and goal positions, and was discretized into $n_{p}=1000$ steps. Thus, the total number of collision avoidance constraints across all benchmarks was $10,000$. 

\begin{figure*}[!h]
  \centering  
  \vspace{-0.3cm}
\subfigure[]{
    \includegraphics[width= 6.2cm, height=4.3cm] {figures/path_corridor.png}
    \label{traj_1_static}
   }\hspace{-0.7cm}
\subfigure[]{
    \includegraphics[width= 6.2cm, height=4.3cm] {figures/path_random.png}
    \label{traj_2_static}
   }                 
\caption[Static benchmark of Alg. \ref{alg_1}]{\small{(a) and (b): Static obstacle benchmarks depicting a narrow corridor-like scene and an environment with randomly placed obstacles. The paths obtained with our proposed optimizer are marked in blue, while the \gls{ccp} approach paths are marked in cyan. The desired trajectory to be tracked is indicated in magenta.}}
\end{figure*}

\begin{figure*}[!h]
  \centering  
  \vspace{-0.3cm}
  \subfigure[]{
    \includegraphics[width= 6.2cm, height=4.3cm] {figures/traj_dyn_1.png}
    \label{traj_1_dyn}
   }\hspace{-0.7cm}
\subfigure[]{
    \includegraphics[width= 6.2cm, height=4.3cm] {figures/traj_dyn_2.png}
    \label{traj_2_dyn}
   }
\caption[Dynamic benchmark of Alg. \ref{alg_1}]{\small{(a) and (b): Dynamic obstacle benchmarks depicting environments where obstacles are moving in opposite and perpendicular directions relative to the agent. The paths obtained with our proposed optimizer are marked in blue, while the \gls{ccp} approach paths are marked in cyan. The desired trajectory to be tracked is indicated in magenta.}}
\end{figure*}

\begin{figure}[!h]
  \centering  
  \vspace{-0.3cm}
    \includegraphics[scale=0.25] {figures/path1_3d.png}
\caption[3D benchmark of Alg. \ref{alg_1}]{\small{3D obstacle benchmark. The paths obtained with our proposed optimizer are marked in blue, while the \gls{ccp} approach paths are marked in cyan. The desired trajectory to be tracked is indicated in magenta.}}
 \label{fig_3d}
\end{figure}

\noindent \textbf{Convergence Validation:}
A key validation for our optimizer, Algorithm \ref{alg_1} is the decrease in different residuals over iteration. Fig. \ref{fig_3d} shows this trend for equality constraints \eqref{collision_proposed_1} and \eqref{new_var_1}. As can be seen, on average, around 100 iterations suffice to achieve a residual on the order of $10^{-3}$.

\begin{figure}[!h]
  \centering  
  \vspace{-0.3cm}
    \includegraphics[scale=0.5] {figures/res_plots.png}
\caption[Convergence validation]{\small{The general trend of residuals of equality constraints \eqref{collision_proposed_1} and consensus term \eqref{new_var_1} with iterations for 2d static and dynamic obstacles}}
 \label{fig_3d}
\end{figure}

\noindent \textbf{Quantitative results:}
\subsubsection{Optimal Cost Analysis}
Fig. \ref{cost_com} presents the statistical analysis of the optimal costs including smoothness and tracking across various benchmarks. A diverse trend is observed in the 2D benchmarks. However, upon averaging the costs across all instances, both the proposed optimizer and \gls{ccp} demonstrate very similar smoothness and tracking costs, with \gls{ccp} showing a marginal superiority. Notably, for the 3D obstacle benchmark, Fig. \ref{optimal_cost}, the proposed optimizer consistently achieves solutions with significantly lower smoothness costs.

\begin{figure}[!h]
  \centering  
  \vspace{-0.3cm}
    \includegraphics[scale=0.4] {figures/optimal_cost.png}
    \vspace{-0.5cm}
\caption[The optimal cost comparisons between Alg. \ref{alg_1} and CCP]{\small{The optimal cost statistics for static 2D obstacles (a)-(b), dynamic 2D obstacles (d)-(e) and 3D environments (f).} } \label{optimal_cost}
\end{figure}

\subsubsection{Computation Time Comparison}
We now introduce one of the key results of this paper. Figs. \ref{cost_com} presents the statistical analysis of computation times across different benchmarks. Notably, for the 2D static obstacle benchmark (see Fig. \ref{cost_com}(a)), the proposed optimizer achieves an average speed-up of up to two orders of magnitude compared to \gls{ccp}. Furthermore, the computation times for \gls{ccp} exhibit high variance, suggesting that the worst-case difference in computation time could be even more pronounced. The proposed optimizer demonstrates a similar speed-up in both the dynamic obstacle (see Fig. \ref{cost_com}(b)) and 3D benchmarks (see Fig. \ref{cost_com}(c)).

\begin{figure}[!h]
 \centering  
  \vspace{-0.3cm}
    \includegraphics[scale=0.4] {figures/com_time_alg_1.png}
    \vspace{-0.5cm}
\caption[Computation time comparison between Alg. 1 and \ref{alg_1}]{\small{The computation time comparison for static 2D obstacles (a), dynamic 2D obstacles (b) and 3D environments (c).}} \label{cost_com}
\end{figure}

\subsubsection{Computation Time Scaling}
Fig. \ref{comptime_scaling} reveals the second important result in this paper. It illustrates how computation time varies with an increase in the number of collision avoidance constraints. \gls{ccp} exhibits quadratic scaling, consistent with a similar observation presented in \cite{augugliaro2012generation} (see Fig. 3 in \cite{augugliaro2012generation}). In contrast, the proposed optimizer displays sub-linear growth in computation time. For instance, doubling the number of collision avoidance constraints only increases the computation time by a factor of 1.4. This favorable characteristic stems from two main reasons. Firstly, the computation time required for solving \eqref{step_x_2d_simplify} depends on our chosen parameterization of $x_{t}$ or, in other words, the dimension of $\textbf{c}_{x}$ which is not related to the number of obstacles. While the computation of matrices on the left-hand side of \eqref{step_x_2d_simplify} does depend on the number of obstacles, numerical libraries like Numpy efficiently leverage multi-threading for these operations. Secondly, since the remainder of our algorithm has symbolic solutions, its evaluation can be easily vectorized to take advantage of parallel computation. It is worth noting that  \gls{ccp} and the proposed optimizer may require different numbers of iterations to solve a given problem. Nevertheless, this result underscores a significant computational distinction between the two approaches. Moreover, as demonstrated earlier, the proposed optimizer outperforms \gls{ccp} in the considered benchmarks.

\subsection{Interrelation:}

This work serves as the foundational cornerstone for all subsequent research presented in this body of work. The conceptualization and modeling of collision avoidance constraints,  as well as additional constraints introduced in subsequent papers, draw inspiration from the intuition developed in this paper. Furthermore, the algorithms presented in our subsequent works extensively leverage the principles of the \gls{am} method, building upon the concepts and analyses outlined in this foundational work.  Key methodologies such as parametrized trajectory optimization and the augmented Lagrangian method, outlined in this foundational work, form an integral part of the analytical framework adopted in subsequent studies.


\section{Paper II}

\subsection{Context:}
 
This paper introduces an innovative trajectory optimization algorithm specifically designed for mobile robots navigating in diverse, dynamic environments, such as factories, malls, and hospitals. The genesis of our current work emerges from our dedicated efforts to develop a fleet of autonomous delivery robots tailored for hospital premises. In these dynamic settings, the arrangement of static obstacles may undergo significant changes over time, further complicated by the presence of dynamic obstacles. The limitations of relying on global motion plans derived from pre-existing maps become apparent in such dynamic scenarios. Thus, there is an increasing demand for algorithms capable of real-time, on-the-fly planning, especially over extended time horizons. 

Existing methods like \gls{ccp}, \gls{gd} and \gls{sqp}, have addressed the collision avoidance issue, but they are susceptible to getting trapped in local optima, particularly if their initial guess is poor (see Fig. \ref{batch_inital}(a)). Furthermore, the challenge of achieving a good initialization becomes notably demanding in cluttered and dynamic environments.

One potential approach to leverage this challenge is to provide multiple initial guesses for the trajectory optimization problem, solve them concurrently across multiple processors, and subsequently select the optimal solution (see Fig. \ref{batch_inital}(b)). However, the practical implementation of this technique is not straightforward. For instance, commonly used off-the-shelf optimizers like \gls{sqp} are designed to operate on \gls{cpu} threads, which are typically constrained by a limited number of cores, thereby limiting the number of initial guesses. In contrast, \gls{gpu}s are available in abundant quantities, often with thousands of cores, but adapting most optimizers, including \gls{sqp}, to effectively leverage \gls{gpu}s remains an unresolved issue.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.46]{figures/initialization.png}
    \vspace{-0.5cm}
    \caption[Naive initialization vs. batch initialization]{\small{(a): Naive initialization (e.g., straight blue line) may lead the trajectory optimizer to unsafe local minima. Our batch setting allows us to run hundreds of different instances of the problem in real-time, obtained by different initializations of the problem. \textcolor{black}{In (b)}, the blue trajectories represent initialization samples drawn from a Gaussian distribution \cite{kalakrishnan2011stomp}. After a few iterations, our batch optimizer returns a distribution of locally-optimal trajectories (green) residing in different homotopies (best cost trajectory: red)}}
    \label{batch_inital}
\end{figure}

This paper bridges the gap by introducing a batchable and \gls{gpu}-accelerated trajectory optimizer, addressing the challenge of local minima in the context of autonomous navigation for a fleet of robots.


\subsection{Contribution:}

Our primary contribution lies in overcoming the challenge of local minima by introducing a sophisticated, batchable, and \gls{gpu}-accelerated trajectory optimizer tailored for autonomous navigation. This novel batch optimizer demonstrates the ability to concurrently process several hundred instances of the problem in real-time. Specifically, our approach involves solving numerous instances of \gls{qp} problems in parallel, revealing that these \gls{qp} problems can be effectively reduced to computing large matrix-vector products. Leveraging an Alternating Minimization approach, we transform a complex trajectory optimization problem into more manageable sub-problems. Notably, our batch optimizer exhibits linear scalability concerning both batch sizes and collision avoidance constraints.

Particularly, we focus on robots with rectangular footprints and represent them as a composition of overlapping circles (see Fig. \ref{multi_circle}). This unique approach harnesses the advantages of enhanced maneuverability, particularly in confined spaces, thanks to the integration of rotational motions.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.24]{figures/Fig_2_multicircle.png}
    \caption[Modelling a robot with a rectangular footprint]{\small{(a): Robots with rectangular footprints can be modeled in two ways: a combination of circles (utilized in this work) and a single circle \cite{schwarting2017parallel}. Using a combination of overlapping circles, as depicted, enables the incorporation of rotational motions, facilitating better maneuverability in confined spaces. In contrast, the circular footprints may be overly conservative, potentially compelling the robot to take larger detours.
    (b) A rectangular footprint with center $O(t) = (x_{i}(t), y_{i}(t))$ and heading angle $\psi_{i}(t)$ is represented through combinations of four circles.}}
    \label{multi_circle}
    \end{figure}

Our work advances the \gls{sota} in several key aspects. Firstly, the parallel initialization naturally identifies a range of locally optimal trajectories within various homotopies. Secondly, we enhance navigation quality, including success rates and tracking performance, compared to the baseline approach, which relies on computing a single locally optimal trajectory at each control loop. Lastly, we demonstrate that when initialized with trajectory samples from a Gaussian distribution, our batch optimizer surpasses the performance of the \gls{sota} \gls{cem} in terms of solution quality.

\subsection{Main Results}\label{main_results_2}

In this section, we elucidate our innovative approach to designing a batchable \gls{gpu}-accelerated trajectory optimizer. We delve into the methodology employed to craft this optimizer, highlighting the key aspects that contribute to its efficiency and applicability in handling multiple instances of trajectory optimization concurrently. We begin by defining the trajectory optimization problem. So, we are interested in solving the following optimization problem.


\small
\begin{subequations}
\begin{align}
   \hspace{-0.17cm}\min_{x_{i}(t), y_{i}(t), \psi_{i}(t)}  \sum_{t} \hspace{-0.12cm} \Big(\ddot{x}_{i}^2(t)\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{y}_{i}^2(t) \hspace{-0.1cm}+ \hspace{-0.1cm}\ddot{\psi}_{i}^2(t) \hspace{-0.1cm} + \hspace{-0.1cm}(x_{i}(t) \hspace{-0.1cm}-\hspace{-0.1cm}x_{des}(t))^2
   \hspace{-0.1cm}+\hspace{-0.1cm}
   (y_{i}(t)\hspace{-0.1cm}-\hspace{-0.1cm}y_{des}(t))^2\Big),  \label{acc_cost}\\ 
   (x_{i}(t_{0}), y_{i}(t_{0}), x_{i}(t_{f}), y_{i}(t_{f})) = \textbf{b},\label{eq_multiagent_1}\\
   (\psi_{i}(t_{0}), \psi_{i}(t_{f})) = \textbf{b}_{\psi},\label{eq1_multiagent_1}\\
    \dot{x}_{i}^{2}(t) + \dot{y}_{i}^{2}(t)  \leq v^{2}_{max}, ~~~
    \ddot{x}_{i}^{2}(t) + \ddot{y}_{i}^{2}(t) \leq a^{2}_{max}, \label{acc_constraint}\\
   \hspace{-0.21cm}
    -\frac{\hspace{-0.07cm}(x_{i}(t)\hspace{-0.07cm}+\hspace{-0.07cm}r_{m}\hspace{-0.04cm}\cos{\psi_{i}(t)}\hspace{-0.095cm}-
 \hspace{-0.095cm}x_{o,j}(t)\hspace{-0.05cm})^{2}}{a^2}\hspace{-0.062cm} - \hspace{-0.062cm}
 \frac{\hspace{-0.072cm}(y_{i}(t) \hspace{-0.075cm}+\hspace{-0.075cm}r_{m}\sin{\psi_{i}\hspace{-0.04cm}(t)}
 \hspace{-0.075cm}-\hspace{-0.065cm}y_{o,j}(t)\hspace{-0.06cm})^{2}}{b^2}
  + 1\leq 0, \label{coll_multiagent}
\end{align}
\end{subequations}
\normalsize

\noindent Where the objective of the cost function \eqref{acc_cost} is to minimize the sum of squared linear and angular accelerations, as well as the tracking error from a desired position trajectory $(x_{\text{des}}(t), y_{\text{des}}(t))$ at different time instants. Here, $\psi_{i}(t)$ represents the heading angle. The vectors $\textbf{b}$ and $\textbf{b}_{\psi}$ in  \eqref{eq_multiagent_1} and \eqref{eq1_multiagent_1} represent the initial and final values of boundary conditions on linear and angular positions and their derivatives. We assume $v_{\text{max}}$ and $a_{\text{max}}$ as the maximum velocity and acceleration, inequality \eqref{acc_constraint} sets bounds on the total velocity and acceleration. Inequality \eqref{coll_multiagent} introduces collision avoidance constraints. The obstacle locations are defined by $(x_{o,j}(t), y_{o,j}(t))$, assumed to be axis-aligned ellipses with dimensions $(a, b)$. The robot's rectangular footprint is approximated by a collection of $n_{c}$ overlapping circles \cite{schwarting2017parallel}, \cite{singh2020bi}, where each circle's coordinate in the local frame is defined as $(\pm r_{m}, 0)$. Thus, \eqref{coll_multiagent} ensures that the $m^{th}$ circle of the footprint does not overlap with the $j^{th}$ elliptical obstacle, as illustrated in Fig. \ref{multi_circle}(b).

Now, we explain the core concept that underpins our approach and how it is leveraged in our trajectory optimization problem.

\noindent\textbf{Main Idea:} Consider a set of equality-constrained \gls{qp}s characterized by a distinctive structure where only the vector $\overline{\textbf{q}}_{i}$ varies among the instances of the problem.

\small
\begin{align}
\min_{\boldsymbol{\xi}_{i}} \Big(\frac{1}{2}\boldsymbol{\xi}^{T}_{i}\overline{\textbf{Q}}\boldsymbol{\xi}_{i} + \overline{\textbf{q}}^{T}_{i}\boldsymbol{\xi}_{i}\Big), \qquad
 \text{st: } \overline{\textbf{A}} \boldsymbol{\xi}_{i} = \overline{\textbf{b}},~~~~ i\in[1,N_{b}] \label{over_1}
\end{align}
\normalsize

\noindent Based on our discussion in Section \ref{qp_definition}, the $i^{th}$ optimization problem \eqref{over_1} can be reduced to a set of linear equations as

\small
\begin{align}
    \begin{bmatrix}
        \overline{\textbf{Q}} & \overline{\textbf{A}}^{T} \\ 
        \overline{\textbf{A}} & \textbf{0}
    \end{bmatrix} \begin{bmatrix}
        \boldsymbol{\xi}_{i}\\ \boldsymbol{\nu}_{i}
    \end{bmatrix} = \begin{bmatrix}
        \overline{\textbf{q}}_{i} \\ \overline{\textbf{b}}
    \end{bmatrix} \label{over_2}
\end{align}
\normalsize

\noindent where $\boldsymbol{\nu}_{i}$ is dual optimization variable. Since the matrix in \eqref{over_2} is constant for different batch instances, and also all batches are independent of each other, we can compute solution across all the batches in one-shot as follows:

\small
\begin{align}
\begin{bmatrix} 
\begin{array}{@{}c|c|cc@{}}
\boldsymbol{\xi}_{1} &...& \boldsymbol{\xi}_{N_{b}} \\ \boldsymbol{\nu}_{1} &...& \boldsymbol{\nu}_{N_{b}}
\end{array}
\end{bmatrix} =
    \overbrace{(\begin{bmatrix}
        \overline{\textbf{Q}} & \overline{\textbf{A}}^{T} \\ 
        \overline{\textbf{A}} & \textbf{0}
    \end{bmatrix}^{-1}) }^{constant}
\begin{bmatrix}
\begin{array}{@{}c|c|cc@{}}
    \overline{\textbf{q}}_{1} & ... & \overline{\textbf{q}}_{N_{b}}  \\
    \overline{\textbf{b}} & ... & \overline{\textbf{b}}
    \end{array}\end{bmatrix},
    \label{over_3}
\end{align}
\normalsize

\noindent where $|$ implies that the columns are stacked horizontally. For more clarification, we visualize our main idea in Fig. \ref{qp_diagram}, providing a graphical representation of the concepts discussed. 

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.6]{figures/qp_diagram.png}
    \vspace{-0.3cm}
    \caption[Visualization of the Main Idea of Alg. \ref{alg_2}]{\small{Visualization of the Main Idea: Schematic representation illustrating the structure and relationships of a set of equality-constrained \gls{qp}s. The diagram demonstrates how varying vectors among instances, denoted as $\overline{\textbf{q}}_{i}$, undergo a reduction process, revealing insights into computational simplifications. Each green box represents an individual \gls{qp} instance. Notably, the matrix inside the blue box remains constant across all \gls{qp} instances, enabling a one-time computation for subsequent matrix-vector productions.}}
    \label{qp_diagram}
    \end{figure}

Our primary \textbf{innovation} involves transforming the non-convex optimization problem \eqref{acc_cost}-\eqref{coll_multiagent} into a form where the most intensive computations have the same structure as (\ref{over_1}). 

\noindent \textbf{Reformulated constraints:} To reach this aim, we extend the polar representation of collision avoidance constraints discussed in Section \ref{main_result_1}, and reformulate \eqref{coll_multiagent} in the form $\textbf{f}_c = \textbf{0}$, where

\small
\begin{align}
\hspace{-0.2cm}\colorbox{my_green}{$ \textbf{f}_{c}(x_{i}(t),y_{i}(t),\psi_{i}(t))\hspace{-0.1cm}=\hspace{-0.1cm}
\hspace{-0.06cm}\left \{ \hspace{-0.23cm}\begin{array}{lcr}
x_{i}(t) \hspace{-0.04cm}+ \hspace{-0.05cm}r_{m} \cos{\psi_{i}}(t)\hspace{-0.07cm}-\hspace{-0.08cm}x_{o,j}(t) \hspace{-0.07cm}-ad_{mj,i}(t)\cos{\alpha_{mj,i}}(t) \\
y_{i}(t)\hspace{-0.04cm} + \hspace{-0.05cm}r_{m} \sin{\psi_{i}}(t)\hspace{-0.07cm}-\hspace{-0.07cm}y_{o,j}(t) 
\hspace{-0.08cm}-bd_{mj,i}(t)\sin{\alpha_{mj,i}(t)}
\end{array} \hspace{-0.25cm} \right \}\hspace{-0.10cm}, $}\nonumber \\  d_{mj,i}(t)\hspace{-0.10cm} \geq \hspace{-0.07cm}1 
\label{collision_1} 
\end{align}
\normalsize

\noindent where $d_{mj,i}(t)$ and $\alpha_{mj,i}(t)$ are the line-of-sight distance and angle between the $m^{th}$ circle of the robot and $j^{th}$ obstacle. As can be seen, \eqref{collision_1} exhibits convexity within the space of $(x_{i}(t), y_{i}(t))$ and $ (\cos{\psi}_{i}(t), \sin{\psi}_{i}(t))$. It should be mentioned that this convex characteristic later becomes advantageous in leveraging the proposed optimization problem. 

Similarly, we reformulate the velocity and acceleration constraints in the form
$ \textbf{f}_{v} =\textbf{0} $ and $\textbf{f}_{a} = \textbf{0}$, where 

\vspace{-0.22cm}
\small
\begin{subequations} 
\begin{align}
 \colorbox{my_pink}{$ \textbf{f}_{v} =\left \{ \hspace{-0.20cm} \begin{array}{lcr}
 \dot{x}_{i}(t) - d_{v,i}(t)v_{max}\cos{\alpha_{v,i}(t)}  \\
 \dot{y}_{i}(t) - d_{v,i}(t)v_{max}\sin{\alpha_{v,i}(t)} 
\end{array} \hspace{-0.20cm} \right \} $}
,d_{v,i}(t) \leq 1 , ~  \forall t,i  \label{fv} \\
\colorbox{my_blue}{$ \textbf{f}_{a} = \left \{ \hspace{-0.20cm}\begin{array}{lcr}
\ddot{x}_{i}(t) - d_{a,i}(t)a_{max}\cos{\alpha_{a,i}(t)} \\
\ddot{y}_{i}(t) - d_{a,i}(t)a_{max}\sin{\alpha_{a,i}(t)}
\end{array} \hspace{-0.20cm} \right \}$},  d_{a,i}(t) \leq 1 , ~\forall t,i \label{fa}
\end{align}
\end{subequations}
 \normalsize

\noindent where $d_{v,i},d_{a,i},\alpha_{v,i}(t)$ and $\alpha_{a,i}(t)$ are variables based on polar representation. Similar to \eqref{collision_1}, \eqref{fv} and \eqref{fa} are also convex in the space of $(\sin{\alpha_{v,i}(t)},\cos{\alpha_{v,i}(t)})$, $d_{v,i}$, $(\sin{\alpha_{a,i}(t)},\cos{\alpha_{a,i}(t)})$ and $d_{a,i}$.

The insights gained from the convex features of \eqref{collision_1}-\eqref{fa} lead us to reformulate the trajectory optimization problem \eqref{acc_cost}-\eqref{coll_multiagent} as follows:

\vspace{-0.22cm}
\small
\begin{subequations}
\begin{align}
\hspace{-0.6cm}\min_{\scalebox{0.7}{$\begin{matrix} x_{i}(t), y_{i}(t), \psi_{i}(t),\\c_{\psi,i}(t),s_{\psi,i}(t),d_{v,i}(t),
 d_{a,i}(t), \\d_{mj,i}(t),\alpha_{v,i}(t),\alpha_{a,i}(t),\alpha_{mj,i}(t)    \end{matrix}$}}
\hspace{-0.9cm}\sum_{t}\hspace{-0.1cm}\Big(\ddot{x}^2_{i}(t)\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{y}^2_{i}(t) +\hspace{-0.1cm}\ddot{\psi}_{i}^2(t) \hspace{-0.1cm} + \hspace{-0.1cm}(x_{i}(t) \hspace{-0.1cm}-\hspace{-0.1cm}x_{des}(t))^2
   \hspace{-0.1cm}+\hspace{-0.1cm}
   (y_{i}(t)\hspace{-0.1cm}-\hspace{-0.1cm}y_{des}(t))^2\Big),   \label{acc_cost1}\\
 (x_{i}(t_{0}), y_{i}(t_{0}), x_{i}(t_{f}), y_{i}(t_{f})) = \textbf{b},\label{eq_multiagent}\\
   (\psi_{i}(t_{0}), \psi_{i}(t_{f})) = \textbf{b}_{\psi},\label{eq1_multiagent}\\
\colorbox{my_pink}{$ \textbf{f}_{v}(t) = \textbf{0}, $} \qquad d_{v,i}(t)  \leq 1,   \forall t,i \label{cond1}  \\
\colorbox{my_blue}{$ \textbf{f}_{a}(t) = \textbf{0}$},  \qquad d_{a,i}(t) \leq 1, \forall t,i \label{fa_fv1} \\
\colorbox{my_yellow}{$  c_{\psi,i}(t) = \cos{\psi_{i}(t)}$} \label{cos_ref}\\ 
 \colorbox{my_purple}{$ s_{\psi,i}(t) =  \sin{\psi_{i}(t)}$} \label{sin_ref}\\
 \colorbox{my_green}{$ 
\textbf{f}_{c} \hspace{-0.1cm}: \hspace{-0.1cm}\left \{ \begin{array}{lcr}\hspace{-0.2cm}
x_{i}(t) + r_{m} c_{\psi,i}(t)-x_{o,j}(t) -ad_{mj,i}(t)\cos{\alpha_{mj,i}}(t) =0\\
\hspace{-0.2cm}y_{i}(t) + r_{m} s_{\psi,i}(t)-y_{o,j}(t) 
-bd_{mj,i}(t)\sin{\alpha_{lj,i}(t)} =0
\end{array} \right \} $}\hspace{-0.2cm}\label{coll_con}% \right \} 
 \\ d_{mj,i}(t) \geq 1, \label{fc1}
\end{align}
\end{subequations}
\normalsize

\noindent where two new slack variables, $c_{\psi,i}(t)$ and $s_{\psi,i}(t)$ are simply the copy of $\cos{\psi_{i}(t)}$ and $\sin{\psi_{i}(t)}$. Our main trick is to treat $c_{\psi,i}(t)$ and $s_{\psi,i}(t)$
as independent variables and somehow ensure that when the optimization converges, they indeed resemble the cosine and sine of $\psi_{i}(t)$. 

The above optimization is defined in terms of time-dependent functions. To ensure smoothness in trajectories, we parameterize the optimization variables as

\small
\begin{align}
     \begin{bmatrix}\hspace{-0.05cm}
x_{i}(t_1)\\
\hspace{-0.05cm}x_{i}(t_2)\\
\vdots\\
\hspace{-0.05cm}x_{i}(t_p)
\end{bmatrix}\hspace{-0.2cm}= \hspace{-0.1cm}\textbf{P}\textbf{c}_{x,i}, \hspace{-0.1cm}
   \begin{bmatrix}
\hspace{-0.05cm}y_{i}(t_1)\\
\hspace{-0.05cm}y_{i}(t_2)\\
\vdots\\
\hspace{-0.05cm}y_{i}(t_p)
\end{bmatrix}\hspace{-0.2cm}= \hspace{-0.1cm}\textbf{P}\textbf{c}_{y,i}, \hspace{-0.1cm}
   \begin{bmatrix}
\hspace{-0.05cm}\psi_{i}(t_1)\\
\hspace{-0.05cm}\psi_{i}(t_2)\\
\vdots\\
\hspace{-0.05cm}\psi_{i}(t_p)
\end{bmatrix}\hspace{-0.2cm}= \hspace{-0.1cm}\textbf{P}\textbf{c}_{\psi,i},
\hspace{-0.2cm}
\begin{bmatrix}
\hspace{-0.05cm}c_{\psi,i}(t_1)\\
\hspace{-0.05cm}c_{\psi,i}(t_2)\\
\vdots\\
\hspace{-0.05cm}c_{\psi,i}(t_p)
\end{bmatrix}\hspace{-0.2cm}= \hspace{-0.1cm}\textbf{P}\textbf{c}_{c,i},
\hspace{-0.1cm}
\begin{bmatrix}
\hspace{-0.05cm}s_{\psi,i}(t_1)\\
\hspace{-0.05cm}s_{\psi,i}(t_2)\\
\vdots\\
\hspace{-0.05cm}s_{\psi,i}(t_p)
\end{bmatrix}\hspace{-0.1cm}= \hspace{-0.1cm}\textbf{P}\textbf{c}_{s,i},
\label{parametrization}
\end{align}
\normalsize

\noindent where $\bold{P}$ is a matrix created using polynomial basis functions that are dependent on time and $\textbf{c}_{x,i}, \textbf{c}_{y,i}, \textbf{c}_{\psi,i}, \textbf{c}_{c,i}$ and $\textbf{c}_{s,i}$ represent the coefficients of the polynomial.  The expression remains applicable for derivatives by utilizing  $\dot{\bold{P}}$ and $\ddot{\textbf{P}}$. 

Now, using \eqref{parametrization} and some simplifications, the problem \eqref{acc_cost1}-\eqref{fc1} can be formulated as 

\small
\begin{subequations}
\begin{align}
 \min_{\boldsymbol{\xi}_{i}, \boldsymbol{\alpha}_{i}, \textbf{d}_{i}, \boldsymbol{\xi}_{\psi,i}} \hspace{-0.1cm}\Big(\frac{1}{2}\boldsymbol{\xi}_{i}^T\textbf{Q}\boldsymbol{\xi}_{i}  + \textbf{q}^T\boldsymbol{\xi}_{i}+ \frac{1}{2}\boldsymbol{\xi}_{\psi,i}^{T}\ddot{\textbf{P}}^{T}\ddot{\textbf{P}}\boldsymbol{\xi}_{\psi,i} \Big)\label{reform_cost},  \\
  \textbf{A}\boldsymbol{\xi}_{i} = \textbf{b}, ~~~ \textbf{A}_{\psi}\boldsymbol{\xi}_{\psi,i} = \textbf{b}_{\psi},   \label{reform_eq}\\
  \textbf{F}\boldsymbol{\xi}_{i} = \textbf{g}_{i}(\boldsymbol{\alpha}_{i},\boldsymbol{\xi}_{\psi,i},\textbf{d}_{i} ) \label{reform_bound},\\
 \textbf{d}_{min}\leq \textbf{d}_{i} \leq \textbf{d}_{max}. \label{d_bound}
\end{align}
\end{subequations}
\normalsize

\noindent where, $\boldsymbol{\xi}_{i} =(\textbf{c}_{x,i}, \textbf{c}_{c,i}, \textbf{c}_{y,i}, \textbf{c}_{s,i}) $, $\boldsymbol{\xi}_{\psi,i}= \textbf{c}_{\psi,i}$, 
$\boldsymbol{\alpha}_{i} = (\boldsymbol{\alpha}_{mj,i}, \hspace{0.1cm} \boldsymbol{\alpha}_{v,i}, \hspace{0.1cm} \boldsymbol{\alpha}_{a,i})$ and $\textbf{d}_{i} = (\textbf{d}_{mj,i},\textbf{d}_{v,i},\textbf{d}_{a,i})$ are optimization variables to be obtained. The matrix $\textbf{A}$ is generated by stacking the first and last row of $\textbf{P}$ and their derivations corresponding to equality boundaries. Similarly, the matrix $\textbf{A}_{\psi}$ is generated by stacking the first and last row of $\textbf{P}$. The constant vectors, $\textbf{d}_{min}$ and $\textbf{d}_{max}$ are formed by stacking the lower $([1,0,0])$ and upper bounds $([\infty,1,1])$ of $\textbf{d}_{mj,i}, \textbf{d}_{v,i}, \textbf{d}_{a,i}$. The matrix and vector $\textbf{Q}$ and $\textbf{q}$ are used to convert the acceleration and tracking cost in \eqref{acc_cost1} into \gls{qp} problem and can be defined as

\small
\begin{align}
\textbf{Q} = \begin{bmatrix}
\ddot{\textbf{P}}^T\ddot{\textbf{P}}+\textbf{P}^{T}\textbf{P}&&&\\
& 0&&\\
&&\ddot{\textbf{P}}^T\ddot{\textbf{P}}+\textbf{P}^{T}\textbf{P}&\\
&&&0
\end{bmatrix} ~~~ \textbf{q} = \begin{bmatrix}
-\textbf{P}^T\textbf{x}_{des}\\
\textbf{0}\\
-\textbf{P}^T\textbf{y}_{des}\\
\textbf{0}\\
\end{bmatrix}
\label{Q_matrix}
\end{align}
\normalsize

\noindent where $\textbf{x}_{des}$ and $\textbf{y}_{des}$ are obtained by stacking $x_{des}(t)$ and $y_{des}(t)$ at different time instances. Also, the matrix $\textbf{F}$ and vector $\textbf{g}_{i}$  in \eqref{reform_bound} are obtained by rewriting constraints  \eqref{cond1} - \eqref{coll_con} in the following manner.

\small
\begin{align}
\overbrace{ \begin{bmatrix} 
\colorbox{my_pink}{$\begin{bmatrix}
\dot{\textbf{P}}  &  \textbf{0}  \\
\end{bmatrix} $}& \textbf{0}   \\
\colorbox{my_blue}{$
\begin{bmatrix}
\ddot{\textbf{P}}  &  \textbf{0}  \\
\end{bmatrix}$} & \textbf{0}    \\
  \colorbox{my_green}{$\textbf{A}_{o}$} & \textbf{0} \\
\colorbox{my_yellow}{$\begin{bmatrix} \textbf{0} & \textbf{P}
\end{bmatrix} $}& \textbf{0} \\
\textbf{0} & \colorbox{my_pink}{$ \begin{bmatrix}
\dot{\textbf{P}}  &  \textbf{0}  \\
\end{bmatrix} $} \\
\textbf{0} &  \colorbox{my_blue}{$\begin{bmatrix}
\ddot{\textbf{P}}  &  \textbf{0}  \\
\end{bmatrix} $}\\
\textbf{0} & \colorbox{my_green}{$\textbf{A}_{o}$} \\
\textbf{0} & \colorbox{my_purple}{$\begin{bmatrix} \textbf{0} & \textbf{P}
\end{bmatrix}$}
\end{bmatrix}}^{\textbf{F}}
\begin{bmatrix}   \textbf{c}_{x,i} \\
\textbf{c}_{c,i} \\ 
\textbf{c}_{x,i} \\
\textbf{c}_{s,i}
\end{bmatrix} =
\overbrace{\begin{bmatrix}
\colorbox{my_pink}{$\textbf{d}_{v,i}\cos(\boldsymbol{\alpha}_{v,i})$} \\
\colorbox{my_blue}{$\textbf{d}_{a,i}\cos(\boldsymbol{\alpha}_{a,i}) $}\\
\colorbox{my_green}{$\textbf{b}_{o_{1,i}}(\textbf{d}_{mj,i},\boldsymbol{\alpha}_{mj,i})$} \\
\colorbox{my_yellow}{$\cos{\boldsymbol{\psi}_{i}}$} \\
\colorbox{my_pink}{$\textbf{d}_{v,i}\sin(\boldsymbol{\alpha}_{v,i})$} \\
\colorbox{my_blue}{$\textbf{d}_{a,i}\sin(\boldsymbol{\alpha}_{a,i})$} \\
 \colorbox{my_green}{$\textbf{b}_{o_{2,i}}(\textbf{d}_{mj,i},\boldsymbol{\alpha}_{mj,i})$} \\
 \colorbox{my_purple}{$\sin{\boldsymbol{\psi}_{i}} $}
\end{bmatrix}}^{\textbf{g}_{i}}
\end{align}

\noindent where 

\small
\begin{align}
\textbf{b}_{o_{1,i}}=\colorbox{my_green}{$\begin{bmatrix}
\textbf{x}_{o,j} \\ \vdots  \\ \textbf{x}_{o,j} 
\end{bmatrix}
+ a \begin{bmatrix}
\textbf{d}_{1j,i} \hspace{0.1 cm}\cos{\boldsymbol{\alpha}_{1j,i}} \\
\vdots\\
\textbf{d}_{mj,i} \hspace{0.1 cm}\cos{\boldsymbol{\alpha}_{mj,l}}
\end{bmatrix}$} , 
\colorbox{my_green}{$\textbf{A}_{o}\hspace{-0.07cm} = \hspace{-0.07cm}\begin{bmatrix}
\textbf{P}  &  r_{1}\textbf{P}  \\
\vdots  & \vdots  \\
\textbf{P}  & r_{m}\textbf{P}\\
\end{bmatrix}$},
 \nonumber \\
\textbf{b}_{o_{2,l}} = \colorbox{my_green}{$\begin{bmatrix} 
\textbf{y}_{o,j} \\ \vdots  \\ \textbf{y}_{o,j} 
\end{bmatrix}
+ b \begin{bmatrix}
\textbf{d}_{1j,i}\sin{\boldsymbol{\alpha}_{1j,i}} \\
\vdots\\
\textbf{d}_{mj,i}\sin{\boldsymbol{\alpha}_{mj,i}}
\end{bmatrix}$}
\end{align}
\normalsize

\noindent and $\textbf{d}_{v,i}$, $\textbf{d}_{a,i}$, $\textbf{d}_{mj,i}$, are constructed by stacking $d_{v,i}(t)$, $d_{a,i}(t)$, and $d_{mj,i}(t)$ at different time instances. Similar derivation is used for generating $\textbf{x}_{o,j}, \textbf{y}_{o,j}$, $\boldsymbol{\alpha}_{v,i}$, $\boldsymbol{\alpha}_{a,i}$, $\boldsymbol{\alpha}_{mj,i}$ and $\boldsymbol{\psi}_{i}$ as well. 

To show how our proposed reformulation \eqref{reform_cost}-\eqref{d_bound} offers a computational advantage over \eqref{acc_cost}-\eqref{coll_multiagent}, an additional layer of simplification is necessary. So, using the augmented Lagrangian method, we relax the non-convex equality constraints \eqref{reform_bound} as $l_2$ penalties.

\small
\begin{align}
\min_{\boldsymbol{\xi}_{i}, \boldsymbol{\alpha}_{i}, \textbf{d}_{i}, \boldsymbol{\xi}_{\psi,i}} 
 \Big(\frac{1}{2}\boldsymbol{\xi}_{i}^T\textbf{Q}\boldsymbol{\xi}_{i}+\textbf{q}^T\boldsymbol{\xi}_{i}
 +\frac{1}{2}\boldsymbol{\xi}_{\psi,i}^T\ddot{\textbf{P}}^{T}\ddot{\textbf{P}}\boldsymbol{\xi}_{\psi,i} 
 - \langle\boldsymbol{\lambda}_{i}, \boldsymbol{\xi}_{i}\rangle 
  - \langle\boldsymbol{\lambda}_{\psi,i}, \boldsymbol{\xi}_{\psi,i}\rangle\nonumber \\
 +\frac{\rho}{2}\left\Vert \textbf{F} \boldsymbol{\xi}_{i}  
 -\textbf{g}(\boldsymbol{\xi}_{\psi,i},\boldsymbol{\alpha}_{i},\textbf{d}_{i} ) \right \Vert_2^2 \Big),
 \label{reform_formulation}
 \end{align}
\normalsize

\noindent where the vectors $\boldsymbol{\lambda}_{i}$ and $\boldsymbol{\lambda}_{\psi,i}$ are known as the Lagrange multipliers and are crucial for ensuring that the $l_2$ penalties of the equality constraints are driven to zero.

Upon careful examination of \eqref{reform_formulation}, it becomes apparent that:

\begin{itemize}
    \item For a given $\boldsymbol{\xi}_{\psi,i},\boldsymbol{\alpha}_{i}$, and $\textbf{d}_{i}$, \eqref{reform_formulation} is convex in the space of $\boldsymbol{\xi}_{i}$.
    \item  For a given $\boldsymbol{\xi}_{i},\boldsymbol{\alpha}_{i}$, and $\textbf{d}_{i}$, \eqref{reform_formulation} is non-convex in terms of $\boldsymbol{\xi}_{\psi,i}$, but it can be replaced with a convex surrogate from \cite{singh2020bi}.
    \item For a given $\boldsymbol{\xi}_{\psi,i},\boldsymbol{\xi}_{i}$, and $\textbf{d}_{i}$, \eqref{reform_formulation} is solvable in a closed-form for $\boldsymbol{\alpha}_{i}$.
    \item For a given $\boldsymbol{\xi}_{\psi,i},\boldsymbol{\alpha}_{i}$, and $\boldsymbol{\xi}_{i}$, \eqref{reform_formulation} is convex in the space of $\textbf{d}_{i}$ and has a closed-form solution.
\end{itemize}

Motivated by the above discussion, we adopt an \gls{am} approach for minimizing \eqref{reform_formulation}. At each step of AM, we only optimize over only one of the optimization variables and the rest of them are considered fixed. Algorithm \eqref{alg_2} explains the steps in solving \eqref{reform_formulation}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!h]
\DontPrintSemicolon
\SetAlgoLined
\SetNoFillComment
\scriptsize
\caption{\scriptsize Proposed Batch Optimizer Algorithm for the $i^{th}$ agent }\label{alg_2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\KwInitialization{Initiate $^{k}\textbf{d}_{i}$, $^{k}\boldsymbol{\alpha}_{i}$, $^{k}\boldsymbol{\xi}_{\psi,i}$ at $k=0$  }
\While{$k \leq maxiter$}{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Update ${^{k+1}}\boldsymbol{\xi}_{i}$ through 
\vspace{-0.3cm}
\begin{align}
\hspace{-0.5cm}{^{k+1}}\boldsymbol{\xi}_{i}\hspace{-0.1cm}=\hspace{-0.1cm}\min_{\boldsymbol{\xi}_{i}}\hspace{-0.07cm}\Big(\frac{1}{2}\boldsymbol{\xi}_{i}^T\textbf{Q}\boldsymbol{\xi}_{i} 
 \hspace{-0.1cm}-\hspace{-0.1cm}\langle {^{k}}\boldsymbol{\lambda}_{i}, \boldsymbol{\xi}_{i}\rangle 
\hspace{-0.1cm} +\hspace{-0.1cm}\frac{\rho}{2}\left\Vert \textbf{F}\boldsymbol{\xi}_{i}  
 \hspace{-0.1cm}-\hspace{-0.1cm}\textbf{g}({^{k}}\boldsymbol{\xi}_{\psi,i},{^{k}}\textbf{d}_{i}, {^{k}}\boldsymbol{\alpha}_{i}) \right \Vert_2^2 
  \Big )
  \label{zeta_1_sepration_1}, \textbf{A}\boldsymbol{\xi}_{i}\hspace{-0.1cm}= \hspace{-0.1cm}\textbf{b}
 \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Update ${^{k+1}}\boldsymbol{\xi}_{\psi,i}$ through
\vspace{-0.3cm}
\begin{align}
\hspace{-0.5cm}{^{k+1}}{\boldsymbol{\xi}_{\psi,i}} = \min_{\boldsymbol{\xi}_{\psi,i}}\Big(\frac{1}{2}
\boldsymbol{\xi}_{\psi,i}^T\ddot{\textbf{P}}^{T}\ddot{\textbf{P}}\boldsymbol{\xi}_{\psi,i}
 - \langle^{k}\boldsymbol{\lambda}_{\psi,i},
\boldsymbol{\xi}_{\psi,i}\rangle  
 \nonumber \\+ \frac{\rho}{2}\left\Vert \textbf{F}^{k+1}\boldsymbol{\xi}_{i}\hspace{-0.1cm} - \hspace{-0.05cm}
 \textbf{g}\hspace{-0.02cm}(\boldsymbol{\xi}_{\psi,i},\hspace{-0.14cm}{^{k}}\boldsymbol{\alpha}_{i},\hspace{-0.14cm}{^{k}}\textbf{d}_{i},\hspace{-0.14cm})\right \Vert_2^2
 \Big), \hspace{-0.05cm}\textbf{A}_{\psi}\boldsymbol{\xi}_{\psi,i} \hspace{-0.1cm}=\hspace{-0.07cm} \textbf{b}_{\psi} \label{compute_psi_tilta}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Update ${^{k+1}}\boldsymbol{\alpha}_{i}$ through
\vspace{-0.3cm}
\begin{align}
\hspace{-0.7cm}{^{k+1}}\boldsymbol{\alpha}_{i} \hspace{-0.1cm} = \hspace{-0.05cm}\min_{\boldsymbol{\alpha}_{i}}\hspace{-0.05cm}\Big(\hspace{-0.05cm} \frac{\rho}{2}\left\Vert \textbf{F}^{k+1} \boldsymbol{\xi}_{i}  
 \hspace{-0.1cm}-\hspace{-0.05cm}\textbf{g}(^{k+1}\boldsymbol{\xi}_{\psi,i}, \boldsymbol{\alpha}_{i},\hspace{-0.13cm}^{k} \textbf{d}_{i} ) \right \Vert_2^2 \Big) 
 \label{compute_ze_3}
\end{align}

%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Update ${^{k+1}}\textbf{d}_{i}$ through
\vspace{-0.3cm}
\begin{align}
\hspace{-0.65cm}{^{k+1}}\textbf{d}_{i} \hspace{-0.1cm}= \hspace{-0.05cm}\min_{\textbf{d}_{i}}\Big(\hspace{-0.05cm} \frac{\rho}{2}\left\Vert \textbf{F}^{k+1} \boldsymbol{\xi}_{i}  \hspace{-0.05cm}
 -
 \hspace{-0.05cm}\textbf{g}(^{k+1}\boldsymbol{\xi}_{\psi,i}, \hspace{-0.2cm}^{k+1}\boldsymbol{\alpha}_{i}, \textbf{d}_{i}) \right \Vert_2^2 \Big)
 \label{compute_ze_4}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\hspace{-0.15cm}Update Lagrange multiplier coefficient through
\vspace{-0.3cm}
\begin{align}
\hspace{-0.57cm}{^{k+1}}\boldsymbol{\lambda}_{i}\hspace{-0.09cm}=\hspace{-0.09cm}{^{k}}\boldsymbol{\lambda}_{i} \hspace{-0.09cm}- \hspace{-0.09cm}\rho( \textbf{F}^{k+1}\boldsymbol{\xi}_{i} 
 -\hspace{-0.09cm}\textbf{g}(^{k+1}\boldsymbol{\xi}_{\psi,i} , ^{k+1}\boldsymbol{\alpha}_{i},^{k+1}\textbf{d}_{i} )\hspace{-0.04cm})\textbf{F}
\label{update_lambda2_1} \\ 
{^{k+1}}\boldsymbol{\lambda}_{\psi,i}\hspace{-0.09cm}=\hspace{-0.09cm}{^{k}}\boldsymbol{\lambda}_{\psi,i} \hspace{-0.09cm}- \hspace{-0.09cm}\rho_{\psi}( \textbf{F}^{k+1}\boldsymbol{\xi}_{i} 
 -\hspace{-0.09cm}\textbf{g}(^{k+1}\boldsymbol{\xi}_{\psi,i} , ^{k+1}\boldsymbol{\alpha}_{i},^{k+1}\textbf{d}_{i} )\hspace{-0.04cm})\textbf{F}
\label{update_lambda2_1} 
\end{align}
}
\noindent \textbf{Return} ${^{k+1}}\boldsymbol{\xi}_{i}, {^{k+1}}\boldsymbol{\xi}_{\psi,i}, {^{k+1}}\boldsymbol{\alpha}_{i}, {^{k+1}}\textbf{d}_{i}$
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Analysis and Description of Algorithm \ref{alg_2}:} We provide a detailed breakdown of each line in Algorithm \ref{alg_2}.

\noindent \textbf{Line 2:} A glance at \eqref{reform_formulation} reveals that \eqref{reform_formulation} has the same structure as \eqref{over_1} where

\vspace{-0.6cm}
\small
\begin{align}
\hspace{-0.2cm}\overline{\textbf{Q}}= \hspace{-0.05cm} \textbf{Q} + \rho \textbf{F}^{T}\textbf{F},~~
\nonumber \\
\overline{\textbf{q}}_{i} = \hspace{-0.05cm} -{^k}\boldsymbol{\lambda}_{i}-\textbf{q}
-( \rho_{o}\textbf{F}^{T}\textbf{g}({^k}\boldsymbol{\xi}_{\psi,i},{^k}\boldsymbol{\alpha}_{i},{^k} \textbf{d}_{i}))^{T}
\label{zeta_1_sepration_3}
 \end{align}
\normalsize

\noindent Thus the solution of \eqref{zeta_1_sepration_1} over all the batches can be computed in one-shot using \eqref{over_3}.

\noindent \textbf{Line 3:}
In this step, we calculate the optimization variable $\boldsymbol{\xi}_{\psi,i}$. To compute this variable, we inspect \eqref{reform_formulation} and determine terms associated with $\boldsymbol{\xi}_{\psi,i}$. Given $^{k+1}\boldsymbol{\xi}{i}$, $^{k}\boldsymbol{\alpha}{i}$, and $^{k}\textbf{d}_{i}$, trajectory optimization \eqref{reform_formulation} can be expressed as \eqref{compute_psi_tilta}. The optimization problem \eqref{compute_psi_tilta} is then simplified as

\small
\begin{align}
\hspace{-0.2cm}{^{k+1}}{\boldsymbol{\xi}_{\psi,i}}\hspace{-0.1cm}= \hspace{-0.1cm}\min_{\boldsymbol{\xi}_{\psi,i}}\Big( \frac{1}{2}
\boldsymbol{\xi}_{\psi,i}^T\ddot{\textbf{P}}^{T}\ddot{\textbf{P}}\boldsymbol{\xi}_{\psi,i}
 \hspace{-0.1cm}-\hspace{-0.1cm}\langle ^{k}\boldsymbol{\lambda}_{\psi,i},
\boldsymbol{\xi}_{\psi,i}\rangle 
 \hspace{-0.1cm}+\hspace{-0.1cm}\frac{\rho_{o}}{2}\left\Vert  \begin{bmatrix}
   {^{k+1}}\boldsymbol{c}_{\psi,i} \\ {^{k+1}}\boldsymbol{s}_{\psi,i}
 \end{bmatrix} \hspace{-0.1cm}-\hspace{-0.1cm}\begin{bmatrix}
    \cos{\textbf{P}\boldsymbol{\xi}_{\psi,i}}\\
    \sin{\textbf{P}\boldsymbol{\xi}_{\psi,i}}
 \end{bmatrix}\right \Vert_2^2
 \Big) \label{compute_psi_tilta1}
\end{align}
\normalsize

\noindent Here, $\boldsymbol{c}_{\psi,i}$ and $\boldsymbol{s}_{\psi,i}$ are formed by aggregating the obtained slack variables, $c_{\psi,i}(t)$ and ${s}_{\psi,i}(t)$, across different time instances. Subsequently, by substituting the third term in \eqref{compute_psi_tilta1} with a convex surrogate \cite{singh2020bi}, $\boldsymbol{\xi}_{\psi,i}$ and consequently $\boldsymbol{\psi}_{i}$ can be determined by solving

\small
\begin{align}
{^{k+1}}{\boldsymbol{\xi}_{\psi,i}} = \min_{\boldsymbol{\xi}_{\psi,i}}\Big( \frac{1}{2}
\boldsymbol{\xi}_{\psi,i}^T\ddot{\textbf{P}}^{T}\ddot{\textbf{P}}\boldsymbol{\xi}_{\psi,i}
 - \langle ^{k}\boldsymbol{\lambda}_{\psi,i},
\boldsymbol{\xi}_{\psi,i}\rangle 
 \nonumber \\
 + \frac{\rho_{o}}{2}
\left\Vert
\arctan2({^{k+1}}\boldsymbol{s}_{\psi,i},{^{k+1}}\boldsymbol{c}_{\psi,i}) - \textbf{P}\boldsymbol{\xi}_{\psi,i}
\right \Vert_2^2 \Big),~ \textbf{A}\boldsymbol{\xi}_{\psi,i} = \textbf{b}_{\psi}.
\label{compute_convex_surrogate}
\end{align}
\normalsize 

\noindent where the optimization problem \eqref{compute_convex_surrogate} takes the form of a \gls{qp}, allowing for the efficient computation of its batch solution in one shot using \eqref{over_3}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Line 4:}
In this stage, our objective is to compute ${^{k+1}}\boldsymbol{\alpha}_{i}$ using \eqref{reform_formulation}. To achieve this, we identify the terms associated with ${^{k+1}}\boldsymbol{\alpha}_{i}$, update $\boldsymbol{\xi}_{i}$ and $\boldsymbol{\xi}_{\psi,i}$, and then simplify our optimization problem as shown in \eqref{compute_ze_3}. ${^{k+1}}\boldsymbol{\alpha}_{i}$ comprises three variables: $\boldsymbol{\alpha}_{mj,i}$, $\boldsymbol{\alpha}_{v,i}$, and $\boldsymbol{\alpha}_{a,i}$, each of which is independent. Consequently, we can decompose \eqref{compute_ze_3} into three parallel optimization problems as

\small
\begin{subequations}
\begin{align}
{^{k+1}}\boldsymbol{\alpha}_{mj,i} =   \min_{\boldsymbol{\alpha}_{mj,i}} 
\hspace{-0.08cm}\frac{\rho_{o}}{2}
\times\left\Vert  \begin{matrix}
 \overbrace{  
   {^{k+1}}\textbf{x}_{i}+ r_{m} \cos{{^{k+1}}\boldsymbol{\psi}_{i}} -  \textbf{x}_{o,j}
}^{{^{k+1}}\Tilde{\textbf{x}}_{i}}
 -a{^{k}} \textbf{d}_{mj,i} \cos{\boldsymbol{\alpha}_{mj,i}} 
\\
 \underbrace{
   {^{k+1}}\textbf{y}_{i} + r_{m}\sin{{^{k+1}}\boldsymbol{\psi}_{i}} -  \textbf{y}_{o,j}
 }_{{^{k+1}}\Tilde{\textbf{y}}_{i}}
 -b{^{k}}\textbf{d}_{mj,i}\sin{\boldsymbol{\alpha}_{mj,i}}
 \end{matrix}
 \right \Vert_2^2 \hspace{-0.2cm}
 \label{compute_zeta_33}  \\
{^{k+1}}\boldsymbol{\alpha}_{v,i} = \min_{\boldsymbol{\alpha}_{v,i}}\frac{\rho_{o}}{2} \left\Vert
\begin{matrix}
{^{k+1}}\dot{\textbf{x}}_{i}-{^{k}}\textbf{d}_{v,i}\cos{\boldsymbol{\alpha}_{v,i}}
\\
 {^{k+1}}\dot{\textbf{y}}_{i}-{^{k}}\textbf{d}_{v,i}\sin{\boldsymbol{\alpha}_{v,i}}
 \end{matrix}
\right \Vert_2^2 \label{compute_av1}
\\
{^{k+1}}\boldsymbol{\alpha}_{a,i}  = \min_{\boldsymbol{\alpha}_{v,i}}
\frac{\rho_{o}}{2} \left\Vert
\begin{matrix}
{^{k+1}}\ddot{\textbf{x}}_{i}-{^{k}}\textbf{d}_{a,i}\cos{\boldsymbol{\alpha}_{a,i}}
\\
 {^{k+1}}\ddot{\textbf{y}}_{i}-{^{k}}\textbf{d}_{a,i}\sin{\boldsymbol{\alpha}_{a,i}}
 \end{matrix}
\right \Vert_2^2 
\label{compute_acc}
\end{align}
\end{subequations}
\normalsize

Similar to our prior work, although \eqref{compute_zeta_33}-\eqref{compute_acc} exhibit non-convexity, their solutions can be readily computed through geometric reasoning.  It is noteworthy that each element of $\boldsymbol{\alpha}_{mj,i}$, $\boldsymbol{\alpha}_{v, i}$, and $\boldsymbol{\alpha}_{a,i}$ is independent of the others for a given position trajectory.
Consequently, \eqref{compute_zeta_33} can be interpreted as the projection of ${{^{k+1}}\Tilde{\textbf{x}}_{i}}$ and ${{^{k+1}}\Tilde{\textbf{y}}_{i}}$ onto an axis-aligned ellipse centered at the origin. Similarly, \eqref{compute_av1} and \eqref{compute_acc} can be viewed as the projection of (${^{k+1}}\dot{\textbf{x}}_{i}$, ${^{k+1}}\dot{\textbf{y}}_{i}$) and (${^{k+1}}\ddot{\textbf{x}}_{i}$, ${^{k+1}}\ddot{\textbf{y}}_{i}$) onto a circle centered at the origin with radii $\textbf{d}_{v,i}\times v_{max}$ and $\textbf{d}_{a,i} \times a_{max}$, respectively. Thus, the solutions of \eqref{compute_zeta_33}-\eqref{compute_acc} can be expressed as

\small
\begin{subequations}
\begin{align}
{^{k+1}}\boldsymbol{\alpha}_{mj,i} = \arctan2 ({^{k+1}}\Tilde{\textbf{y}}_{i}, {^{k+1}}\Tilde{\textbf{x}}_{i}).
\label{zeta_2}\\
{^{k+1}}\boldsymbol{\alpha}_{v,i} = \arctan2 ({^{k+1}}\dot{\textbf{y}}_{i}, {^{k+1}}\dot{\textbf{x}}_{i}).
\label{alpha_v}\\
{^{k+1}}\boldsymbol{\alpha}_{a,i} = \arctan2 ({^{k+1}}\ddot{\textbf{y}}_{i}, {^{k+1}}\ddot{\textbf{x}}_{i}).
\label{alpha_a}
 \end{align}
 \end{subequations}
 \normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Line 5:} We update the acquired optimization variables and reformulate the optimization problem \eqref{reform_formulation} in terms of ${^{k+1}}\textbf{d}_{i}$ as shown in \eqref{compute_ze_4}. Following a similar procedure as in the previous step, our optimization problem \eqref{compute_ze_4} can be reduced into three independent optimization problems:

\small
\begin{subequations}
    \begin{align}
{^{k+1}}\textbf{d}_{mj,i} = \min_{\textbf{d}_{mj,i} \geq 1 }  \frac{\rho_{o}}{2}\left\Vert \begin{matrix}
{^{k+1}}\Tilde{\textbf{x}}_{i}
- a\textbf{d}_{mj,i} \cos{{^{k+1}}\boldsymbol{\alpha}_{mj,i}} \\
{^{k+1}}\Tilde{\textbf{y}}_{i}
 -b\textbf{d}_{mj,i} \sin{{^{k+1}}\boldsymbol{\alpha}_{mj,i}} \end{matrix}  \right \Vert_2^2
 \label{compute_d_mij} \\
 {^{k+1}}\textbf{d}_{v,i} = \max_{\textbf{d}_{v,i}\leq 1}\frac{\rho_{o}}{2} \left\Vert \begin{matrix} {^{k+1}}\dot{\textbf{x}}_{i}-\textbf{d}_{v,i}\cos{{^{k+1}}\boldsymbol{\alpha}_{v,i}}\\
 {^{k+1}}\dot{\textbf{y}}-\textbf{d}_{v,i}\sin{{^{k+1}}\boldsymbol{\alpha}_{v,i}}
 \end{matrix}
\right \Vert_2^2  \label{compute_dv}\\
{^{k+1}}\textbf{d}_{a,i} =  \max_{\textbf{d}_{a,i}\leq 1}\frac{\rho_{o}}{2} \left\Vert \begin{matrix} 
{^{k+1}}\ddot{\textbf{x}}_{i}-\textbf{d}_{a,i}\cos{{^{k+1}}\boldsymbol{\alpha}_{a,i}} \\
  {^{k+1}}\ddot{\textbf{y}}_{i}-\textbf{d}_{a,i}\sin{{^{k+1}}\boldsymbol{\alpha}_{a,i}}
  \end{matrix}
\right \Vert_2^2 \label{compute_da}
\end{align}
\end{subequations}
\normalsize

\noindent Since elements of $\textbf{d}_{a,i}$ and $\textbf{d}_{v,i}$ at different time instances are independent of each other, the problem can be reduced to $i \times n_{v}$ \gls{qp} parallel problems, allowing for simultaneous solution. In a similar way, we can reduce \eqref{compute_d_mij} problem into  $i\times m \times n_{v}$ \gls{qp}s. 

\noindent \textbf{Line 6:}
Lagrange multipliers are updated based on residuals \cite{goldstein2009split}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation and Benchmarking}
\noindent \textbf{Implementation Details:} We implemented both our algorithm and \gls{cem} in Python, utilizing the JAX \cite{bradbury2018jax} libraries as a \gls{gpu}-accelerated backend. Additionally, we developed a \gls{mpc} framework on our batch optimizer, initializing Lagrange multipliers $\boldsymbol{\lambda}_{i}$ and $\boldsymbol{\lambda}_{\psi, i}$ with the solution from the preceding control loop. The \gls{mpc} executed within a time budget of $0.04s$, sufficient for ten iterations of our optimizer with a batch size of 1000. We employ three metrics to evaluate our proposed method, each defined as: 
\begin{itemize}
     \item Success-Rate: Total evaluated problems ($20$) in benchmark divided by successful runs with no collisions.
    \item Tracking Error: defined as $(x_i(t)-x_{des}(t))^2+(y_{i}(t)-y_{des}(t))^2$. The desired trajectory is chosen as a straight line between the initial and final point with a constant velocity.
    \item Smoothness cost: acceleration value used in navigation.
\end{itemize}
Furthermore, the validation benchmarks used are outlined below.

\begin{itemize}
    \item Benchmark 1, Static Crowd: In this benchmark, we generated an environment including static human crowds with size 30.
    \item Benchmark 2, Same Direction Flow: In this benchmark, the human crowd is in motion in the same direction as the robot and with a max velocity of $0.3 m/s$. The robot follows a straight-line trajectory with a velocity of $1.0 m/s$ and needs to overtake the human crowds.
    \item Benchmark 3, Opposite Direction Flow:
    For this benchmark, the crowd is moving with a max velocity of $1.0 m/s$, and the robot is moving in the opposite direction tracking a straight-line trajectory with $1.0 m/s$ desired speed.
\end{itemize}

\noindent \textbf{Qualitive Results:} In Fig. \ref{modeling_snapshots}, we illustrated the qualitative results of \gls{mpc} built on top of our proposed optimizer at three different snapshots for Benchmark 1 and Benchmark 2 (For better visualization, visit our youtube video \footnote{https://www.youtube.com/watch?v=ZlWJk-w03d8}). 

\begin{figure}[!h]
\centering
    \includegraphics[scale=0.6]{figures/snap_shot.png}
    \caption[Qualitative result of MPC built on top of our batch optimizer]{\small{Qualitative result of \gls{mpc} built on top of our batch optimizer. The top and bottom rows show the navigation in Benchmarks 2 and 1, respectively. The green trajectories are the different locally optimal solutions obtained with our batch optimizer. The blue trajectories show the past positional traces of the robot. The trajectories in red show the predicted motion of the obstacles }}
    \label{modeling_snapshots}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Validating the batch optimizer:}
\noindent In Fig.\ref{convergence}, we show the changes of non-convex equality constraints residuals, \eqref{reform_eq}, and the convex surrogate residuals, introduced in \eqref{compute_convex_surrogate} for different iterations. Here, we are only plotting the residual for the best trajectory of the batch. As can be seen, by increasing the number of iterations,  the residuals approach zero. Thus, the kinematic and collision avoidance constraints are gradually satisfied. We also provided another validation in Fig.\ref{homotopy}; as iteration progresses, we get more locally optimal trajectories residing in different homotopies.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.35]{figures/convergence.png}
    \caption[Batch optimizer residuals]{Validating optimizer convergence empirically. The residual constraints, $\Vert \textbf{F}\boldsymbol{\xi}_{i}-\textbf{g}_{i}\Vert$ and $\Vert \arctan2(s_{\psi,i},c_{\psi,i})-\textbf{P}\boldsymbol{\xi}_{\psi,i}\Vert$ go to zero over iterations.}
    \label{convergence}
\end{figure}

\begin{figure}[!h]
\centering
    \includegraphics[scale=0.22]{figures/homotopies_1.eps}
    \caption[increasing the number of homotopies over iterations]{The number of feasible homotopies increases by iterations. Trajectories are plotted over 5, 20, 30, and 50 iterations in Fig. (a), (b), (c), (d), respectively. The initial guess trajectories, the best trajectory among batches, and feasible trajectories are in blue, red, and green, respectively. }
    \label{homotopy}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Quantitive results:}
\begin{enumerate}
    \item \textit{Comparison with Baseline \gls{mpc}}:
    In this step, our objective is to analyze how the navigation performance evolves with an increase in batch size. For comparison, we establish the \gls{mpc} setting with a batch size of one as the baseline and subsequently increase the number of batches. It is important to note that any off-the-shelf optimizer can be employed in this comparison. We tried to use ACADO \cite{houska2011acado}, but it could not achieve reliable and real-time performance for the provided benchmarks.
    
    Table \ref{Table_batch_size} presents our results. Notably, the \gls{mpc} baseline exhibits a very low success rate, approximately one percent. However, with an increase in the number of batches, our success rate experiences a gradual ascent and reaches to 97\% success rate for 1000 batches. Additionally, a slight increase in tracking error and acceleration is observed, attributed to the necessity for our optimizer to take detours in order to furnish a collision-free trajectory.

%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\scriptsize
\centering
\caption{\small{Performance Metrics with Respect to Batch Size }}
\label{Table_batch_size}
\begin{tabular}{|l|l|l|l|}
\hline
\rowcolor[HTML]{9698ED} 
Batch size                            & Success rate & \begin{tabular}[c]{@{}l@{}}Tracking error (m)\\ mean/max/min\end{tabular} & \begin{tabular}[c]{@{}l@{}}Acceleration ($m/s^{2}$)\\ mean/max/min\end{tabular} \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{009901}1 (Baseline)  & 0.016        & 3.19/4.78/1.69                                       & 0.097/0.29/0.0003                 \\ \hline
\cellcolor[HTML]{009901}200           & 0.8          & 3.15/4.89/1.51                                         & 0.15/0.37/0.0006                 \\ \hline
\cellcolor[HTML]{009901}400           & 0.88         & 3.10/4.77/1.32                                        & 0.139/0.32/0.0005             \\ \hline
\cellcolor[HTML]{009901}600           & 0.9          & 3.09/4.74/1.39                                         & 0.139/0.32/0.0005               \\ \hline
\cellcolor[HTML]{009901}800           & 0.95         & 3.07/4.75/1.45                                       & 0.136/0.31/0.004               \\ \hline
\cellcolor[HTML]{009901}\textbf{1000} & \textbf{100} & \textbf{3.06/4.65/1.56}                                                   & \textbf{0.166/0.31/0.03}        \\ \hline
\end{tabular}
\end{table}
\normalsize

%%%%%%%%%%%%%
    \item \textit{Comparison with \gls{cem}}:
    We present the pivotal results of our paper by comparing our optimizer with the \gls{sota}, \gls{cem}, in an \gls{mpc} setting in Table \ref{table_com_cem}. To make the comparison, we consider 8k samples (8 times of the number of our samples) and heavily vectorized the cost evaluations in \gls{cem}. Through trial and error, we obtained the number of iterations of CEM that can be performed within $0.04s$ (the computation time of our MPC).

    On \textbf{Benchmark 1}, our success rate is an impressive 100\%, surpassing \gls{cem} by 15\%. Furthermore, our average tracking error is 43\% lower than \gls{cem} on the same benchmark. For \textbf{Benchmark 2} and \textbf{Benchmark 3}, our optimizer's success rates are 20\% and 45\% higher than \gls{cem}, respectively. Similarly, our tracking error remains lower than \gls{cem} on these benchmarks. Notably, the \gls{cem} method generally deploys less acceleration on average compared to our proposed method. This arises from our method's dual focus on minimizing acceleration and addressing the need to navigate obstacles while following the desired trajectory. In more challenging scenarios, our method may utilize more acceleration to yield feasible trajectories, contributing to a higher success rate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\scriptsize
\centering
\caption{\small{Comparison with \gls{cem}}}
\label{table_com_cem}
\begin{tabular}{|l|l|l|l|}
\hline
\rowcolor[HTML]{268A22} 
Method                   & Success rate   & \begin{tabular}[c]{@{}l@{}}Tracking error (m)\\ mean/max/min\end{tabular} & \begin{tabular}[c]{@{}l@{}}Acceleration ($m/s^{2}$)\\ mean/max/min\end{tabular} \\ \hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Our Benchmark 1} & \textbf{100\%} & \textbf{2.44/5.44/0.079}                                                  & \textbf{0.13/0.32/0.0}             \\ \hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Our Benchmark 2} & \textbf{95\%}  & \textbf{3.11/5.01/0.88}                                                   & \textbf{0.20/0.49/0.0}           \\ \hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Our Benchmark 3} & \textbf{95\%}  & \textbf{2.74/4.82/0.07}                                                   & \textbf{0.17/0.45/0.0}          \\ \hline
\rowcolor[HTML]{FFA7A7} 
CEM Benchmark            & 85\%           & 3.5/5.22/1.94                                                             & 0.09/0.36/0.0                       \\ \hline
\rowcolor[HTML]{FFA7A7} 
CEM Benchmark            & 75\%           & 3.99/6.87/1.12                                                            & 0.09/0.28/0.0                    \\ \hline
\rowcolor[HTML]{FFA7A7} 
CEM Benchmark            & 40\%           & 3.25/4.05/2.56                                                            & 0.13/0.46/0.0                     \\ \hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item \textit{Computation Time Scaling:} Fig. \ref{modeling} visually presents the per-iteration computation time scaling of our batch optimizer for varying numbers of circles and obstacles. Notably, the plot indicates a (sub)linear scaling of per-iteration computation time in relation to the number of circles and obstacles. This trend can be attributed to the matrix algebra employed in our optimizer. Specifically, a linear increase in~the number of footprint circles or obstacles leads to a similar increase in the number of rows of matrices $\textbf{F}$ and $\textbf{g}_{i}$, while the number of columns remains constant. Consequently, the computation cost of obtaining $\textbf{F}^T\textbf{g}_{i}$ in \eqref{zeta_1_sepration_3} can be made approximately linear through suitable \gls{gpu} parallelization. Also, the matrices $\textbf{F}^T\textbf{F}$ need to be computed only once since they remain constant across iterations and batches. A similar linear complexity analysis applies to the solutions of (\ref{compute_psi_tilta}) as well, where solutions are available as symbolic formulae, ensuring linear complexity concerning the variables $n_{c}$ and $n_{o}$.

    
    \begin{figure}[h]
\centering
    \includegraphics[scale=0.2]{figures/fig_66.png}
    \caption[Computation time-scaling]{Time per iteration(ms) for batch size 1000. Solutions are typically obtained within $5-10$ iterations. The figure presents the scaling with respect to the number of circles used to approximate the footprint of the robot and the number of obstacles in the environment.}
    \label{modeling}
\end{figure}


    Additionally, we assess the per-iteration computation time of our vectorized batch optimizer across \gls{gpu}s and multi-threaded \gls{cpu}s in Table. \ref{gpu-cpu}. The advantage of the latter lies in its ability to execute any off-the-shelf optimizer in parallel CPU threads without necessitating changes to the underlying matrix algebra. However, CPU parallelization introduces a scenario where each problem instantiation competes with others for computational resources, potentially slowing down the overall computation time. Our experiments revealed that a C++ version of our optimizer performed smoothly with a batch size of 5, achieving a per-iteration computation time of $0.0015s$, which was competitive with our \gls{gpu} implementation. Nevertheless, scaling beyond this batch size resulted in a significant slowdown. For instance, with a batch size of 6, the per-iteration CPU time increased to $0.03s$. Hence, for larger batch sizes, it became more practical to run sequential instantiations with mini-batches of 5. We note that a more rigorous implementation might improve batch equality-constrained \gls{qp} structure in some critical steps in the performance of multi-threaded CPU-based batch optimization. However, our current bench-marking establishes the computational benefit derived from several layers of reformulation that induced equality-constrained \gls{qp} structure in some critical steps of our batch optimizer and allowed for effortless \gls{gpu} acceleration. 
 


%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\scriptsize
\centering
\caption{\small{Per-iteration comparison for \gls{gpu} vs multi-threaded \gls{cpu}}}
\label{gpu-cpu}
\begin{tabular}{|l|llllll|}
\hline
\rowcolor[HTML]{036400} 
\cellcolor[HTML]{FFFFFF}                   & \multicolumn{6}{c|}{\cellcolor[HTML]{036400}{\color[HTML]{FFFFFF} Batch size}}  \\ \cline{2-7} 
\rowcolor[HTML]{9AFF99} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}5}               & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}200}             & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}400}             & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}600}             & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}800}             & 1000            \\ \hline
\rowcolor[HTML]{DAE8FC} 
GPU                                        & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}0.0016}          & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}\textbf{0.0017}} & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}\textbf{0.0026}} & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}\textbf{0.0033}} & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}\textbf{0.0039}} & \textbf{0.0045} \\ \hline
\rowcolor[HTML]{FFCC67} 
CPU                                        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}\textbf{0.0015}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}0.075}           & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}0.12}            & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}0.18}            & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}0.24}            & 0.3             \\ \hline
\end{tabular}
\end{table}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interrelation:}

The concept of representing rectangular robots using multiple overlapping circles is drawn from the polar representation of collision avoidance constraints outlined in the earlier paper. Similarly, the approach to reformulating boundaries is inspired by previous work.

Moreover, the \gls{qp} structure proposed in Paper I acts as a foundation for the notion of formulating trajectory optimization for multiple initial guesses concurrently and redefining the problem. Additionally, Algorithm \ref{alg_2} serves as an extension of Algorithm \ref{alg_1} and employs analogous procedures to solve the trajectory optimization problem. By getting inspiration from batch trajectory optimization, we will establish our next paper. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Paper III}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Context:}

%%%%%%%%%%%%%%%%%%%%General sentence
Efficient and collision-free navigation in dynamic, unknown environments is a critical requirement for deploying mobile robots in diverse settings such as hospitals, warehouses, and airports. These environments present challenges due to the changing layouts of static obstacles and the introduction of dynamic obstacles through human movement. As a consequence, precomputed global plans may become infeasible during robot motion, necessitating local planners with the capability to explore different trajectory homotopies in real-time over extended horizons. In this paper, our focus is on empowering mobile robots with such capabilities, particularly through optimization-based local planners known for their constraint satisfaction and smooth motion generation.

Trajectory optimization methods fall into two main categories: gradient-based approaches and sampling-based planners. Gradient-based approaches, \cite{metz2003rockit, vanroye2023fatrop}, rely on the differentiability of cost and constraint functions. These methods often require a well-initialized trajectory, posing challenges in rapidly changing environments. On the other hand, sampling-based planners, such as \gls{cem} \cite{bharadhwaj2020model} and CMA-ES \cite{jankowski2023vp}, explore the state-space through random sampling, allowing them to find locally optimal solutions without relying on differentiability. Despite their exploration capabilities, these optimizers face challenges when all sampled trajectories end up in the infeasible (high-cost) region (see Fig. \ref{fig_teaser}(a-c)).

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.6
    ]{figures/teaser_44.png}
    \caption[Simple comparison between CEM and PRIEST]{\small{A comparison between \gls{cem} (left column) and \gls{priest} (middle column). Fig.(a)-(c) shows how \gls{cem} (or any typical sampling-based optimizer) struggles when all the sampled initial trajectories lie in the infeasible (high-cost) region. Our approach, \gls{priest}, integrates a projection optimizer within any standard sampling-based approach that guides the samples toward feasible regions before evaluating their cost. Fig.(g)-(h) presents changes in the cost function values, and constraint residuals change across both \gls{cem} and \gls{priest} iterations.}}
    \label{fig_teaser}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%Our goal
Our main motivation is to integrate the advantages of both sampling-based and gradient-based methods. Previous attempts in this direction have mostly focused on utilizing sampling-based optimizers to generate~an initial trajectory, which is then input to the gradient-based solver \cite{kim2022mppi}.~In the next section, we will explain the main idea and innovations of our current work.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contribution:}

%%%%%%%%%%%%%%%%%main idea
Our main idea in this paper is to use gradient-based approaches to improve the inner workings of sampling-based optimizers. To do this, we introduce a projection optimization that directs the sampling process toward feasible(low-cost) regions at each iteration. Thus, our approach can handle pathological cases where all sampled trajectories are infeasible, e.g., due to violation of collision constraints(see Fig.\ref{fig_teaser}(d-f)). Our core innovations and their benefits are summarized in the following highlights.

\begin{enumerate}
    \item \textbf{Algorithmic Contribution:} The heart of \gls{priest} lies in an innovative optimizer with the distinct ability to take a set of trajectories, project each one onto the feasible set, and refine the sampling distribution. In this paper, we illustrate how our projection optimizer can be effectively parallelized and accelerated on \gls{gpu}s. The key to this achievement lies in the reformulation of underlying collision and kinematic constraints into polar form, coupled with an \gls{am} approach to tackle the resulting problem. Furthermore, our optimizer naturally integrates with decentralized variants of sampling-based optimizers \cite{zhang2022simple}, wherein multiple sampling distributions~are refined in parallel to enhance the optimality of the solution. 
    \item \textbf{Improvement over \gls{sota}:} \gls{priest} shines when compared to existing approaches. It demonstrates superior performance in terms of success rate, time-to-reach the goal, computation time, etc. Notably, on the \gls{barn} dataset \cite{perille2020benchmarking}, \gls{priest} surpasses the \gls{ros} Navigation stack, boasting at least a 7\% increase in success rate and halving the travel time. On the same benchmarks,~our success rate is at least 35\% better than \gls{sota} local sampling-based optimizers like \gls{mppi} \cite{williams2017model} and log-MPPI \cite{mohamed2022autonomous}. Additionally, we consider a point-to-point navigation~task and compare \gls{priest} with the SOTA gradient-based solvers, ROCKIT \cite{metz2003rockit}(a collection of optimizers like IPOPT, ACADO, etc) and \gls{fatrop} \cite{vanroye2023fatrop}, and sampling-based methods \gls{cem} and \gls{vpsto} \cite{jankowski2023vp}. We show up to a $2$x improvement in success rate over these baselines. Finally, we show that \gls{priest} respectively has 17\% and 23\% higher success rates than the \gls{ros} Navigation stack and other \gls{sota} approaches in dynamic environments. 
\end{enumerate}

\subsection{Problem Formulation}

%%%%%%%%%%%%%%%%%55Differential flatness
\noindent \textbf{Differential flatness:} We assume that the control inputs, $\textbf{u}$,  can be expressed as analytical mapping functions, $\boldsymbol{\Phi}$, of the $q^{th}$ level derivatives of the position-level trajectory: $\textbf{u} = \boldsymbol{\Phi}(x^{(q)}(t), y^{(q)}(t), z^{(q)}(t))$. For example, the forward velocity and curvature control input for a car-like robot can be expressed as $\boldsymbol{\Phi}\hspace{-0.12cm}=\hspace{-0.12cm}(\hspace{-0.07cm}\sqrt{\dot{x}(t)^2+\dot{y}(t)^2}, \frac{\ddot{y}(t)\dot{x}(t)-\ddot{x}(t)\dot{y}(t) }{ (\dot{x}(t)^2+\dot{x}(t)^2)^{1.5}})$, or for a quadrotor, the pitch, roll, yaw angles, and thrust can be analytically expressed in terms of axis-wise accelerations. The adoption of differential flatness serves to eliminate the explicit necessity for nonlinear equality constraints originating from the motion model \cite{han2023efficient}, which is instrumental for the parallelized and \gls{gpu}-accelerated structure in \gls{priest}.

%%%%%%%%%%%%%%%%%%%%%%%%%%Trajectory optimzation
\noindent \textbf{Trajectory Optimization:}
We are interested in solving the following 3D trajectory optimization:

\vspace{-0.45cm}
\small
\begin{subequations}
\begin{align}
   \hspace{-2.5cm}\min_{x(t), y(t), z(t)} c_1(x^{(q)}(t), y^{(q)}(t), z^{(q)}(t)),  
\label{acc_cost_priest}\\
x^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.05cm}y^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.05cm}z^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm})|_{t=t_{0}}\hspace{-0.05cm}=\hspace{-0.05cm}\textbf{b}_{0},~
   x^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm}),\hspace{-0.05cm}y^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm}), \hspace{-0.05cm}z^{(\hspace{-0.02cm}q\hspace{-0.02cm})}\hspace{-0.05cm}(\hspace{-0.02cm}t\hspace{-0.02cm})|_{t=t_{f}}\hspace{-0.05cm}= \hspace{-0.05cm}\textbf{b}_{f},\label{eq1_multiagent_1_priest}\\
    \dot{x}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.05cm}+\hspace{-0.05cm} \dot{y}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.05cm}+ \hspace{-0.05cm}\dot{z}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm}) \leq v^{2}_{max}, ~
    \ddot{x}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm}) \hspace{-0.05cm}+\hspace{-0.05cm} \ddot{y}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm}) \hspace{-0.05cm}+ \hspace{-0.05cm}\ddot{z}^{2}(\hspace{-0.02cm}t\hspace{-0.02cm}) \leq a^{2}_{max}, \label{acc_constraint_priest}\\
    s_{min} \leq (x(t), y(t), z(t)) \leq s_{max}, \label{affine_ineq_priest}  \\
    \hspace{-0.4cm}
    -\frac{\hspace{-0.07cm}(x(t)\hspace{-0.09cm}-
 \hspace{-0.06cm}x_{o, j}(t)\hspace{-0.01cm})^{2}}{a^2}\hspace{-0.09cm} - \hspace{-0.09cm}
 \frac{\hspace{-0.07cm}(y(t) \hspace{-0.075cm}-\hspace{-0.065cm}y_{o, j}(t)\hspace{-0.02cm})^{2}}{a^2} 
  \hspace{-0.09cm}-\hspace{-0.09cm}\frac{\hspace{-0.07cm}(z(t)\hspace{-0.09cm}- 
 \hspace{-0.08cm}z_{o, j}(t)\hspace{-0.01cm})^{2}}{b^2}\hspace{-0.06cm} \hspace{-0.06cm}
  + \hspace{-0.05cm}1\leq 0, \label{coll_multiagent_priest}
\end{align}
\end{subequations}
\normalsize

\noindent where the cost function $c_1(\cdot)$ is expressed in terms of $q^{th}$ derivatives of position-level trajectories, allowing for the inclusion of penalties related to accelerations, velocities, curvature, etc., where $q\hspace{-0.10cm}=\hspace{-0.10cm}{0,1,2}$. Additionally, we leverage differential flatness to enhance control costs within $c_1(\cdot)$. It should be mentioned that in our approach, the cost functions $c_1(\cdot)$ are not required to be convex, smooth, or even possess an analytical form. The vectors $\textbf{b}_{0}$ and $\textbf{b}_{f}$ in \eqref{eq1_multiagent_1_priest} denote the initial and final values of boundary conditions. The affine inequalities in \eqref{affine_ineq_priest} set bounds on the robot's workspace. Constraints on velocity and acceleration are imposed by \eqref{acc_constraint_priest}. Lastly, \eqref{coll_multiagent_priest} enforces collision avoidance, assuming obstacles are modeled as axis-aligned ellipsoids with dimensions $(a, a, b)$.

By adapting the parametrized optimization \eqref{param} and compact version of variables, we can reformulate \eqref{acc_cost_priest}-\eqref{coll_multiagent_priest} as

\vspace{-0.55cm}
\small
\begin{subequations}
\begin{align}   \min_{\hspace{0.1cm}\boldsymbol{\xi}} c_1(\boldsymbol{\xi}),  \label{cost_modify} \\
    \textbf{A}\boldsymbol{\xi} = \textbf{b}_{eq},\label{eq_modify}\\
   \textbf{g}(\boldsymbol{\xi}) \leq \textbf{0} \label{reform_bound},
   \vspace{-0.2cm}
\end{align}
\end{subequations}
\normalsize
\vspace{-0.5cm}

\noindent Where $\boldsymbol{\xi} = \begin{bmatrix}
\bold{c}_{x}^{T}&\hspace{-0.3cm}\bold{c}_{y}^{T}&\hspace{-0.3cm}
\bold{c}_{z}^{T}
\end{bmatrix}^T$. With a slight abuse of notation, $c_1(\cdot)$ is now used to denote a cost function dependent on $\boldsymbol{\xi}$. The matrix $\textbf{A}$ is block diagonal, where each block on the main diagonal consists of $ \begin{bmatrix}
\bold{P}_{0}&\hspace{-0.22cm}\dot{\bold{P}}_{0}&\hspace{-0.22cm}\ddot{\bold{P}}_{0}&\hspace{-0.22cm} \bold{P}_{-1}
\end{bmatrix}$. The subscripts $0$ and $-1$ signify the first and last row of the respective matrices, corresponding to the initial and final boundary constraints. The vector $\textbf{b}_{eq}$ is simply the stack of $\textbf{b}_{0}$ and $\textbf{b}_{f}$. The function $\textbf{g}$ contains all the inequality constraints \eqref{acc_constraint_priest}-\eqref{coll_multiagent_priest}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Main Algorithmic Results}
%%%%%%%%%%%%%%%%%%%%main idea
This section presents our fundamental algorithmic contributions. Fig. \ref{fig_overview} provides a visual overview of our proposed approach, highlighting its distinctive features compared to existing baselines. A pivotal distinction lies in the insertion of the projection optimizer between the sampling and cost evaluation blocks. 

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.6
    ]{figures/teaser_10.png}
    \caption{Comparison between a sampling-based optimizer (a) and PRIEST~(b).}
    \label{fig_overview}
\end{figure}

Now, we introduce our main block, the projection optimizer, and subsequently, we detail its integration into a sampling-based optimizer.

\subsubsection{Projection Optimization}
We can demonstrate that for a specific class of constraint functions $\textbf{g}$ involving quadratic and affine constraints, the optimization problem

\vspace{-0.5cm}
\small
\begin{subequations}
\begin{align}
     \min_{\overline{\boldsymbol{\xi}}_{i}} \frac{1}{2}\Vert \overline{\boldsymbol{\xi}}_i-\boldsymbol{\xi}_{i}\Vert_2^2, ~ i=1,2,...,N_{b} 
    \label{projection_cost}\\
    \textbf{A}\overline{\boldsymbol{\xi}}_{i} = \textbf{b}_{eq}, \qquad \textbf{g}(\overline{\boldsymbol{\xi}}_{i}) \leq  \textbf{0}, \label{projection_const}
\end{align}
\end{subequations}
\normalsize

\noindent where the cost function \eqref{projection_cost} aims to minimally modify the $i^{th}$ sampled trajectory $\boldsymbol{\xi}_i$ to $\overline{\boldsymbol{\xi}}_{i}$ in order to satisfy the equality and inequality constraints, can be reduced to the fixed-point iteration of the following form

\vspace{-0.5cm}
\small
\begin{subequations}
    \begin{align}
    {^{k+1}}\textbf{e}_i, {^{k+1}}\boldsymbol{\lambda}_i = \textbf{h} ({^k} \overline{\boldsymbol{\xi}}_{i}, {^k}\boldsymbol{\lambda}_i )\label{fixed_point_1}\\
\hspace{-0.2cm}{^{k+1}}\overline{\boldsymbol{\xi}}_{i} \hspace{-0.1cm}=\hspace{-0.1cm}\arg\min_{\overline{\boldsymbol{\xi}}_{i}} \frac{1}{2}\Vert \overline{\boldsymbol{\xi}}_{i}-\boldsymbol{\xi}_i\Vert_2^2 +\frac{\rho}{2} \left\Vert \textbf{F}\overline{\boldsymbol{\xi}}_{i} -{^{k+1}}\textbf{e}_{i} \right\Vert_2^2\hspace{-0.2cm}-\hspace{-0.1cm}{^{k+1}}\boldsymbol{\lambda}_i^T\overline{\boldsymbol{\xi}}_{i}, \nonumber \\ \qquad \textbf{A}\overline{\boldsymbol{\xi}}_{i} = \textbf{b}_{eq} \label{fixed_point_2}
\end{align}
\end{subequations}
\normalsize

\noindent The vector ${^{k+1}}\boldsymbol{\lambda}_i$ is the Lagrange multiplier at iteration $k+1$ of the projection optimization. Additionally, $\textbf{F}$ and  $\textbf{e}_{i}$ present a constant matrix and vector which will be defined later. The $\textbf{h}$ is a closed-form analytical function. The primary computational challenge associated with projection optimization arises from solving the \gls{qp} \eqref{fixed_point_1}. However, due to the absence of inequality constraints in \eqref{fixed_point_2}, the \gls{qp} simplifies to an affine transformation, taking the following form:

\vspace{-0.48cm}
\small
\begin{subequations}
    \begin{align}
({^{k+1}}\overline{\boldsymbol{\xi}}_{i}, {^{k+1}}\boldsymbol{\nu}_i) = \textbf{M}\boldsymbol{\eta}({^k} \overline{\boldsymbol{\xi}}_{i}),
    \label{affine_trans} \\
    \textbf{M} \hspace{-0.1cm}= \hspace{-0.1cm}\begin{bmatrix}
        \textbf{I}+\rho\textbf{F}^T\textbf{F} & \textbf{A}^{T} \\ 
        \textbf{A} & \textbf{0}
    \end{bmatrix}^{-1}\hspace{-0.2cm}, \boldsymbol{\eta} = \begin{bmatrix}
        -\rho\textbf{F}^T {^{k+1}}\textbf{e}_i+{^{k+1}}\boldsymbol{\lambda}_i+\boldsymbol{\xi}_i\\
        \textbf{b}_{eq}
    \end{bmatrix} \label{matrix_vec}
\end{align}
\end{subequations}
\normalsize

\vspace{-0.13cm}
\noindent where $\boldsymbol{\nu}_i$ presents the dual variables regarding with the equality constraints. 

\begin{proof}
    \noindent\textbf{Reformulated constraints:}
     Considering the same motivation as Section \ref{main_result_1}, we reformulate the collision avoidance and boundary inequality constraints, \eqref{affine_ineq_priest} \eqref{coll_multiagent_priest}, $\textbf{f}{_{o,j}}=0$, $\textbf{f}{_{v}}=0$ and $\textbf{f}{_{a}}=0$ as follows

\vspace{-0.3cm}
\small
\begin{subequations} 
\begin{align}
\hspace{-0.2cm}\colorbox{my_green}{$\textbf{f}_{o,j}=\hspace{-0.1cm}
\left \{ \begin{array}{lcr}
x(t)-x_{o,j}(t)-ad_{o,j}(t)\cos{\alpha_{o,j}}(t)\sin{\beta_{o,j}}(t) \\
y(t)-y_{o,j}(t)-bd_{o,j}(t)\sin{\alpha_{o,j}(t)}\sin{\beta_{o,j}}(t)\\
z(t)-z_{o,j}(t)-bd_{o,j}(t)\cos{\beta_{o,j}}
\end{array} \hspace{-0.25cm} \right \}\hspace{-0.10cm} $},  d_{o,j}(t) \geq 1, 
\label{collision_priest} \\
 \colorbox{my_pink}{$ \textbf{f}_{v} =\left \{ \hspace{-0.20cm} \begin{array}{lcr}
 \dot{x}(t) - d_{v}(t)v_{max}\cos{\alpha_{v}(t)}\sin{\beta_{v}(t)}  \\
 \dot{y}(t) - d_{v}(t)v_{max}\sin{\alpha_{v}(t)} \cos{\alpha_{v}(t)} \\
 \dot{z}(t) - d_{v}(t)v_{max}\cos{\beta_{v}(t)} 
\end{array} \hspace{-0.20cm} \right \} $}
,d_{v}(t) \leq 1 , ~  \forall t \label{fv_priest} \\
\colorbox{my_blue}{$ \textbf{f}_{a} = \left \{ \begin{array}{lcr}
\ddot{x}(t) - d_{a}(t)a_{max}\cos{\alpha_{a}(t)}\sin{\beta_{a}(t)} \\
\ddot{y}(t) - d_{a}(t)a_{max}\sin{\alpha_{a}(t)}\sin{\beta_{a}(t)}\\
\ddot{z}(t) - d_{a}(t)a_{max}\cos{\beta_{a}(t)} 
\end{array} \hspace{-0.20cm} \right \}$},  d_{a}(t) \leq 1 , ~\forall t \label{fa_priest}
\end{align}
\end{subequations}
 \normalsize
 
 \noindent where variables $d_{o,j}(t),\alpha_{o,j}(t),\beta_{o,j}(t),d_{v}(t),d_{a}(t),\alpha_{v}(t),\alpha_{a}(t)$, $\beta_{a}(t)$ and $\beta_{v}(t)$ are additional variables which will be computed along the projection part.

 \noindent \textbf{Reformulated Problem:} Now, we leverage \eqref{collision_priest}-\eqref{fa_priest} and rewrite the projection problem \eqref{projection_cost}-\eqref{projection_const} as

\vspace{-0.4cm}
\small
\begin{subequations}
\begin{align} \overline{\boldsymbol{{\xi}}}_{i} = \arg\min_{\overline{\boldsymbol{\xi}}_{i}} \frac{1}{2}\Vert \overline{\boldsymbol{\xi}}_{i}-\boldsymbol{\xi}_i\Vert_2^2 \label{cost_modify} \\
    \textbf{A}\overline{\boldsymbol{\xi}}_{i} = \textbf{b}_{eq}, \label{eq_modify_our}\\
   \Tilde{\textbf{F}}\overline{\boldsymbol{{\xi}}}_{i} = 
   \Tilde{\textbf{e}}(\boldsymbol{\alpha}_{i}, \boldsymbol{\beta}_{i}, \textbf{d}_{i})\label{reform_bound},\\
 \textbf{d}_{min} \leq \textbf{d}_{i}\leq \textbf{d}_{max}, \label{ine_1} \\
 \textbf{G}\overline{\boldsymbol{\xi}}_{i} \leq \boldsymbol{\tau} \label{bound_con}
\end{align}
\end{subequations}
\normalsize

\vspace{-0.2cm}
\noindent where $\hspace{-0.05cm}\boldsymbol{\alpha}_{i}, \boldsymbol{\beta}_{i}$ and $\hspace{-0.03cm}\textbf{d}_{i}$ are the representation of \hspace{-0.2cm}$\begin{bmatrix}
      \boldsymbol{\alpha}_{o,i}^{T} &\hspace{-0.28cm}\boldsymbol{\alpha}_{v,i}^{T}&\hspace{-0.28cm}
      \boldsymbol{\alpha}_{a,i}^{T} 
  \end{bmatrix}^{T}\hspace{-0.22cm},\hspace{-0.1cm}\begin{bmatrix}
      \boldsymbol{\beta}_{o,i}^{T} &\hspace{-0.28cm}\boldsymbol{\beta}_{v,i}^{T} &
    \hspace{-0.28cm}  \boldsymbol{\beta}_{a,i}^{T} \hspace{-0.28cm}
  \end{bmatrix}^{T}\hspace{-0.3cm}$ and $
     \begin{bmatrix}
     \textbf{d}^{T}_{o,i}&\hspace{-0.2cm}
     \textbf{d}^{T}_{v,i} &\hspace{-0.2cm} \textbf{d}^{T}_{a,i}
  \end{bmatrix}^{T}$\hspace{-0.1cm} respectively. The constant vector $\boldsymbol{\tau}$ is formed by stacking the $s_{min}$ and $s_{max}$ in appropriate form. The matrix $\textbf{G}$ is formed by stacking $ -\bold{P}$ and $\bold{P}$ vertically. Similarly, $\textbf{d}_{min}$, $\textbf{d}_{max}$ are formed by stacking the lower ($[1, 0, 0]$), and upper bounds ($[\infty, 1, 1]$) of $\textbf{d}_{o,i}, \textbf{d}_{v,i}, \textbf{d}_{a,i}$. Also, $ \Tilde{\textbf{F}}$, and $\textbf{e}$ are formed as

\vspace{-0.3cm}
  \small
  \begin{align}
      \tilde{\textbf{F}}\hspace{-0.10cm} =\hspace{-0.15cm} \begin{bmatrix}
        \begin{bmatrix}
       \colorbox{my_green}{$ \textbf{F}_{o}$} \\
       \colorbox{my_pink}{$ \dot{\bold{P}}$} \\
        \colorbox{my_blue}{$\ddot{\bold{P}}$}
    \end{bmatrix} \hspace{-0.25cm}&\hspace{-0.25cm} \textbf{0} \hspace{-0.25cm}&\hspace{-0.25cm} \textbf{0} \\ \textbf{0}\hspace{-0.25cm} & \hspace{-0.25cm}\hspace{-0.15cm}\begin{bmatrix}
       \colorbox{my_green}{$ \textbf{F}_{o} $}\\
        \colorbox{my_pink}{$\dot{\bold{P}} $}\\
        \colorbox{my_blue}{$\ddot{\bold{P}}$}
    \end{bmatrix} \hspace{-0.25cm}& \hspace{-0.25cm} \textbf{0}\\
         \textbf{0}\hspace{-0.25cm}& \hspace{-0.25cm}\textbf{0} \hspace{-0.25cm}&\hspace{-0.25cm} \begin{bmatrix}
        \colorbox{my_green}{$\textbf{F}_{o}$} \\
        \colorbox{my_pink}{$\dot{\bold{P}}$} \\
       \colorbox{my_blue}{$ \ddot{\bold{P}}$}
    \end{bmatrix}
    \end{bmatrix}\hspace{-0.15cm}, \hspace{-0.05cm}
    \Tilde{\textbf{e}} \hspace{-0.1cm}= \hspace{-0.15cm}\begin{bmatrix}
       \colorbox{my_green}{$ \textbf{x}_{o} +
      a\textbf{d}_{o,i}\cos{ \boldsymbol{\alpha}_{o,i}} \sin{ \boldsymbol{\beta}_{o,i}}$} \\ \colorbox{my_pink}{$\textbf{d}_{v,i}v_{max}\cos{\boldsymbol{\alpha}_{v,i}}\sin{\boldsymbol{\beta}_{v,i}}$} \\
\colorbox{my_blue}{$\textbf{d}_{a,i}a_{max}\cos{\boldsymbol{\alpha}_{a,i}}\sin{\boldsymbol{\beta}_{a,i}}$}\\
       \colorbox{my_green}{$ \textbf{y}_{o} +
      a\textbf{d}_{o,i}\sin{ \boldsymbol{\alpha}_{o,i}} \sin{ \boldsymbol{\beta}_{o,i}}$} \\
\colorbox{my_pink}{$\textbf{d}_{v,i}v_{max}\sin{\boldsymbol{\alpha}_{v,i}}\sin{\boldsymbol{\beta}_{v,i}}$}\\
\colorbox{my_blue}{$\textbf{d}_{a,i}a_{max}\sin{\boldsymbol{\alpha}_{a,i}}\sin{\boldsymbol{\beta}_{a,i}}$}\\
     \colorbox{my_green}{$ \textbf{z}_{o} +
      b\hspace{0.1cm} \textbf{d}_{o,i}\cos{ \boldsymbol{\beta}_{o,i}}$} \\
\colorbox{my_pink}{$\textbf{d}_{v,i}v_{max}\cos{\boldsymbol{\beta}_{v,i}}$}\\
\colorbox{my_blue}{$\textbf{d}_{a,i}a_{max}\cos{\boldsymbol{\beta}_{a,i}}$}
    \end{bmatrix}\hspace{-0.15cm},\label{f_e}
  \end{align} 
  \normalsize

\noindent where $\textbf{F}_{o}$ is formed by stacking as many times as the number of obstacles. Also, $\textbf{x}_{o}, \textbf{y}_{o}, \textbf{z}_{o}$ is obtained by stacking $x_{o,j}(t),y_{o,j}(t), z_{o,j}(t)$ at different time stamps and for all obstacles. 

\noindent \textbf{Solution Process:}
we relax the equality and affine constraints \eqref{reform_bound}-\eqref{bound_con} as $l_{2}$ penalties utilizing the augmented Lagrangian method

\vspace{-0.3cm}
\small
\begin{align}
\hspace{-0.20cm}\mathcal{L}\hspace{-0.1cm}=\hspace{-0.1cm}\frac{1}{2}\hspace{-0.1cm}\left\Vert \overline{\boldsymbol{\xi}}_{i}\hspace{-0.1cm} - \hspace{-0.1cm}\boldsymbol{\xi}_{i}\right\Vert ^{2}_{2}\hspace{-0.1cm}- \hspace{-0.13cm}\langle\boldsymbol{\lambda}_{i}, \overline{\boldsymbol{\xi}}_{i}\rangle \hspace{-0.1cm}
 +\hspace{-0.1cm}\frac{\rho}{2}\left\Vert \Tilde{\textbf{F}}\overline{\boldsymbol{\xi}}_{i}  
 \hspace{-0.15cm}-\Tilde{\textbf{e}} \right \Vert_2^2 
 \hspace{-0.1cm}+\hspace{-0.1cm}\frac{\rho}{2}\left\Vert \textbf{G}\overline{\boldsymbol{\xi}}_{i}  
 \hspace{-0.15cm}-\boldsymbol{\tau}+\hspace{-0.08cm}\textbf{s}_{i} \right \Vert_2^2 , \nonumber \\
 =\hspace{-0.1cm} \frac{1}{2}\left\Vert \overline{\boldsymbol{\xi}}_{i} - \boldsymbol{\xi}_{i}\right\Vert ^{2}_{2}\hspace{-0.1cm}- \hspace{-0.1cm}\langle\boldsymbol{\lambda}_{i}, \overline{\boldsymbol{\xi}}_{i}\rangle \hspace{-0.1cm}
 +\hspace{-0.1cm}\frac{\rho}{2}\left\Vert \textbf{F}\overline{\boldsymbol{\xi}}_{i}  
 \hspace{-0.15cm}-\textbf{e} \right \Vert_2^2 
 \label{lagrange} 
 \end{align}
\normalsize

\noindent where,
$\hspace{-0.05cm}\textbf{F} = \hspace{-0.1cm}\begin{bmatrix}
    \Tilde{\textbf{F}} \\ \textbf{G}
\end{bmatrix}\hspace{-0.1cm},
\textbf{e} =\hspace{-0.1cm}\begin{bmatrix}
   \Tilde{\textbf{e}} \\ \boldsymbol{\tau}\hspace{-0.1cm}-\textbf{s}_{i}
\end{bmatrix}$. Also, $\boldsymbol{\lambda}_{i}$, $\rho$ and $\textbf{s}_{i}$ are Lagrange multiplier, scalar constant and slack variable. We reduce the problem \eqref{lagrange} subject to \eqref{eq_modify_our} using \gls{am} method as follows

\vspace{-0.3cm}
\small
\begin{subequations}
\begin{align}
    ^{k+1}\boldsymbol{\alpha}_{i} = \text{arg} \min_{\boldsymbol{\alpha}_{i}}\mathcal{L}(^{k}\overline{\boldsymbol{\xi}}_{i}, \boldsymbol{\alpha}_{i}, \hspace{0.1cm}^{k}\boldsymbol{\beta}_{i}, \hspace{0.1cm}^{k}\textbf{d}_{i}, \hspace{0.1cm}^{k}\boldsymbol{\lambda}_{i},
    \hspace{0.1cm}^{k}\textbf{s}_{i} ) \label{comp_alpha} \\
    ^{k+1}\boldsymbol{\beta}_{i} = \text{arg} \min_{\boldsymbol{\beta}_{i}}\mathcal{L}(^{k}\overline{\boldsymbol{\xi}}_{i}, \hspace{0.1cm}^{k+1}\boldsymbol{\alpha}_{i}, \boldsymbol{\beta}_{i}, \hspace{0.1cm}^{k}\textbf{d}_{i}, \hspace{0.1cm}^{k}\boldsymbol{\lambda}_{i},
    \hspace{0.1cm}^{k}\textbf{s}_{i} ) \label{comp_beta}\\
    ^{k+1}\textbf{d}_{i} = \text{arg} \min_{\textbf{d}_{i}}\mathcal{L}(\hspace{0.1cm}^{k}\overline{\boldsymbol{\xi}}_{i}, \hspace{0.1cm}^{k+1}\boldsymbol{\alpha}_{i}, \hspace{0.1cm}^{k+1}\boldsymbol{\beta}_{i},\textbf{d}_{i}, \hspace{0.1cm}^{k}\boldsymbol{\lambda}_{i},
    \hspace{0.1cm}^{k}\textbf{s}_{i} )\label{comp_d}\\
     ^{k+1}\textbf{s}_{i} = \max (\textbf{0}, -\textbf{G}\hspace{0.1cm}^{k}\overline{\boldsymbol{\xi}}_{i}+ \boldsymbol{\tau})\\
    \hspace{0.1cm}^{k+1}\boldsymbol{\lambda}_{i} = ^{k}\boldsymbol{\lambda}_{i}
- \rho \textbf{F}^{T}(\textbf{F}\hspace{0.1cm} ^{k}\overline{\boldsymbol{\xi}}_{i} 
 -^{k}\Tilde{\textbf{e}})\label{lag} \\
     ^{k+1}\textbf{e}=
     \begin{bmatrix}
        \Tilde{\textbf{e}}(\hspace{0.1cm}^{k+1}\boldsymbol{\alpha}_{i},^{k+1}\boldsymbol{\beta}_{i}, ^{k+1}\textbf{d}_{i}) \label{obtain_e}\\
    \boldsymbol{\tau} -^{k+1}\textbf{s}_{i}\end{bmatrix}\\
  ^{k+1}\overline{\boldsymbol{\xi}}_{i} = \text{arg} \min_{\overline{\boldsymbol{\xi}}_{i}}\mathcal{L}({\boldsymbol{\xi}}_{i}, {^{k+1}}\textbf{e}_i,  ^{k+1}\boldsymbol{\lambda}_{i},
) \label{comp_zeta}
\end{align}
\end{subequations}
\normalsize
\vspace{-0.2cm}

\noindent where that stacking of right-hand sides of \eqref{obtain_e} and \eqref{lag} provide the function $\textbf{h}$ presented~in \eqref{fixed_point_1} and  \eqref{comp_zeta} is a representation of \eqref{proj_cost}-\eqref{reform_bound_p}. Also, the steps \eqref{comp_alpha}-\eqref{comp_d} have closed form solutions in terms of ${^k}\overline{\boldsymbol{\xi}}_i$ (see analysis of Alg. \ref{alg_1} and Alg. \ref{alg_2} in Sections \ref{main_result_1} and \ref{main_results_2}). Note that for each \gls{am} step, we only optimize one group of variables while others are held fixed. 
\end{proof}

\noindent \textbf{GPU Accelerated Batch Operation:} Our method involves projecting multiple sampled trajectories onto the feasible set (see Fig.\ref{fig_overview}). However, as it mentioned before, performing these projections sequentially can be computationally burdensome. Fortunately, our projection optimizer exhibits certain structures conducive to batch and parallelized operations. 
To delve into this concept, consider the matrix $\textbf{M}$ in \eqref{affine_trans}, which remains constant regardless of the input trajectory sample $\boldsymbol{\xi}_{i}$. In essence, $\textbf{M}$ remains unchanged irrespective of the specific trajectory sample requiring projection onto the feasible set. This characteristic enables us to express the solution \eqref{affine_trans} for all trajectory samples $\boldsymbol{\xi}_{i}, i = 1,2,\dots,N_b$ as a single large matrix-vector product. This computation can be effortlessly parallelized across GPUs.
Similarly, acceleration is attainable for the function $\textbf{h}$, which primarily involves element-wise products and sums. This allows for efficient parallelization and leveraging GPU capabilities to enhance overall performance.

\noindent \textbf{Scalability:} The matrix $\textbf{M}$ in \eqref{affine_trans} requires a one-time computation, as $\textbf{A}$ and $\textbf{F}$ remain constant throughout the projection iteration. Conversely, the matrix $\boldsymbol{\eta}$ is recalculated at each iteration, with its computational cost primarily dominated by $\hspace{-0.05cm}\textbf{F}^{T}{^{k+1}}\textbf{e}_{i}$. The number of rows in both $\textbf{F}$ and $\textbf{e}$ increases linearly with the planning horizon, the number of obstacles, or the batch size (see Remark \ref{matrix_scaling}). This characteristic, in conjunction with GPU acceleration, endows our approach with remarkable scalability for long-horizon planning in highly cluttered environments.
Fig.\ref{comp_time} presents the average per-iteration time of the projection optimizer. It also demonstrates how it scales with the number of obstacles and batch size. 

\begin{figure}[!h]
% \vspace{-0.10cm}
    \centering
        \includegraphics[scale=0.42]{figures/fig_46.png}
        \vspace{-0.2cm}
    \caption[PRIEST scalability]{Scalability of per-iteration computation time of our projection optimizer to number of obstacles and batch size}
    \label{comp_time}
\end{figure}

\subsubsection{Projection Guided Sampling-Based Optimizer}
\noindent\textbf{Algorithm Description:} Alg. \ref{alg_3} presents another core contribution of this paper. It starts by generating $N_{b}$ samples of polynomial coefficients $\boldsymbol{\xi}$ from a Gaussian distribution with $\mathcal{N}({^l}\boldsymbol{\mu},\hspace{-0.08cm}{^l}\boldsymbol{\Sigma})$ at iteration $l\hspace{-0.1cm}=\hspace{-0.1cm}0$ (line 3). The~sampled $\hspace{-0.05cm}\boldsymbol{\xi}_i\hspace{-0.09cm}$ is subsequently projected onto the feasible set (lines~4-5). Due to real-time constraints, it may not be impractical to execute the projection optimization long enough to push all the sampled trajectories to feasibility. Thus, in line 6, we compute the constraint residuals $r(\overline{\boldsymbol{\xi}}_{i})$ associated with each sample. In line 7, we select the top $N_{proj}$ samples with the least constraint residuals and append them to the list $ConstraintEliteSet$. Lines 8-9 involve the creation of an augmented cost, $c_{aug}$, achieved by appending the residuals to the primary cost function. Subsequently, $c_{aug}$ is evaluated on the samples from $ConstraintEliteSet$.
In line 11, we once again select the top $N_{elite}$ samples with the lowest $c_{aug}$ and append them to the list $EliteSet$. Finally, moving to line 12, we update the distribution based on the samples of the $EliteSet$ and the associated $c_{aug}$ values. The final output of the optimizer is the sample from the $EliteSet$ with the lowest $c_{aug}$.

\vspace{-0.47cm}
 \small
    \begin{subequations}
        \begin{align}
         ^{l+1}\boldsymbol{\mu} = (1-\sigma)\hspace{0.1cm} ^{l}\boldsymbol{\mu} +\hspace{-0.05cm} \sigma (\frac{1}{\sum\limits_{m \in C} c_{m}})
         \sum\limits_{m\in C}\overline{\boldsymbol{\xi}}_{m} c_{m}, \label{update_mean} \\
        \hspace{-0.27cm}^{l+1} \boldsymbol{\Sigma}\hspace{-0.1cm} = \hspace{-0.1cm}(1\hspace{-0.1cm}-\hspace{-0.1cm}\sigma)  \hspace{0.05cm}^{l}\boldsymbol{\Sigma} \hspace{-0.1cm}+ \hspace{-0.1cm} \sigma \frac{\sum\limits_{m \in C} c_{m}(\overline{\boldsymbol{\xi}}_{m}-^{~l+1}\boldsymbol{\mu})(\overline{\boldsymbol{\xi}}_{m}-^{~l+1}\boldsymbol{\mu})^{T}}{\sum\limits_{m \in C} c_{m}}, 
         \label{update_covariance} \\
          c_{m} = \exp\big({\gamma^{-1}(c_{aug}(\overline{\boldsymbol{\xi}}_{m}) - \delta )}\big),
        \end{align}
    \end{subequations}
    \normalsize

\vspace{-0.15cm}
\noindent where the scalar constant $\sigma$ is the so-called learning rate. The set $C$ consists of the top $N_{elite}$ selected trajectories (line 11). The constant $\gamma$ specifies the sensitivity of the exponentiated cost function $c_{aug}(\overline{\boldsymbol{\xi}}_{m})$ for top selected trajectories. $\delta = \min c_{aug}(^{l}\overline{\boldsymbol{\xi}}_{m})$ is defined to prevent numerical instability. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\scriptsize
\DontPrintSemicolon
\SetAlgoLined
\SetNoFillComment
\caption{\scriptsize Projection Guided Sampling-Based Optimization (PRIEST) }\label{alg_3}
\KwInput{Initial states}
\KwInitialization{Initiate $^{l}\boldsymbol{\mu}$ and $^{l}\boldsymbol{\Sigma} $ at $i=0$}
\For{$l \leq N$}{
\hspace{-0.15cm}Initialize $CostList = []$
    
\hspace{-0.15cm}Draw $N_{b}$ samples $\boldsymbol{\xi}_{1},...,\boldsymbol{\xi}_{N_{b}}$ from $\mathcal{N}(^{l}\boldsymbol{\mu},^{l}\boldsymbol{\Sigma})$\tcp*[l]{Generating samples from a Gaussian distribution}
   
\hspace{-0.15cm}Solve the inner convex optimizer to obtain $\overline{\boldsymbol{\xi}}_{i}$\tcp*[l]{Pushing the samples into feasible trajectory space}
    \begin{subequations}
        \begin{align}
            \min_{\overline{\boldsymbol{{\xi}}}_{i}} \frac{1}{2} \left\Vert \overline{\boldsymbol{\xi}}_{i} - \boldsymbol{\xi}_{i}  \right\Vert ^{2}_{2},  
            \label{proj_cost} \\
        \bold{A}\overline{\boldsymbol{\xi}}_{i}= \bold{b}_{eq}\label{eq_modify_p} \\
            \textbf{g}(\overline{\boldsymbol{\xi}}_{i}) \leq \textbf{0} \label{reform_bound_p},
        \end{align}
    \end{subequations}

    % Compute $\textbf{u}_i=\boldsymbol{\Phi}(\overline{\boldsymbol{\xi}}_{i})$
    \vspace{-0.15cm}
   \hspace{-0.15cm} Compute the residuals set $r(\overline{\boldsymbol{\xi}}_{i})$ \hspace{-0.2cm}\tcp*[l]{\hspace{-0.1cm}getting residuals to know how well the constraints are satisfied}
   
\hspace{-0.15cm} $ConstraintEliteSet\leftarrow$   Select $N_{proj}$ samples from $r(\overline{\boldsymbol{\xi}}_{i})$ with the lowest values. \tcp*[l]{Select top samples with the lowest residuals}
    
\hspace{-0.15cm}Evaluate the cost
    
    $c_{aug} \leftarrow  c_1(\overline{\boldsymbol{\xi}}_{i})+ r(\overline{\boldsymbol{\xi}}_{i})$
    \tcp*[l]{Cost evaluatio}
    Append $cost$ to the $CostList$
    
   $EliteSet \leftarrow$  Select $N_{elite}$ top samples with the lowest cost obtained from the $CostList$.
   \hspace{-0.2cm}\tcp*[l]{\hspace{-0.10cm}Select top samples which influence sampling distribution}
    
    Update the new mean and covariance, $^{l+1}\boldsymbol{\mu}$~and~$^{l+1}\boldsymbol{\Sigma}$, using \eqref{update_mean}-\eqref{update_covariance}
    \tcp*[l]{Update mean and covariance based on the top samples}
}
\hspace{-0.07cm}\textbf{Return} \hspace{-0.06cm}$\overline{\boldsymbol{\xi}}_{i}$\hspace{-0.09cm} corresponding to the lowest cost in \hspace{-0.06cm}$\small EliteSet \normalsize$
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation and Benchmarking}

\noindent \textbf{Implementation Details} We implemented Algorithm \ref{alg_3}, \gls{priest}, using Python with the JAX \cite{bradbury2018jax} library as the GPU-accelerated algebra backend. Our simulation framework for experiments was developed on the ROS \cite{koubaa2017robot} platform, utilizing the Gazebo physics simulator. All benchmarks were conducted on a Legion7 Lenovo laptop featuring an Intel Core i7 processor and an Nvidia RTX 2070 GPU. We employed the open3d library for downsampling PointCloud data \cite{zhou2018open3d}.
We selected $t_{f}\hspace{-0.1cm}=\hspace{-0.1cm}10,N \hspace{-0.1cm}=\hspace{-0.1cm}13,N_{b}\hspace{-0.1cm}=\hspace{-0.1cm}110$, $N_{proj}\hspace{-0.1cm}=\hspace{-0.1cm}80$ and $N_{elite}\hspace{-0.1cm}=\hspace{-0.1cm}20$. All the compared baselines operated with the same planning horizon. Furthermore, to provide the best possible opportunity for \gls{mppi} and log-MPPI, they were executed with their default sample size of 2496, which is over 20 times higher than that utilized by \gls{priest}. The benchmarking against other baselines is based on the following metrics:

\begin{itemize}
    \item \textbf{Success Rate}: A run is considered successful when the robot approaches the final point within a 0.5m radius without any collision. The success rate is calculated as the ratio of the total number of successful runs to the overall number of runs.
     \item \textbf{Travel Time}: This metric represents the duration it takes for the robot to reach the vicinity of the goal point.
     \item \textbf{Computation Time}: This metric quantifies the time required to calculate a solution trajectory.
\end{itemize}

Furthermore, we compared our approach with different baselines in four sets of benchmarks, including:

\begin{itemize}
    \item \textbf{Comparison on \gls{barn} Dataset \cite{perille2020benchmarking}:}
    In this benchmark, we used a holonomic mobile robot modeled as a double-integrator system. The robot is tasked with iteratively planning its trajectory through an obstacle field in a receding horizon manner. Consequently, the differential flatness function for extracting control inputs was defined as $\boldsymbol{\Phi} = (\ddot{x}(t),\ddot{y}(t))$. The cost function ($c_1$) took the following form:

\small
\begin{align}
    \sum_t{\ddot{x}(t)^2+\ddot{y}(t)^2+c_{\kappa}+c_{p}}
    \label{barn_cost}
\end{align}
\normalsize

\noindent where $c_{\kappa}=(\frac{\ddot{y}(t)\dot{x}(t)-\ddot{x}(t)\dot{y}(t) }{(\dot{x}(t)^2+\dot{x}(t)^2)^{1.5}})^2$ penalizing curvature, $c_{p}$ minimizes the orthogonal distance of the computed trajectory from a desired straight-line path to the goal. It is important to note that $c_{p}$ does not have an analytical form as it necessitates the computation of the projection of a sampled trajectory waypoint onto the desired path.
We utilized the \gls{barn} dataset, consisting of 300 environments with varying complexity, designed to create local-minima traps for the robot. The evaluation involves comparing our approach against \gls{dwa} \cite{fox1997dynamic}, \gls{teb} \cite{rosmann2017kinodynamic} implemented in the \gls{ros} navigation stack, \gls{mppi} \cite{williams2017model}, and log-MPPI \cite{mohamed2022autonomous}. All baselines, including \gls{priest}, had access only to the local cost map or point cloud. \gls{teb} and \gls{dwa} employed a combination of graph search and optimization, while \gls{priest} and log-MPPI were purely optimization-based approaches. 

\item \textbf{Point to Point Navigation with Differentiable Cost:} 
In this benchmark, our aim is to generate a single trajectory between a start and a goal location. The cost function  $c_1$ incorporates the first term of \eqref{barn_cost}. For comparison, we considered \gls{sota} gradient-based optimizers ROCKIT \cite{metz2003rockit} and \gls{fatrop} \cite{vanroye2023fatrop} and sampling-based optimizers \gls{cem}, and \gls{vpsto} \cite{jankowski2023vp}.

\item \textbf{Comparison in a Dynamic Environment:} In this evaluation, we benchmark against \gls{cem}, log-MPPI, \gls{mppi}, \gls{teb} and \gls{dwa}, employing the same cost function as used for \gls{barn} Dataset \eqref{barn_cost}. In this dynamic scenario, we introduced ten obstacles, each with a velocity of $0.1m/s$, moving in the opposite direction of the robot. Simulations were conducted across 30 distinct obstacle configurations and velocities. The robot model used for this benchmark is a nonholonomic mobile robot known as Jackal.

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Qualitative Results}

\subsubsection{A Simple Benchmark}
Fig. \ref{fig_teaser} presents a comparison of the behaviors of \gls{cem} and \gls{priest} in a scenario wherein all the initial sampled trajectories lie within a high-cost/infeasible region. The results clearly demonstrate that while \gls{cem} samples persistently remain in the infeasible region, \gls{priest} samples move toward the out-of-infeasible region. Additionally, Fig. \ref{fig_teaser} (g-h) empirically validates Alg. \ref{alg_3} by illustrating the gradual reduction and saturation of both constraint residuals and cost values as the iterations progress. The projection optimizer is essentially a set of analytical transformations over the sampled trajectories. Thus, Alg.\ref{alg_3} retains the convergence properties of the base sampling-based optimizer upon which the projection part is embedded. For example, it will~inherit the properties of CEM when integrated with \gls{cem}-like a sampler. Moreover, the projection optimizer by construction satisfies the boundary constraints on the trajectories and ensures a reduction in the cost by pushing the samples toward the feasible region.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsubsection{Receding Horizon Planning on \gls{barn} Dataset} 

In Fig. \ref{methods_traj}, we show trajectories generated by \gls{priest} at three different snapshots within one of the \gls{barn} environments. These trajectories are compared with those produced by \gls{mppi}, \gls{teb}, \gls{dwa}, and log-MPPI in the same environment. As can be seen in Fig. \ref{methods_traj}(e), \gls{priest} successfully generated collision-free trajectories while other methods faced challenges and got stuck (see the bottom row of Fig. \ref{methods_traj}(a)-(d). Furthermore, to illustrate the exploration of various homotopies at each iteration, we compare the behavior of \gls{priest} with \gls{teb} in one of the \gls{barn} environments in Fig. \ref{qual_homo}. While \gls{teb} employs graph search, \gls{priest} leverages the stochasticity inherent in the sampling process, guided by the projection optimizer. Consequently, \gls{priest} can explore over a more extended horizon and a broader state space. It's noteworthy that increasing the planning horizon of \gls{teb} significantly raises computation time, potentially degrading overall navigation performance rather than enhancing it. We provide a quantitative comparison with \gls{teb} and other baselines in the next subsection.

\begin{figure}[!h]
    \includegraphics[scale=0.5]{figures/methods_traj.png}
    \vspace{-0.7cm}
    \caption[Comparative visualization of qualitative results from MPC built on MPPI, log-MPPI, TEB, DWA, and PRIEST]{\small{Comparative visualization of qualitative results from \gls{mpc} built on \gls{mppi} (a), log-MPPI(b), \gls{teb}(c), \gls{dwa}(d), and \gls{priest}(e). We showed the best trajectory obtained from each optimizer at three distinct snapshots.}}
    \label{methods_traj}
    \end{figure}
    
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.90]{figures/homotopy.png}
    \vspace{-0.2cm}
    \caption[Qualitative result of MPC built on PRIEST and TEB]{\small{Qualitative result of MPC built on \gls{priest} (a-b) and \gls{teb} (c-d). Blue and purple trajectories show top samples in the PRIEST and TEB planner. }}
    \label{qual_homo}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\subsubsection{Point-to-Point Navigation Benchmark} 
Fig. \ref{traj_plot} illustrates trajectories generated by \gls{priest}, as well as those produced by gradient-based optimizers ROCKIT and \gls{fatrop}, and sampling-based optimizers \gls{cem} and \gls{vpsto}. In the specific 2D example presented, both \gls{priest} and \gls{vpsto} successfully generated collision-free trajectories, surpassing the performance of other baselines. In the showcased 3D environment, only \gls{priest} and \gls{cem} achieved collision-free trajectories. In the next subsection, we present the quantitative statistical trends for all the baselines across different randomly generated environments.

\begin{figure}[!h]
    \centering
        \includegraphics[scale=0.71]{figures/qual_4.png}
    \caption[Qualitative result of point-to-point navigation.]{\small{Qualitative result of point-to-point navigation. Trajectories for different approaches have the same color in both 2D and 3D configurations.} }
    \label{traj_plot}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Decenteralized Variant}
Fig.\ref{com_plot} shows the application of D-PRIEST for car-like vehicle trajectory planning. The cost function $c_1$ penalizes the magnitude of axis-wise accelerations and steering angle. Leveraging the differential flatness property, we express the steering angle as a function of axis-wise velocity and acceleration terms \cite{han2023efficient}. In Fig.\ref{com_plot}, D-PRIEST demonstrates three different distributions (depicted in green, red, and blue) in parallel, resulting in multi-modal behaviors. These maneuvers intuitively correspond to overtaking static obstacles (depicted in black) from left to right or slowing down and shifting to another lane. In contrast, traditional \gls{cem} could only obtain a single maneuver for the vehicle.

\begin{figure}[!h]
\centering
    \includegraphics[scale=0.55]{figures/comparison_2.png}
    \caption[Comparison of D-PRIEST with baseline cem]{\small{Comparison of D-PRIEST with baseline \gls{cem}. As is shown, the former updates multiple parallel distributions, resulting in multi-modal optimal trajectory distribution upon convergence. D-PRIEST maintained three different distributions (shown in green, red, and blue) and thus could obtain multi-modal behavior. In contrast, \gls{cem}, which only has a single distribution, provides a limited set of options for collision-free trajectories.}}
    \label{com_plot}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Quantiative Results}

\begin{enumerate}[label=\alph*)]
  \item \textit{Comparison with \gls{mppi}, Log-MPPI, \gls{teb}, \gls{dwa}:} Table 1 summarizes the quantitative results. \gls{priest} achieves a 90\% success rate, outperforming the best baseline (\gls{teb}) with an 83\% success rate. \gls{teb}, along with \gls{dwa}, employs graph search and complex recovery maneuvers to improve success rates, albeit with increased travel time. Conversely, purely optimization-based approaches \gls{mppi} and log-MPPI exhibit a 32\% and 35\% lower success rate than PRIEST, accompanied by slightly higher travel times. Although \gls{priest} shows a slightly higher mean computation time, it remains fast enough for real-time applications.
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h] 
\small
\caption{Comparisons on the \gls{barn} 
Dataset}\label{Barn}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
                             Method    & \cellcolor[HTML]{009901}\begin{tabular}[c]{@{}c@{}}Success\\  rate\end{tabular} & \cellcolor[HTML]{009901}\begin{tabular}[c]{@{}c@{}}Travel time (s)\\    Mean/ Min/Max\end{tabular}  & \cellcolor[HTML]{009901}\begin{tabular}[c]{@{}c@{}}Computation time (s)\\ Mean/ Min/Max\end{tabular} \\ \hline
\cellcolor[HTML]{3166FF}DWA      & 76\%                                                                          & \begin{tabular}[c]{@{}c@{}}52.07/ 33.08/145.79\end{tabular}                                                                   & \begin{tabular}[c]{@{}c@{}}0.037/ 0.035/0.04\end{tabular}                                            \\ \hline
\cellcolor[HTML]{3166FF}TEB      & 83\%                                                                          & \begin{tabular}[c]{@{}c@{}}52.34/ 42.25/106.32\end{tabular}                                                                        & \begin{tabular}[c]{@{}c@{}}0.039/0.035/0.04\end{tabular}                                            \\ \hline
\cellcolor[HTML]{3166FF}MPPI     & 58\%                                                                            & \begin{tabular}[c]{@{}c@{}}36.66/ 31.15/99.62\end{tabular}                                                                         & \begin{tabular}[c]{@{}c@{}}0.019/0.018/0.02\end{tabular}                                            \\ \hline
\cellcolor[HTML]{3166FF}log-MPPI & 55\%                                                                            & \begin{tabular}[c]{@{}c@{}}36.27/30.36/58.84\end{tabular}                                                                          & \begin{tabular}[c]{@{}c@{}}0.019/0.018/0.02\end{tabular}                                            \\ \hline
\cellcolor[HTML]{3166FF}{\textbf{PRIEST}}   & \textbf{90\%}                                                                 & \begin{tabular}[c]{@{}c@{}}\textbf{33.59}/ 30.03/70.98\end{tabular}                                                                           & \begin{tabular}[c]{@{}c@{}}0.071/0.06/0.076\end{tabular}                                            \\ \hline
\end{tabular}
\normalsize
\end{table}
  \item \textit{Comparison with Additional Gradient-Based and Sampling-based Optimizers:} Table \ref{grad_based} compares the performance of \gls{priest} with all the baselines in 2D and 3D cluttered environments (see Fig.\ref{traj_plot}). ROCKIT and \gls{fatrop} were initialized with simple straight-line trajectories between the start and the goal, typically not collision-free. Due to conflicting gradients from neighboring obstacles, both methods often failed to obtain a collision-free trajectory. Interestingly, the sampling-based approaches didn't fare much better, as both \gls{cem} and \gls{vpsto} reported a large number of failures. We attribute the failures of \gls{vpsto} and \gls{cem} to two reasons. First, most of the sampled trajectories for both \gls{cem} and \gls{vpsto} fell into the high-cost/infeasible area, creating a pathologically difficult case for sampling-based optimizers. Second, both \gls{cem} and \gls{vpsto} roll constraints into the cost as penalties and can be sensitive to tuning the individual cost terms. In summary, Table \ref{grad_based} highlights the importance of PRIEST, which uses convex optimization to guide trajectory samples toward constraint satisfaction. 
  
  \gls{priest} also shows superior computation time than ROCKIT and \gls{fatrop}. The \gls{cem} run times are comparable to PRIEST. Although \gls{vpsto} numbers are high, we note that the original author implementation that we use may not have been optimized for computation speed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\vspace{-0.01cm}
\caption{Comparing \gls{priest} with Gradient/Sampling-Based Optimizers }
\small
\label{grad_based}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Method & Success rate  & \begin{tabular}[c]{@{}c@{}}Computation time (s) \color{black}(Mean/Min/Max)\end{tabular} \\ \hline
\rowcolor[HTML]{009901} 
ROCKIT-2D & 46\%          & 2.57/0.6/6.2                       \\ \hline
\rowcolor[HTML]{009901} 
FATROP-2D & 64\%          & 0.63/0.07/2.87                                                           \\ \hline
\rowcolor[HTML]{009901} 
\textbf{PRIEST-2D}   & \textbf{95\%} & \textbf{0.043/0.038/0.064}                            
\\ \hline
\rowcolor[HTML]{009901} 
CEM-2D   & 78\%         & 0.017/0.01/0.03                                                              \\ \hline
\rowcolor[HTML]{009901} 
VPSTO-2D & 66\%         & 1.63/0.78/4.5                                                                                      \\ \hline
\rowcolor[HTML]{EBC85D} 
ROCKIT-3D &      65\%     &      1.65/0.68/5                                                                            \\ \hline
\rowcolor[HTML]{EBC85D} 
FATROP-3D &    81\%      &    0.088/0.034/0.23                                                                    \\ \hline
\rowcolor[HTML]{EBC85D} 
\textbf{PRIEST-3D}  & \textbf{90\%} & \textbf{0.053/0.044/0.063}                                                       \\ \hline
\rowcolor[HTML]{EBC85D} 
CEM-3D   & 74\%         & 0.028/0.026/0.033                                      \\ \hline
\rowcolor[HTML]{EBC85D} 
VPSTO-3D & 37\%          & 3.5/0.93/3.5                                  \\ \hline
\end{tabular}
\normalsize
\end{table}
%%%%%%%%%%%%%%%%%%
  \item Combination of Gradient-Based and Sampling-based Optimizers: \noindent A simpler alternative to PRIEST can be just to use a sampling-based optimizer to compute a good guess for the gradient-based solvers \cite{kim2022mppi}. However, such an approach will only be suitable for problems with differentiable costs. Nevertheless, we evaluate this alternative for the point-to-point benchmark of Fig.\ref{traj_plot}. We used CEM to compute an initial guess for ROCKIT and FATROP. The results are summarized in Table \ref{sto_based}. As can be seen, while the performance of both ROCKIT and FATROP improved in 2D environments, the success rate of the latter decreased substantially in the 3D variant. The main reason for this conflicting trend is that the CEM (or any initial guess generation) is unaware of the exact capabilities of the downstream gradient-based optimizer.  This unreliability forms the core motivation behind PRIEST, which outperforms all ablations in Table \color{red}\ref{sto_based}\color{black}. By embedding the projection optimizer within the sampling process itself (refer Alg.\ref{algo1}) and augmenting the projection residual to the cost function, we ensure that the sampling and projection complement each other.
%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!h]
\caption{Comparing \gls{priest} with Hybrid Gradient-Sampling Baselines. }
\small
\centering
\label{sto_based}
\begin{tabular}{|c|c|c|c|}
\hline
Method   & Success rate & \begin{tabular}[c]{@{}c@{}}Computation time (s) \color{black} (Mean/Min/Max)\end{tabular}  \\ \hline
\rowcolor[HTML]{009901} 
ROCKIT-CEM & 94\%         & 2.07/0.69/6.0                                                         \\ \hline
\rowcolor[HTML]{009901} 
FATROP-CEM & 84\%          & 0.34/0.06/0.96   
\\ \hline
\rowcolor[HTML]{009901} 
\textbf{PRIEST-2D}\color{black}   & \textbf{95\%} & \textbf{0.043/0.038/0.064}                     
\\ \hline
\rowcolor[HTML]{EBC85D} 
ROCKIT-CEM & \textbf{100\%}          & 1.19/0.7/2.56                                             \\ \hline
\rowcolor[HTML]{EBC85D} 
FATROP-CEM & 25\%          & 0.056/0.039/0.079                                  \\ \hline
\rowcolor[HTML]{EBC85D} 
\textbf{PRIEST-3D}\color{black}   & 90\% & \textbf{0.053/0.044/0.063}                              \\ \hline                       
\end{tabular}
\normalsize
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Benchmarking in Dynamic Environments:
Table \ref{dynamic} presents the results obtained from the experiments in dynamic environments. Herein, the projection optimizer of PRIEST ensures collision constraint satisfaction with respect to the linear prediction of the obstacles' motions. By having a success rate of 83\%, our method outperforms other approaches. Furthermore, our method shows competitive efficiency with a mean travel time of 11.95 seconds. Overall, the results show the superiority of our approach in dealing with the complexities of cluttered dynamic environments, making it a promising solution for real-world applications in human-habitable environments.

\begin{table}[!h]
\caption{Comparisons in cluttered and dynamic environments}
\small
\centering
\label{dynamic}
\begin{tabular}{|
>{\columncolor[HTML]{3166FF}}p{2cm}|p{1cm}|p{4.1cm}|p{0.5cm}|}
\hline
\cellcolor[HTML]{FFFFFF}Method & \cellcolor[HTML]{009901}Success rate  & \cellcolor[HTML]{009901}Travel time(s)(mean,min/max) \\ \hline
log-MPPI                       &60\%                                 & 18.80/15.68/24.3                                                                            \\ \hline
MPPI                           & 53\%                                 &19.38,16.28/27.08                                                  \\ \hline
CEM                            & 46\%                                 & 11.95/9.57/14.21 
\\ \hline
DWA                            & 66\%                                 &      33.4,31.4/37.17  
\\ \hline\textbf{PRIEST}                          & \textbf{83\%}                        & \textbf{11.95}/\textbf{11.43/13.39}                                                              \\ \hline
\end{tabular}
\end{table}
\normalsize
\end{enumerate}

\noindent \textbf{Real-world Demonstration}

To conduct real-world experiments and compare the performance of \gls{priest} against \gls{teb}, \gls{dwa}, \gls{mppi}, and log-MPPI, we created a series of random indoor cluttered environments simulating scenarios similar to those available in the \gls{barn} dataset, with dimensions of $4m \times 8m$. The experimental platform involved a Clearpath Jackal equipped with Velodyne \gls{lidar}, and the robot's state was tracked using the OptiTrack Motion Capture System. The results of these experiments can be accessed on our website (\url{https://sites.google.com/view/priest-optimization}). The website includes videos demonstrating that \gls{priest} consistently outperforms the considered baselines in terms of the success rate metric.


\subsection{Interrelation:}

We extended the idea of proposing several initial guesses for trajectory optimization from our previous papers and utilized their techniques to leverage the optimization problem. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Paper IV}
% \subsection{Context:}
% \subsection{Contribution}
% \subsection{Main Results}
% \subsection{Validation and Benchmarking}
% \subsection{Interrelation:}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Paper VI}
\subsection{Context:}
This paper is the extension of paper I, and it introduces an innovative joint multi-agent trajectory optimization within the convex costs function frameworks. Our joint multi-agent trajectory optimization can be defined as:

\small
\begin{subequations}
\begin{align}
    \min_{x_{i}(t), y_{i}(t), z_{i}(t)} \sum_{i=1}^{N_{a}}\sum_{t=0}^{n_{p}} \Big(\ddot{x}^{2}_{i}(t)+\ddot{y}^{2}_{i}(t)+\ddot{z}^{2}_{i}(t) \Big)\label{cost_multiagent}  \\
    (x_{i}(t),\dot{x}_{i}(t),\ddot{x}_{i}(t) y_{i}(t), \dot{y}_{i}(t),\ddot{y}_{i}(t) z_{i}(t),\dot{z}_{i}(t),\ddot{z}_{i}(t))|_{t=t_{0}} = \textbf{b}_{0} \label{eq_multiagent_start}\\
    (x_{i}(t),\dot{x}_{i}(t),\ddot{x}_{i}(t) y_{i}(t), \dot{y}_{i}(t),\ddot{y}_{i}(t) z_{i}(t),\dot{z}_{i}(t),\ddot{z}_{i}(t))|_{t=t_{f}} = \textbf{b}_{f} \label{eq_multiagent_final}\\
   -\frac{(x_{i}(t)-x_{o}(t))^{2}}{a^2}-\frac{(y_{i}(t)-y_{o}(t))^{2}}{a^2}-\frac{(z_{i}(t)-z_{o}(t))^{2}}{b^2}+1\leq 0, \label{quadratic_multiagent}
\end{align}
\end{subequations}
\normalsize

\noindent In the cost function \eqref{cost_multiagent}, we aim to minimize the acceleration along the $x$, $y$, and $z$ axes. The vectors $\textbf{b}_{0}$ and $\textbf{b}_{f}$ denote the boundary values for each motion axis and its derivatives. The inequality constraint \eqref{quadratic_multiagent} captures collision avoidance constraints, modeling obstacles as spheroids with dimensions $(a, a, b)$. Solving this problem poses two main challenges: firstly, the complexity scales linearly with the number of agents, and secondly, the non-convex collision avoidance constraints exhibit exponential growth, ${n_o\choose{2}}$.

Existing solutions fall into two categories. The first group comprises sequential approaches \cite{park2020efficient}, where planners tackle one robot at a time. In this approach, the trajectories computed for previously planned robots serve as dynamic obstacles for the current robot under consideration. However, sequential planners encounter a significant drawback: as the planning process unfolds, each subsequent robot faces increasingly constrained feasible maneuvering space, potentially leading to infeasible solutions. 

On the other hand, \gls{mpc} decouples the planning process, allowing each~agent to perceive all others as dynamic obstacles with known trajectories at any given moment \cite{luis2019trajectory}. However, MPC implicitly accounts for cooperation between agents through trajectory prediction, and it tends to be conservative, offering access to a smaller feasible space.  Therefore, both classes of approaches suffer from conservatism and have limited access to feasible space.  

Based on the above discussion, in this paper, we explicitly address inter-agent cooperation by formulating a large-scale optimization problem to jointly compute the trajectories of all agents. The primary objective of this work is to enhance the computational efficiency of such large-scale optimization problems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contribution:}

The primary algorithmic challenge in multiagent trajectory optimization arises from the non-convex quadratic nature of inter-agent collision avoidance constraints, whose complexity escalates with an increasing number of agents. In this study, we address this challenge by first modeling non-convex collision avoidance as non-linear equality constraints through polar representation. Subsequently, we propose an \gls{am} procedure that organizes the optimization variables into specific blocks and optimizes them sequentially. An essential insight is that each block within our optimization problem exhibits a \gls{qp} structure with a fixed inverse component applicable to all agents. This allows us to precompute and cache the inverse part offline, effectively decomposing the large optimization problem into several parallel single-variable optimization subproblems.

\noindent Our proposed optimizer offers several distinct advantages over the \gls{sota} at the time of developing this paper:

\begin{enumerate}
    \item Ease of Implementation and \gls{gpu} Acceleration: Our optimizer's numerical computation primarily involves element-wise operations on vectors or matrix-vector products. These operations can be efficiently accelerated on \gls{gpu}s using libraries such as CUPY \cite{nishino2017cupy} and JAX \cite{bradbury2018jax}. We also provide an open-source implementation, which can compute trajectories for 32 agents in just 0.7 seconds on a desktop computer equipped with an RTX-2080 \gls{gpu}.
    \item \gls{sota} Performance: Our optimizer significantly outperforms the computation time of joint trajectory optimization methods \cite{augugliaro2012generation} while achieving trajectories of comparable quality. It also surpasses the current \gls{sota} sequential approaches \cite{park2020efficient} by producing shorter trajectories in benchmark tests. Moreover, it exhibits improved computation times on several benchmarks despite conducting a more rigorous joint search over the agents' trajectory space.
    \item Suitability for Edge Devices: Our optimizer can efficiently compute trajectories for 16 agents in approximately 2 seconds on an Nvidia Jetson-TX2. This performance is nearly two orders of magnitude faster than the computation time of \cite{augugliaro2012generation} on standard desktop computers. As a result, our work enhances the onboard decision-making capabilities of agents like quadrotors, which may have limited computational resources. To our knowledge, there are no existing works that achieve similar performance on edge devices at the time of working on this paper.

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Main Results}
Considering the same motivation as Section \ref{main_result_1}, we reformulate collision avoidance constraint, $\textbf{f}_{o} =0$ as

\vspace{-0.2cm}
\small
\begin{align}
     \textbf{f}_{o} = \left \{ \begin{array}{lcr}
\colorbox{my_green}{$x_{i}(t) -x_{j}(t)-a d_{ij}(t)\sin\beta_{ij}(t)\cos\alpha_{ij}(t)$}\\
\colorbox{my_pink}{$y_{i}(t) -y_{j}(t)-a d_{ij}(t)\sin\beta_{ij}(t)\sin\alpha_{ij}(t)$}\\ 
\colorbox{my_blue}{$z_{i}(t) -z_{j}(t)-b d_{ij}\cos\beta_{ij}(t)$} \\
\end{array} \right \},d_{ij}\geq 1
\label{sphere_proposed}
\end{align}
\normalsize

\noindent where $d_{ij}(t), \alpha_{ij}(t)$ and $\beta_{ij}(t)$ are optimization variables which are needed to be computed. Similar to previous works, to exploit the hidden convex structure within \eqref{cost_multiagent}-\eqref{eq_multiagent_final} and \eqref{sphere_proposed}, we utilize the augmented Lagrangian method for our optimization problem.

\small
\begin{subequations}
\begin{align}
\min_{\scalebox{0.7}{$\begin{matrix}x_{i}(t), y_{i}(t), z_{i}(t), \\
\alpha_{ij}(t), \beta_{ij}(t), d_{ij}(t)\end{matrix}$}}  \hspace{-0.2cm}\sum_{i=1}^{N_{a}}\sum_{t=t_1}^{n_{p}}\hspace{-0.1cm}\Big( \ddot{x}^{2}_{i}(t)\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{y}^{2}_{i}(t)\hspace{-0.1cm}+\hspace{-0.1cm}\ddot{z}^{2}_{i}(t)
\hspace{-0.1cm}+\hspace{-0.3cm}\sum_{j=1, j \neq i}^{j=N_{a}}\hspace{-0.1cm}\big (\frac{\rho_{o}}{2}(\hspace{-0.05cm}\frac{\lambda_{x_{ij}}(\hspace{-0.02cm}t\hspace{-0.02cm})}{\rho_{o}}\hspace{-0.01cm}\colorbox{my_green}{\hspace{-0.2cm}$+\hspace{-0.1cm}x_{i}(t)\hspace{-0.1cm}-x_{j}(t)$}\nonumber \\\colorbox{my_green}{\hspace{-0.2cm}$-ad_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})\sin\beta_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})\cos\alpha_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})$})^2  \hspace{-0.1cm}+\hspace{-0.1cm}\frac{\rho_{o}}{2}(\colorbox{my_blue}{$z_{i}(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.1cm}-\hspace{-0.1cm}z_{j}(\hspace{-0.02cm}t\hspace{-0.02cm})\hspace{-0.1cm}-\hspace{-0.1cm}bd_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})\cos\beta_{ij}(t)\hspace{-0.1cm}+\hspace{-0.1cm}\frac{\lambda_{z_{ij}}(\hspace{-0.02cm}t\hspace{-0.02cm})}{\rho_{o}})$}^2\big)\nonumber \\
    +\frac{\rho_{o}}{2}(\colorbox{my_pink}{$y_{i}(t) -y_{j}(t)-ad_{ij}(t)\sin\beta_{ij}(t)\sin\alpha_{ij}(t)$}+\frac{\lambda_{y_{ij}}(t)}{\rho_{o}})^2 \Big)
    \label{aug_lagrange_multi}
\end{align}
\end{subequations}
\normalsize

\noindent where $\lambda_{x_{ij}}(t), \lambda_{y_{ij}}(t), \lambda_{z_{ij}}(t)$ are time-dependent Lagrange multipliers and  $\rho_{o}$ is a scalar constant. We can utilize the \gls{am} method to solve \eqref{aug_lagrange_multi} with respect to optimization variables. Alg. \ref{alg_5} provides a summary of the steps involved in solving \eqref{aug_lagrange_multi} subject to \eqref{eq_multiagent_start} and \eqref{eq_multiagent_final}. In the next section, we go through the details of each step of Alg. \ref{alg_5}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!h]
\DontPrintSemicolon
\SetAlgoLined
\SetNoFillComment
\scriptsize
\caption{\scriptsize Alternating Minimization for Solving Multi-agent Trajectory Optimization \eqref{cost_multiagent}-\eqref{quadratic_multiagent}}\label{alg_5}
\KwInitialization{Initiate $^{k}d_{ij}(t)$, $^{k}\alpha_{ij}(t)$, $^{k}\beta_{ij}(t)$  }
\While{$k \leq maxiter$}{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Compute $^{k+1}x_{i}(t)$,$^{k+1}y_{i}(t)$ and $^{k+1}z_{i}(t)$ 
\vspace{-0.4cm}
\begin{subequations}
    \begin{align}
^{k+1}x_{i}(t)=\arg \min_{x_{i}(t)}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\ddot{x}_{i}^{2}(t) \nonumber \\
\hspace{-0.1cm}+\hspace{-0.1cm}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\sum_{j=1,j\neq i}^{j=N_{a}}\hspace{-0.1cm}\frac{\rho_{o}}{2}(\colorbox{my_green}{$\hspace{-0.1cm}x_{i}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}x_{j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k}d_{ij}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.05cm}\cos{^{k}\alpha_{ij}}(\hspace{-0.02cm}t\hspace{-0.03cm}) \hspace{0.03cm}\sin{^{k}\beta_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}}\hspace{-0.1cm}+\hspace{-0.1cm}\frac{^{k}\lambda_{x_{ij}}}{\rho_{o}})^{2} \label{com_xi}\\
   ^{k+1}y_{i}(t)
  =\arg \min_{y_{i}(t)}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\ddot{y}_{i}^{2}(t)\nonumber \\
\hspace{-0.2cm}+\hspace{-0.1cm}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\sum_{j=1,j\neq i}^{j=N_{a}}\hspace{-0.1cm}\frac{\rho_{o}}{2}(\colorbox{my_pink}{$\hspace{-0.1cm}y_{i}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.07cm}-\hspace{-0.07cm}y_{j}(\hspace{-0.03cm}t\hspace{-0.03cm})
\hspace{-0.07cm}-\hspace{-0.07cm}a\hspace{0.03cm}^{k}d_{ij}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}\sin{^{k}\alpha_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}\sin{^{k}\beta_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}$}\hspace{-0.1cm}+\hspace{-0.1cm}\frac{^{k}\lambda_{y_{ij}}}{\rho_{o}})^2 \label{com_yi}\\
^{k+1}z_{i}(t)=\arg \min_{z_{i}(t)}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\ddot{z}_{i}^{2}(t)\nonumber \\
\hspace{-0.07cm}+\hspace{-0.2cm}\sum_{t=0}^{t=n_p}\sum_{i=1}^{i=N_{a}}\sum_{j=1,j\neq i}^{j=N_{a}}\frac{\rho_{o}}{2}(\colorbox{my_blue}{$z_{i}(t)-z_{j}(t) -b\hspace{0.05cm}^{k}d_{ij}\hspace{0.05cm}\cos{^{k}\beta_{ij}}(t)$}+\frac{^{k}\lambda_{z_{ij}}}{\rho_{o}} )^{2} \label{com_zi}
\end{align}
\end{subequations}
\vspace{-0.45cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}\alpha_{ij}(t)$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.3cm}
\begin{align}
    \hspace{0.05cm}^{k+1}\alpha_{ij}(t) =  \arctan 2\Big((^{k+1}y_{i}(t)-^{k+1}y_{j}(t)),(^{k+1}x_{i}(t)-^{k+1}x_{j}(t))\Big) \label{com_alpha_i}
\end{align}
\vspace{-0.4cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}\beta_{ij}(t)$
%%%%%%%%%%%%%%%%%%
\vspace{-0.3cm}
\begin{align}
    \hspace{0.05cm}^{k+1}\beta_{ij}(t) = \arctan 2\Big((\frac{^{k+1}x_{i}(t)-^{k+1}x_{j}(t)}{a \cos{^{k+1}\alpha_{ij}(t)}}),(\frac{^{k+1}z_{i}(t)-^{k+1}z_{j}(t)}{b })\Big)
    \label{com_beta_i}
\end{align}
\vspace{-0.5cm}
%%%%%%%%%%%%%%%%%%%%%%%

\hspace{-0.15cm}Compute $\hspace{0.05cm}^{k+1}d_{ij}(t)$ through 
\begin{align}
    \hspace{-0.5cm}^{k+1}d_{ij}(t)\hspace{-0.1cm}=\hspace{-0.1cm}\arg \min_{d_{ij}(t)}\hspace{-0.1cm}\sum_{t}\sum_{i}\sum_{j}\hspace{-0.07cm}\frac{\rho_{o}}{2}\hspace{-0.04cm}\Big(\hspace{-0.07cm}(\colorbox{my_blue}{\hspace{-0.1cm}$^{k+1}z_{i}(t)-^{k+1}z_{j}(t) -b\hspace{0.05cm}^{k+1}d_{ij}\hspace{0.05cm}\cos{^{k+1}\beta_{ij}}(t)$\hspace{-0.2cm}}\hspace{-0.05cm}+\frac{^{k}\lambda_{z_{ij}}}{\rho_{o}} )^{2}
    \nonumber \\+(\colorbox{my_green}{$\hspace{-0.1cm}^{k+1}x_{i}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}^{k+1}x_{j}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}-\hspace{-0.1cm}a\hspace{0.03cm}^{k+1}d_{ij}(\hspace{-0.03cm}t\hspace{-0.03cm})\cos{^{k+1}\alpha_{ij}}(\hspace{-0.02cm}t\hspace{-0.03cm}) \sin{^{k+1}\beta_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})$\hspace{-0.1cm}}\hspace{-0.1cm}+\hspace{-0.1cm}\frac{^{k}\lambda_{x_{ij}}}{\rho_{o}})^{2}+ \nonumber \\(\colorbox{my_pink}{$\hspace{-0.1cm}^{k+1}y_{i}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.07cm}-\hspace{-0.07cm}^{k+1}y_{j}(\hspace{-0.03cm}t\hspace{-0.03cm})
\hspace{-0.07cm}-\hspace{-0.07cm}a\hspace{0.03cm}^{k+1}d_{ij}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}\sin{^{k+1}\alpha_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{0.03cm}\sin{^{k+1}\beta_{ij}}(\hspace{-0.03cm}t\hspace{-0.03cm})\hspace{-0.1cm}$}\hspace{-0.1cm}+\hspace{-0.1cm}\frac{^{k}\lambda_{y_{ij}}}{\rho_{o}})^2
    \label{com_d_i}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{-0.15cm}Update $\lambda_{x_{ij}}(t), \lambda_{y_{ij}}(t), \lambda_{z_{ij}}$ at $k+1$
}
\normalsize

\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Analysis and Description of Alg. \ref{alg_5}:}

\noindent \textbf{Line 2}: 
The significant characteristic of the optimization problem \eqref{aug_lagrange_multi} is that we can transform the optimization problem into \gls{qp} forms where matrices remain constant across iterations. To achieve this, we examine \eqref{aug_lagrange_multi} and restructure the optimization problem by including only terms involving $x_{i}(t)$ as \eqref{com_xi}.  Subsequently, using \eqref{param}, we parameterize the optimization variable, $x_{i}(t)$ and $x_{j}(t)$ and rewrite each terms of \eqref{com_xi} as

\small
\begin{subequations}
\begin{align}
\hspace{-0.2cm}\min_{\textbf{c}_{x}} \frac{1}{2}\textbf{c}_{x}^T\textbf{Q}_{x} \textbf{c}_x\hspace{-0.1cm}+\hspace{-0.1cm}\hspace{-0.1cm}\Big(\frac{1}{2}\rho_{o}\textbf{c}_{x}^T\textbf{A}_{f_o}^T\textbf{A}_{f_o}\textbf{c}_{x}\hspace{-0.1cm}-\hspace{-0.1cm}(\rho_{o}\textbf{A}_{f_o}^T{^k}\textbf{b}_{f_o}^x)^T\textbf{c}_x\Big),
\text{st:}~~\textbf{A}_{eq}\textbf{c}_x\hspace{-0.1cm}=\hspace{-0.1cm}\textbf{b}_{eq}^x \label{eq_step_x}
\end{align}
\end{subequations}
\normalsize

\noindent where $\textbf{c}_{x}$ is the stack of $\textbf{c}_{x_{i}}$ for all the agents and $\textbf{c}_{x_{i}}$ is the coefficient associated with the basis functions. The initial two terms in \eqref{eq_step_x} are the parameterized and simplified representations of the corresponding terms in \eqref{com_xi}. In the following, we show how this simplification is done and define each matrix and vector used in \eqref{eq_step_x}

\vspace{-0.2cm}
\small
\begin{subequations}
\begin{align}
   \sum_{t}\sum_{i}\ddot{x}_i(t)^2 \Rightarrow \frac{1}{2}\textbf{c}_x^T\textbf{Q}_x\textbf{c}_x,  \textbf{Q}_x = \begin{bmatrix}
    \ddot{\textbf{P}}^T\ddot{\textbf{P}} & & \\
    & \ddots  & \\
    & & \ddot{\textbf{P}}^T\ddot{\textbf{P}}
    \end{bmatrix}\\
    \sum_{t}\sum_{i}\sum_{j} \frac{\rho_{o}}{2}\Big(x_i(t)\hspace{-0.1cm}-\hspace{-0.1cm}x_j(t)\hspace{-0.1cm}-\hspace{-0.1cm}a{^k}d_{ij}(t)\sin{^k}\beta_{ij}(t)\cos{^k}\alpha_{ij}(t)\hspace{-0.1cm}+\hspace{-0.1cm}\frac{{^k}\lambda_{x_{ij}}(t)}{\rho}\Big)^2  \nonumber \\
        \Rightarrow \frac{\rho}{2}\Vert \textbf{A}_{f_c} \textbf{c}_x-{^k}\textbf{b}_{f_c}^x\Vert_2^2,  
          {^k}\textbf{b}_{f_c}^x = a{^k}\textbf{d} \sin{^k}\boldsymbol{\beta}\cos{^k}\boldsymbol{\alpha}-\frac{\boldsymbol{{^k}\lambda_{x_{ij}}}}{\rho}
\nonumber \\
\textbf{A}_{f_c}\hspace{-0.1cm}=\hspace{-0.1cm}\begin{bmatrix}
    \textbf{A}_{1}\hspace{-0.1cm}& & \\
    & \hspace{-0.1cm}\ddots \hspace{-0.1cm}& \\
    & &\hspace{-0.1cm}\textbf{A}_{n_{o}}
  \end{bmatrix},
\textbf{A}_{n_{o}}\hspace{-0.1cm}=\hspace{-0.1cm}\begin{bmatrix}
     \begin{pmatrix}
     \textbf{P}\\
     \textbf{P}\\
      \vdots\\
      \textbf{P}
     \end{pmatrix}_{\hspace{-0.1cm}\times n-n_{o}}\hspace{-0.2cm}&\hspace{-1.2cm}\begin{bmatrix}
    -\textbf{P} & & \\
    & \ddots & \\
    & & -\textbf{P}
  \end{bmatrix}_{\hspace{-0.1cm}\times n-n_{o}}
    \end{bmatrix}
    \label{A_f} \\
  \textbf{A}_{eq} = \begin{bmatrix}
    \textbf{A} & & \\
    & \ddots & \\
    & & \textbf{A}
    \end{bmatrix}, \textbf{A} = \begin{bmatrix}
    \textbf{P}_{0}&
    \dot{\textbf{P}}_{0}&
    \ddot{\textbf{P}}_{0}&
    \textbf{P}_{-1}&
    \dot{\textbf{P}}_{-1}&
    \ddot{\textbf{P}}_{-1}&
    \end{bmatrix}^{T}
\end{align}
\end{subequations}
\normalsize



\noindent Now, the problem \eqref{eq_step_x} can be reduced to a set of linear equations as 

\small
\begin{align}
    \overbrace{\begin{bmatrix}
(\textbf{Q}_x+\rho\textbf{A}_{f_c}^T\textbf{A}_{f_c}) & \textbf{A}_{eq}^T\\
    \textbf{A}_{eq} & \textbf{0}
    \end{bmatrix} }^{\widetilde{\textbf{Q}}_x} \begin{bmatrix}
    \textbf{c}_x\\
    \boldsymbol{\nu}
    \end{bmatrix} = \overbrace{\begin{bmatrix}
    \rho\textbf{A}_{f_c}^T{^k}\textbf{b}_{f_c}^x\\
    \textbf{b}_{eq}^x
    \end{bmatrix}}^{\widetilde{\textbf{q}}_x}
\label{kkt_step_x}
\end{align}
\normalsize

\noindent where $\boldsymbol{\nu}$ is the dual optimization variable. 

\noindent \textbf{Line 3:} We adopt the geometrical intuition from the main results of the first provided paper, Section \ref{main_result_1} to solve \eqref{com_alpha_i}. 

\noindent \textbf{Line 4:} Similar to previous step, we obtain \eqref{com_beta_i}.

\noindent \textbf{Line 5-6:} As the optimization variables $d_{ij}(t)$ are independent across different time instances and agents, the optimization problem \eqref{com_d_i} can be decomposed into $n_{p}\times{n_o\choose{2}}$ \gls{qp} problems, each with a single variable. Consequently, we can readily express the problem symbolically. It is important to note that the bounds on $d_{ij}(t)$ are maintained by clipping the values to the interval $[0,1]$ at each iteration.

\noindent \textbf{Line 7:} We update the Lagrange multipliers as

\vspace{-0.3cm}
\small
\begin{subequations}
    \begin{align}
        \hspace{-0.15cm}{^{k+1}\hspace{-0.05cm}}\lambda_{x_{ij}}\hspace{-0.05cm}(\hspace{-0.032cm}t\hspace{-0.032cm})\hspace{-0.1cm}=\hspace{-0.15cm}^{k\hspace{-0.05cm}}\lambda_{x_{ij}}\hspace{-0.05cm}\hspace{-0.05cm}(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}+\hspace{-0.1cm}\rho_{o}(\hspace{-0.033cm}{^{k+1}\hspace{-0.05cm}}x_i(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}-\hspace{-0.17cm}{^{k+1}\hspace{-0.05cm}}x_j(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}-\hspace{-0.1cm}a{^{k+1}\hspace{-0.05cm}}d_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\sin{^{k+1}\hspace{-0.05cm}}\beta_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\cos{^{k+1}\hspace{-0.05cm}}\alpha_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.033cm}) \label{update_lamda_xi} \\
 \hspace{-0.15cm}{^{k+1}\hspace{-0.05cm}}\lambda_{y_{ij}}\hspace{-0.05cm}(\hspace{-0.032cm}t\hspace{-0.033cm})\hspace{-0.1cm}=\hspace{-0.15cm} {^{k}\hspace{-0.05cm}}\lambda_{y_{ij}}\hspace{-0.05cm}(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}+\hspace{-0.1cm}\rho_{o}({^{k+1}\hspace{-0.05cm}}y_i(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}-\hspace{-0.17cm}{^{k+1}\hspace{-0.05cm}}y_j(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.1cm}-\hspace{-0.1cm}a{^{k+1}\hspace{-0.05cm}}d_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\sin{^{k+1}\hspace{-0.05cm}}\beta_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\sin{^{k+1}\hspace{-0.05cm}}\alpha_{ij}(\hspace{-0.033cm}t\hspace{-0.033cm})\hspace{-0.033cm}) \label{update_lamda_yi} \\
 \hspace{-0.1cm}{^{k+1}}\lambda_{z_{ij}}(\hspace{-0.02cm}t\hspace{-0.02cm}) =  {^{k}}\lambda_{z_{ij}}(\hspace{-0.02cm}t\hspace{-0.02cm})+\rho_{o}({^{k+1}}z_i(\hspace{-0.02cm}t\hspace{-0.02cm}) -{^{k+1}}z_j(\hspace{-0.02cm}t\hspace{-0.02cm})-b{^{k+1}}d_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})\cos{^{k+1}\hspace{-0.05cm}}\beta_{ij}(\hspace{-0.02cm}t\hspace{-0.02cm})).\label{update_lamda_zi}
    \end{align}
\end{subequations}
\normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation and Benchmarking}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Implementation Details:}

We implemented Algorithm 5 using
Python with the JAX \cite{bradbury2018jax} and CUPY \cite{nishino2017cupy} library as the GPU-accelerated algebra backend. More specifically, the CUPY is used for trajectory optimization of up to 32 agents. All the benchmarks were conducted on a desktop computer with RTX 2080 featuring an Intel Core i7 processor and 32 GB RAM. 

In our implementations, agents were modeled as spheres for simplicity, and a circumscribing sphere was constructed for static obstacles to integrate them into our optimizer. In addition, to enhance the convergence of Alg. \ref{alg_5}, we precomputed the inverse of $\widetilde{\textbf{Q}}_x$ in \eqref{kkt_step_x} for ten incrementally higher values of $\rho_{o}$. These values were used in the latter iterations of Alg. \ref{alg_5} and are inspired from \cite{xu2017admm}.
For a fair comparison with \cite{augugliaro2012generation} and \cite{park2020efficient}, we utilized their open-source implementations and datasets. In the comparison with \cite{augugliaro2012generation}, we omitted hard bounds on position, velocities, and accelerations, resulting in a reduction in the number of inequality constraints. Similarly, we adjusted the "downwash" parameter in \cite{park2020efficient} to 1 to align with our optimizer's implementation. As trajectories obtained from our optimizer, \cite{augugliaro2012generation}, and \cite{park2020efficient} operate at different time scales, we employed the second-order finite difference of the position as a proxy for comparing accelerations across these three methods. In addition, we compared our approach with different baselines in two sets of benchmarks, including:

\begin{itemize}
\item \textbf{Square Benchmark:} The agents are positioned along the perimeter of a square and tasked with reaching their antipodal positions.
\item \textbf{Random  Benchmark with static obstacles:} In this scenario, the starting and goal positions of the agents are randomly sampled. Additionally, we introduce a modified version of this benchmark where static obstacles are randomly distributed within the workspace.
\end{itemize}

\noindent \textbf{Qualitative Results}

We showed the qualitative results for different benchmarks that we used in Fig. \ref{multi-bench}. Also, we provided snapshots of 32 agents exchanging positions in a narrow hallway in Fig. \ref{multi-snap}. For better understanding, we demonstrated trajectories obtained from our proposed algorithm and \gls{rvo} in Fig. \ref{rvo_multi}. 

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.325]{figures/qual_2.png}
    \caption[Qualitative trajectories for different benchmarks]{\small{Qualitative trajectories for square and random benchmarks without static obstacles and random benchmark with static obstacles.}}
    \label{multi-bench}
    \end{figure}
    
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.325]{figures/multiagent_snapshots.png}
    \caption[Qualitative trajectories for 32 agents in a narrow hallway]{\small{Collision avoidance snapshots of 32 agents exchanging positions in a
 narrow hallway is shown. The start and goal positions are marked with a "X" and a "o" respectively.}}
    \label{multi-snap}
    \end{figure}
    

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.37]{figures/Document systems_4.png}
    \caption[RVO vs. Alg. \ref{alg_5} trajectories for different number of agents]{\small{Trajectories obtained for the proposed optimizer for the 16, 32, and 64 agents are shown in the first column, while trajectories obtained using RVO are shown in the second column}}
    \label{rvo_multi}
    \end{figure}

\noindent \textbf{Algorithm Validation:}
As mentioned in previous works, a key to validating our trajectory optimization algorithm is to show that residuals are going to zero over iterations across various benchmarks. e generated this plot by averaging residuals from 20 distinct problem instances. Typically, around 150 iterations were adequate to achieve residuals of approximately $0.01$. It's worth noting that these residuals represent the norm of a vector comprising tens of thousands (${n\choose 2} m$) of elements. For instance, with 64 robots, each of the collision avoidance vectors along the x, y and z axis, $\textbf{f}_c^x, \textbf{f}_c^y, \textbf{f}_c^z$ contains more than $2\times10^6$ elements. Hence, it's crucial to monitor both the norm and the maximum magnitude across these vector elements to ascertain the convergence of Algorithm \ref{alg_5}. We observed that individual elements of the residual vector often have magnitude around $10^{-3}$ or lower even when the residual is around $0.01$. We can allow the optimizer to run for more iterations to obtain even lower residuals. Our implementation uses an additional practical trick.  We inflate the radius of the agents by four times the typical residual we observe after 150 iterations of our optimizer. In practice, this increased the agent's dimensions by around $4 cm$.

\noindent \textbf{Quantitative Results}

\begin{enumerate}[label=\alph*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textit{Computation time}
Fig. \ref{comp_time_room} (a) shows the average computation time of our optimizer for varying numbers of agents (with radii of 0.4 meters), relative to the proximity of initial and final positions. Specifically, we randomly sampled initial and final positions within square rooms of varying dimensions to generate problem instances of differing complexity levels. As can be seen, even in the most challenging scenarios, our optimizer successfully computed trajectories for 32 agents in approximately 1 second.

In Fig. \ref{comp_time_room} (b), we depict the computation time for 16 agents under varying numbers of static obstacles. Our optimizer exhibits nearly linear scalability in computation time. This behavior arises because the inclusion of static obstacles primarily impacts the computational cost of obtaining $\textbf{A}{f_o}^T{^k}\textbf{b}{f_o}^x$ in equation (\ref{kkt_step_x}). Furthermore, both the matrix and vector dimensions increase linearly with the number of obstacles, and the resultant product is distributed across \gls{gpu}s.

\begin{figure}[!h]
  \centering  
    \includegraphics[scale=0.3] {figures/comp_time_room.png}
\caption[Computation time]{ Fig. (a) shows computation time for a varying number of agents
for benchmarks where we sample start and goal positions from a square with varying lengths. Fig. (b) shows the linear scaling of computation time with obstacles for a given number of agents.  }
    \label{comp_time_room}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\item \textit{Comparison with \gls{rvo} \cite{van2008reciprocal}:}

The \gls{rvo} \cite{van2008reciprocal} is a widely used local, reactive planning approach in multi-agent navigation. While \gls{rvo} focuses on immediate collision avoidance in a single step, our optimizer tackles the more intricate task of global multi-agent trajectory optimization across multiple steps (100 in our implementation). Despite this fundamental difference, we benchmark our optimizer against \gls{rvo} to establish a baseline for trajectory quality comparison.

It is worth noting that the computation time of \gls{rvo} is notably faster (three times faster in the benchmark with 16 agents) compared to our optimizer. However, the trajectory comparison results, summarized in Table \ref{RVO-table}, reveal that \gls{rvo} produces slightly shorter trajectories than our optimizer. This discrepancy arises because \gls{rvo} operates with single-integrator agents, allowing for abrupt velocity changes. In contrast, our optimizer generates polynomial trajectories that prioritize higher-order differentiability.

Furthermore, while \gls{rvo}'s use of abrupt velocity changes enables shorter trajectories, it also incurs a substantially higher smoothness cost compared to our optimizer. This trade-off highlights the differing optimization priorities between the two methods.

%%%%%%%%%%%%%
\begin{table}[]
\centering
\scriptsize
\caption{\small{Comparison with \gls{rvo} \cite{van2008reciprocal}}}
\label{RVO-table}
\begin{tabular}{|l|l|l|l|}
\hline
\rowcolor[HTML]{009901} 
Number of agents                                    & \multicolumn{1}{l|}{\cellcolor[HTML]{009901}Benchmark} & \multicolumn{1}{l|}{\cellcolor[HTML]{009901}Arc-length(m)} & \multicolumn{1}{l|}{\cellcolor[HTML]{009901}Smoothness cost}     \\ \hline
\rowcolor[HTML]{9ADC9A} 
\cellcolor[HTML]{009901}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}RVO}       & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}9.491/1.12}    & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}0.217/0.1}           \\ \cline{2-4} 
\rowcolor[HTML]{66BC8D} 
\multirow{-2}{*}{\cellcolor[HTML]{009901}16 agents} & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}Our}       & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}9.877/1.33}    & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}\textbf{0.062/0.01}} \\ \hline
\rowcolor[HTML]{9ADC9A} 
\cellcolor[HTML]{009901}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}RVO}       & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}9.348/0.94}    & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}0.26/0.11}           \\ \cline{2-4} 
\rowcolor[HTML]{66BC8D} 
\multirow{-2}{*}{\cellcolor[HTML]{009901}32 agents} & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}Our}       & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}9.613/1.12}    & \multicolumn{1}{l|}{\cellcolor[HTML]{66BC8D}\textbf{0.06/0.01}}  \\ \hline
\rowcolor[HTML]{9ADC9A} 
\cellcolor[HTML]{009901}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}RVO}       & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}9.360.99}      & \multicolumn{1}{l|}{\cellcolor[HTML]{9ADC9A}0.228/0.09}          \\ \cline{2-4} 
\rowcolor[HTML]{66BC8D} 
\multirow{-2}{*}{\cellcolor[HTML]{009901}64 agents} & Our                                                    & 9.439/1.07                                                 & \textbf{0.064/0.01}                                              \\ \cline{1-1}
\end{tabular}
\end{table}
%%%%%%%%%%%


\item \textit{Comparison with \cite{augugliaro2012generation}}
Fig. \ref{scp_compare} provides a comparison of trajectory quality between our optimizer and the approach proposed in \cite{augugliaro2012generation}. Despite both optimizers converging to different trajectories, the arc-length statistics observed across all agents are remarkably similar. Moreover, our optimizer demonstrates superior performance in terms of trajectory smoothness cost compared to \cite{augugliaro2012generation}.

The mean computation time required by the \gls{scp} approach of \cite{augugliaro2012generation} across various 8-agent square benchmarks was approximately 6.79 seconds. In contrast, our optimizer exhibited significantly faster computation times, being 28 times faster with an average of only $0.242$ seconds. This gap in computation time became even more pronounced with an increase in the number of agents to 16, with the \gls{scp} approach of \cite{augugliaro2012generation} taking approximately $160.76$ seconds, while our optimizer was 613 times faster at $0.262$ seconds.

The observed trend in computation time is unsurprising, as the number of inequality constraints in \cite{augugliaro2012generation}, stemming from collision avoidance, scales combinatorially as ${n \choose 2}$. In contrast, our optimizer employs a computational structure that circumvents this intractability by pre-computing expensive matrix inverses and parallelizing matrix-vector products on \gls{gpu}s.

It is essential to note that GPU acceleration of the \gls{scp} approach of \cite{augugliaro2012generation} remains a challenging open problem.


\begin{figure}[!h]
\centering
\includegraphics[scale=0.31] {figures/new-fig5.png}
\caption[Comparisons with state-of-the-art]{Comparisons with \gls{sota} \cite{augugliaro2012generation} in terms of arc-length and smoothness cost}
\label{scp_compare}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \textit{Comparison with \cite{park2020efficient}}
Fig. \ref{rbp_compare} shows the most important results of this study, where we compare our optimizer with the current \gls{sota} method, \cite{park2020efficient}. The \cite{park2020efficient} employs a sequential approach with a batch of agents and harnesses the parallel \gls{qp} solving capabilities of CPLEX \cite{cplex} on multi-core \gls{cpu}s. Our optimizer yields trajectories with comparable smoothness to \cite{park2020efficient} but with significantly shorter arc lengths. This disparity can be attributed to the reduced feasible space accessible to a sequential approach.

Moreover, our optimizer surpasses \cite{park2020efficient} in terms of computation time for 16 and 32 agent benchmarks, while achieving comparable performance on the 64 agent benchmark. It's crucial to contextualize these timings by acknowledging that our optimizer conducts a much more exhaustive search than \cite{park2020efficient} across the joint trajectory space of the agents. The trends in computation time can be explained as follows: for a smaller number of agents, the computation time of \cite{park2020efficient} is primarily influenced by the trajectory initialization derived from sampling-based planners. Additionally, the overhead of \gls{cpu} parallelization is substantial for fewer agents, but this overhead is offset by the computational speed-up attained for a larger number of agents.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.27] {figures/new-out.png}
\caption[Comparisons with state-of-the-art]{Comparisons with \gls{sota} \cite{park2020efficient} in terms of arc-length and smoothness cost and computation time}
\label{rbp_compare}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\item \textit{Performance on Jetson TX2}
Table \ref{table_jetson} displays the computation time for varying numbers of agents in the square benchmark conducted on the Nvidia Jetson TX2 platform. The starting and ending positions are randomly selected within an 8-meter square area. The results demonstrate that our optimizer facilitates rapid on-board decision-making for up to 16 agents. Furthermore, even with 32 agents, the computation time remains sufficiently low to be applicable in practical scenarios.

\begin{table}[]
\centering
\scriptsize
\caption{\small{Computation time on Nvidia-Jetson TX2}:}
\label{table_jetson}
\begin{tabular}{|l|l|} 
\hline
\rowcolor[HTML]{036400} 
{\color[HTML]{FFFFFF} Square Benchmark} & {\color[HTML]{FFFFFF} Computation time} \\ \hline
\rowcolor[HTML]{68CBD0} 
8 agents, radius $= 0.1/0.6/1.2$        & 1.01/1.32/1.27                          \\ \hline
\rowcolor[HTML]{68CBD0} 
16 agents, radius $= 0.3/0.6$           & 2.10/2.34                               \\ \hline
\rowcolor[HTML]{68CBD0} 
32 agents, radius $= 0.25$              & 7.70                                    \\ \hline
\end{tabular}
\end{table}
\end{enumerate}




%%%%%%%%%%%%%





\subsection{Interrelation:}

Our optimizer extends the single-agent trajectory optimization method introduced in paper I to a multi-agent setting. More specifically, we develop the multi-agent version of the collision avoidance model and reconfigure the underlying matrix algebra to facilitate distributed computations on \gls{gpu}. This approach explores a feature that has not been previously leveraged in previous work.



==> sections/listofpublications2.tex <==
\chapter*{List of Other Publications}
\addcontentsline{toc}{chapter}{List of other publications}
\section*{Other Publications}

